Factor Adjusted Spectral Clustering for Mixture Models

This paper studies a factor modeling-based approach for clustering high-dimensional data generated from a mixture of strongly correlated variables. Statistical modeling with correlated structures pervades modern applications in economics, finance, genomics, wireless sensing, etc., with factor modeling being one of the popular techniques for explaining the common dependence. Standard techniques for clustering high-dimensional data, e.g., naive spectral clustering, often fail to yield insightful results as their performances heavily depend on the mixture components having a weakly correlated structure. To address the clustering problem in the presence of a latent factor model, we propose the Factor Adjusted Spectral Clustering (FASC) algorithm, which uses an additional data denoising step via eliminating the factor component to cope with the data dependency. We prove this method achieves an exponentially low mislabeling rate, with respect to the signal to noise ratio under a general set of assumptions. Our assumption bridges many classical factor models in the literature, such as the pervasive factor model, the weak factor model, and the sparse factor model. The FASC algorithm is also computationally efficient, requiring only near-linear sample complexity with respect to the data dimension. We also show the applicability of the FASC algorithm with real data experiments and numerical studies, and establish that FASC provides significant results in many cases where traditional spectral clustering fails.

==> texfiles/old/intro.tex <==
\section{Introduction}

Highly correlated data are a stylized feature in  many applications. Examples scatter arounds the applications in macroeconomic \citep{bai2002determining}, finance \citep{fama2015five}, and computational biology \citep{fan2014challenges} and social science \citep{zhou2015measuring}.   This feature affects adversally statistical analysis such as model selection \citep{FAN202071} and  multiple testing \citep{doi:10.1080/01621459.2018.1527700}, as well as clustering, which is a subject of our study.

Clustering, an important unsupervised problem in statistics and machine learning that aims to partition data into groups of  more homogeneous samples, is also adversely affected by the correlations among observed variables. To illustrate this, consider the following toy example of the Gaussian mixture model in $d$-dimension: 
% \begin{equation*}
%     \bx_{i} \sim \frac{1}{2}\mathcal{N}(-\bmu, \bSigma) + \frac{1}{2}\mathcal{N}(\bmu, \bSigma)
% \end{equation*}
\begin{equation*}
    \PP(y_i=1)=\PP(y_i=-1)=\frac{1}{2} \quad \mbox{and} \quad \bx_i | y_i \sim \mathcal{N}(y_i \bmu, \bSigma)
\end{equation*}
with the goal to recover the unobserved class label $y_i \in \pm 1$ for each observation $\bx_i$.  
Given $\boldsymbol{\mu}$ and $\bSigma$, the optimal classifier is $\text{sgn}(\langle  \bx_{i} , \bSigma^{-1} \boldsymbol{\mu} \rangle)$, which achieves the optimal misclassification rate $\Phi(-\sqrt{\text{SNR}}) $, where the signal-to-noise ratio is  $\text{SNR}=\boldsymbol{\mu}^{T} \bSigma^{-1} \boldsymbol{\mu}$. However, when the variables are highly correlated, this optimal misclassification rate is not always achievable by many conventional computationally efficient clustering algorithms (e.g., spectral clustering), as the following numerical experiment (Figure \ref{spectral clustering for different correlation}) exhibits. 
% Consider the sample size $n=200$, dimension $d=100$,  $\mu = (10,0,\cdots, 0)^{T}$  and $\bSigma = t\bB\bB^{T}+ \bI_d$ for some $t \in [0,1]$, where the rows of $\bB\in \mathbb{R}^{100 \times 3}$ are drawn from i.i.d. $\mathcal{N}(0,\bI_{3})$ and $t \in [0, 1]$ indicates the strength of correlation.  For each given $t$ with a step size $0.01$, we conduct the spectral clustering (Algorithm \ref{alg2}) on generated data $\{\bx_i\}_{i=1}^n$ with $K=2$ and $k=1$ and compute the misclassification rate. Figure \ref{spectral clustering for different correlation} depicts the misclassification rate of spectral clustering and the optimal rate $\Phi(-\sqrt{\text{SNR}})$ with respect to $t$,
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{Spectral_clustering_for_different_correlation_w_oprimal_rate.png}
    \caption{Spectral clustering for different correlation. For $t=0,0.01,0.02,\cdots,1$, generate data $\{\bx_i\}_{i=1}^n$ with sample size $n=200$, dimension $d=100$,  $\mu = (10,0,\cdots, 0)^{T}$  and $\bSigma = t\bB\bB^{T}+ \bI_d$ where $t$ indicates the strength of correlation. The rows of $\bB\in \mathbb{R}^{100 \times 3}$ are drawn from i.i.d. $\mathcal{N}(0,\bI_{3})$. For each given $t$, the spectral clustering (Algorithm \ref{alg2}) are conducted on $\{\bx_i\}_{i=1}^n$ with $K=2$ and $k=1$. The misclassification rate of spectral clustering and the optimal rate $\Phi(-\sqrt{\text{SNR}})$ are plotted with respect to $t$.}
    \label{spectral clustering for different correlation}
\end{figure}
Figure \ref{spectral clustering for different correlation} reveals the performance deterioration as $t$ increases due to the stretched covariance matrix. When $t$ increases, the SNR (blue points) remains high, but $\|\bSigma\|$ can be quite large, resulting in a small 
$ \text{S}=\frac{\|\bmu\|_{2}^{2}}{\|\bSigma\|_{2}}$.
Many computationally efficient algorithms, such as spectral clustering (e.g., \cite{abbe2022ellp,zhang2022leaveoneout}), can only  achieve a misclassification rate of $e^{-\Omega(\text{S})}$ instead of $e^{-\Omega(\text{SNR})}$. Since we always have $\text{S} \leq \text{SNR}$, the rate is not optimal, and will be quite poor when $S$ is significantly smaller than SNR, as Figure \ref{spectral clustering for different correlation} shows.
% \r{Q:  this is not what is going on.  Also show the performance of our method in this figure.}


To overcome the problem caused by high correlation, we focus on the case where the correlation is caused by latent factors and propose a clustering method named Factor-Adjusted Spectral Clustering (FASC).  Specifically, we consider the following standard clustering model with the data $\{\boldsymbol{x}_{i}\}_{i=1}^{n}$ from $\bx_{i}=\bmu_{y_{i}} + \be_{i}$, where $\{y_{i}\}_{i=1}^n$ are class labels, $\{\bmu_{j}\}_{j=1}^{K}$ are the  cluster centers, and $\be_{i}$ is independent from $y_{i}$. Previous works often focus  on the case that $\boldsymbol{e}_{i}$ has a nearly isotropic covariance matrix, yet  in reality the measurements are usually highly correlated.  A popular approach to model the dependence among high-dimensional covariates is the factor model, which has been widely used in economics and finance, psychology and data sciences \citep{bai2002determining, fama2015five, fan2020statistical}.  Following the work in the literature,  we assume that $\be_{i}$ is generated from the following factor model $\be_{i}=\bB \bff_{i} + \bepsilon_{i}$, where $\bB \in \mathbb{R}^{d \times r}$ is a factor loading matrix, $\bff_{i} \in \RR^{r}$ is a vector of  latent factors, $\bepsilon_{i} \in \RR^{d}$ is the noise that independent from all other quantities.  
% \r{Q: too simple the model?  Accomodate $\bSigma_{\epsilon} $ with a bounded operator norm? Normality needed}.
The model is equivalent to $\bx_{i}=\bB \bff_{i}+\bu_{i}$ where $\bu_{i} =  \bmu_{y_{i}} + \bepsilon_{i}$ is the idiosyncratic components that are uncorrelated with $\bff_{i}$.  

Leveraging this factor structure, we propose a method named Factor-Adjusted Spectral Clustering (FASC) (\prettyref{algo:1}). Our approach is to first learn the latent factor components $\{\bB\bff_{i}\}$ by using principal component analysis, estimate the idiosyncratic components $\{\bu_{i}\}$ by subtracting the latent factors, and then conduct spectral clustering (Algorithm \ref{alg2}) on the estimated $\{\hat{\bu}_{i}\}_{i=1}^{n}$. By subtracting the latent factor components, we not only decorrelate the dependence among variables but also reduce the noise with a smaller covariance matrix, therefore achieving the optimal misclassification rate $e^{-\Omega(\text{SNR})}$ with near linear sample complexity $n=\tilde{\Omega}(d)$, which will be rigorously shown by Theorem \ref{main_thm}. Simulation studies and real data analysis are also provided, justifying the applicability of FASC.



%In the rest of this paper, we will first introduce the basic settings and preliminaries. Then we will introduce our methodology in detail. After that we will give our theoretical results, which certify that our method, FASC, has both the optimal sample complexity $n = \tilde{\Omega}(d)$ and the optimal misclassification rate $e^{-\Omega(\text{SNR})}$. We will give some numerical evidence to justify our theory and compare FASC with vanilla spectral clustering. Experiments on real data are also provided, showing the applicability of FASC.




\subsection{Related work}
\paragraph{Classification and clustering of mixture models}




The exploration of classification and clustering in the context of mixture models, particularly Gaussian mixture models (GMM), can date back to the seminal work \cite{fisher1936use}. Fisher's work elucidated that, the optimal misclassification rate for GMM is $e^{-\Omega(\text{SNR})}$, even when the means and covariance matrix are known. Subsequently, when the means and covariance matrix are unknown, \cite{Friedman1989RegularizedDA} showed the necessity for the sample size $n$ to exceed the dimension $d$ to achieve the Bayes optimal rate, even when the true labels are observed. In scenarios where $d$ surpasses $n$,  \cite{bickel2004some} expounded upon the superiority of the "independence" rule over the Fisher linear discriminant rule. Additionally, \cite{fan2008high} contributed to this body of knowledge by shedding light on the challenges posed by noise accumulation in high-dimensional feature spaces when employing all features for classification. In response to this, they introduced FAIR, which selects a subset of critical features for high-dimensional classification, yielding commendable performance.






% The study for classification and clustering of mixure models, especially Gaussian mixture models (GMM), can date back to \cite{fisher1936use}, which shows the optimal misclassification rate for GMM is $e^{-\Omega(\text{SNR})}$, even when the means and covariance matrix are known. When the means and covariance matrix are unknown, \cite{Friedman1989RegularizedDA} showed the necessity for sample size $n=\Omega(d)$ to achieve Bayes optimal rate, even when the true labels are observed. For the regime that $d \geq n$, \cite{bickel2004some} showed the "independence" rule greatly outperforms
% the Fisher linear discriminant rule. \cite{fan2008high} further demonstrated that classification using all the features can be poor due to noise accumulation in high-dimensional feature space. They therefore proposed FAIR, which selects a subset of important features for
% high-dimensional classification, and achieves good performance.  

% Even when the labels are observed, sample size $n=\Omega(d)$ is needed for achieving Bayes optimal rate \citep{Friedman1989RegularizedDA}, since estimating the covariance matrix will need such sample size. Therefore,  $n=\Omega(d)$ serves as an optimal sample complexity for this kind of clustering problems. \shange{optimal sample complexity? change to linear}

Unsupervised clustering problems are relatively less understood until recent developments. When the covariance matrix is known to be spherical, i.e., $\bSigma=\bI_{d}$, many methods have been proposed, including iterative methods \citep{lu2016statistical,jana2023adversarially,jana2024general}, spectral methods \citep{VEMPALA2004841,jin2017phase,Ndaoud2018SharpOR,loffler2021optimality}, EM algorithms \citep{balakrishnan2017statistical,pmlr-v65-daskalakis17b,kwon2020algorithm} and etc. Of particular relevance to our investigation, \cite{loffler2021optimality} demonstrated that vanilla spectral clustering achieves the optimal misclassification rate of $e^{-\Omega(\text{SNR})}$ with a linear sample complexity $n= \Omega (d)$ in the context of Gaussian mixture models with spherical covariance matrices. In scenarios where the covariance matrix $\bSigma$ is unknown, \cite{abbe2022ellp, zhang2022leaveoneout} showed spectral clustering achieves the misclassification rate $e^{-\Omega(\text{S})}$ with a (nearly) linear sample size $n = \tilde{\Omega}(d)$ for sub-Gaussian mixture models. However, these rates fall considerably short of optimality when $\text{S} \ll \text{SNR}$. Other than spectral clustering, various other works \citep{Brubaker2008IsotropicPA, Ge2015LearningMO, 10.1145/3519935.3519953} have sought to devise clustering algorithms applicable to general GMM, striving to achieve the optimal rate of $e^{-\Omega(\text{SNR})}$. However, these methods necessitate a sample complexity of $n = \tilde{\Omega}(d^{2})$ or even larger. \cite{davis2021clustering} conjecture that there does not exist a computationally efficient algorithm for general GMM which achieves optimal misclassification rate with a linear sample complexity. In their work, they introduce an efficient spectral algorithm that attains the optimal rate but requires a quadratic sample size. Compared to prior arts, our research leverages factor structures for sub-Gaussian mixture models to propose a computationally efficient algorithm that concurrently achieves the optimal rate and linear sample complexity.

% Unsupervised clustering problems are relatively less understood until recent. When the covariance matrix is known to be spherical, i.e., $\bSigma=\bI_{d}$, many methods are proposed, including spectral methods \citep{VEMPALA2004841,jin2017phase,Ndaoud2018SharpOR,loffler2021optimality}, EM algorithms \citep{balakrishnan2017statistical,pmlr-v65-daskalakis17b,kwon2020algorithm} and etc. Most relevant to our work, \cite{loffler2021optimality} showed vanilla spectral clustering achieves the optimal misclassification rate $e^{-\Omega(\text{SNR})}$, with a linear sample complexity $n= \Omega (d)$, for GMM with spherical covariance matrix. However, when the covariance matrix $\bSigma$ is unknown, spectral clustering can only achieve a misclassification rate of $e^{-\Omega(\text{S})}$ with the (near) linear sample size $n = \tilde{\Omega}(d)$ \citep{abbe2022ellp,zhang2022leaveoneout} for sub-Gaussian mixture models. These rates are far from optimal when $\text{S} \ll \text{SNR}$. Other than spectral clustering, a number of works \citep{Brubaker2008IsotropicPA,Ge2015LearningMO,10.1145/3519935.3519953} developed clustering algorithms for general GMM that achieve the optimal rate $e^{-\Omega(\text{SNR})}$, but a sample complexity of $n = \tilde{\Omega}(d^{2})$ or larger is needed. \cite{davis2021clustering} conjecture that there does not exist a computationally efficient algorithm for general GMM which achieves optimal misclassification rate with a linear sample complexity. They develop an efficient spectral algorithm that attains the optimal rate but requires a quadratic sample size. Compared to prior arts, our work leverages factor structures for sub-Gaussian mixture models to propose an computationally efficient algorithm that achieves the optimal rate and linear sample complexity at the same time.


% \r{Q: writing is not smooth and the literature review is not good enough.  Work by Bickel and Levina and FAIR in Fan and Fan are very relevant}

\paragraph{Factor models}
Factor models \citep{lawley1971factor}, have emerged as a prominent and effective approach for characterizing dependence, finding widespread utility in various domains, including genomics \citep{bmc2006}, neuroscience \citep{pournara2007factor}, economics \citep{Bai2003InferentialTF, bai2002determining}, finance \citep{fama2015five}, and the social sciences \citep{zhou2015measuring}. Factor-adjusted strategies have found extensive application in numerous statistical analyses, such as model selection \citep{FAN202071}, multiple testing \citep{doi:10.1080/01621459.2018.1527700}, nonparametric regression utilizing neural networks \citep{fan2023factor}, and more.

Various methods have been devised for estimating factor models, with principal components analysis (PCA) \citep{RePEc:bes:jnlasa:v:97:y:2002:m:december:p:1167-1179} emerging as the most prevalent. Multiple variants of PCA have also been introduced for factor estimation, including projected PCA \citep{10.1214/15-AOS1364}, diversified projection \citep{Fan2019LearningLF}, and others. Extensive exploration of PCA's asymptotic behavior under high-dimensional scenarios has been conducted in the literature, including \cite{johnstone2009consistency}, \cite{fan2013large}, \cite{shen2016statistics}, \cite{fan2015asymptotics}, and more. Another strand of research has been dedicated to the estimation of the number of factors, with notable studies conducted by \cite{bai2002determining}, \cite{luo2009contour}, \cite{hallin2007determining}, \cite{lam2012factor}, and \cite{ahn2013eigenvalue}, among others. For a comprehensive overview of recent advancements in high-dimensional factor models and their applications to statistics, refer to \cite{fan2021robust}.















% Factor models \citep{lawley1971factor} have become one of the most popular and effective tools for characterizing dependence, with wide applications in genomics \citep{bmc2006}, neuroscience \citep{pournara2007factor}, economics \citep{Bai2003InferentialTF,bai2002determining}, finance \citep{fama2015five} and social sciences \citep{zhou2015measuring}. Factor adjusted strategies are widely adopted in many statistical analyses, e.g., model selection \citep{FAN202071}, multiple testing \citep{doi:10.1080/01621459.2018.1527700}, nonparametric regression by neural networks \citep{fan2023factor} and etc. 

% Various methods are proposed for estimating the factor model, among which principal components analysis \citep{RePEc:bes:jnlasa:v:97:y:2002:m:december:p:1167-1179} is most popular. Many variants of PCA are also deployed for factor estimation, including projected PCA \citep{10.1214/15-AOS1364}, diversified projection \citep{Fan2019LearningLF} and etc. Asymptotic behavior of PCA under the high dimensional regime has been well studied in literature, such as \cite{johnstone2009consistency}, \cite{fan2013large}, \cite{shen2016statistics}, \cite{fan2015asymptotics} and etc. Another line of work contributed to the estimation of the number of factors, including \cite{bai2002determining}, \cite{luo2009contour}, \cite{hallin2007determining}, \cite{lam2012factor} and \cite{ahn2013eigenvalue} among others. For a selective overview of recent advances in high-dimensional factor models and their applications to statistics, see \cite{fan2021robust}.

% A very common way to characterize the stylized feature that in high dimension, covariates are often highly correlated, is to assume there exist some unobserved latent factors that correlate with the observed outcome
% \citep{lawley1971factor}. Factor models have become one of the most popular and effective tools in multivariate analysis, with wide applications in genomics \citep{bmc2006}, financial economics \citep{Bai2003InferentialTF,bai2002determining}, etc.  Some recent works consider factor adjusted strategy in different statistical analyses, e.g., model selection \citep{FAN202071}, multiple testing \citep{doi:10.1080/01621459.2018.1527700}, etc. 

% For the estimation of the factor model, principal components analysis is of the highest importance \citep{RePEc:bes:jnlasa:v:97:y:2002:m:december:p:1167-1179}. There are also many variants of PCA for factor estimation, including projected PCA \citep{10.1214/15-AOS1364}, diversified projection \citep{Fan2019LearningLF} and etc. 


% \shange{need more related work about factor model?}





% Consider the following standard clustering model: data $\{\boldsymbol{x}_{i}\}_{i=1}^{n}$ satisfies
% \begin{equation} 
%     \boldsymbol{x}_{i}=\boldsymbol{\mu}_{y_{i}} + \boldsymbol{e}_{i},
% \end{equation}
% where $y_{i}$ is the true label, $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ is the set of true cluster centers, and $\boldsymbol{e}_{i}$ is independent from $y_{i}$. Previous work often considers the case that $\boldsymbol{e}_{i}$ has a nearly spherical covariance matrix. However, in reality, the covariates are usually highly correlated, thus the covariance is often stretched. To handle this case, in this paper we assume that $\boldsymbol{e}_{i}$ is generated from the following factor model:
% \begin{equation} 
%     \boldsymbol{e}_{i}=B\boldsymbol{f}_{i} + \boldsymbol{\epsilon}_{i}, 
% \end{equation}
% where $B \in \mathbb{R}^{d \times r}$ is the fixed factor loading matrix, $\boldsymbol{f}_{i} \sim \mathcal{N}(0,I_{r})$ is the latent factor, $\boldsymbol{\epsilon}_{i} \sim \mathcal{N}(0,\sigma^{2}I_{d})$ is the noise that independent from all other quantities. We can see that in this case, $\boldsymbol{e}_{i} \sim \mathcal{N}(0,BB^{T} + \sigma^{2} I_{d})$. Another equivalent way of stating this model is to introduce another quantity
% \begin{equation} 
%     \boldsymbol{u}_{i}=\boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i},
% \end{equation}
% and rewrite the model as a factor model
% \begin{equation} \label{factor_model}
% \boldsymbol{x}_{i}=B\boldsymbol{f}_{i}+\boldsymbol{u}_{i},
% \end{equation}
% where $\boldsymbol{u}_{i}$ can be view as the idiosyncratic component that are uncorrelated with $\boldsymbol{f}_{i}$, and all the information of clustering is on $\boldsymbol{u}_{i}$.  

% Leveraging this factor structure, we propose a strategy named Factor-Adjusted Spectral Clustering (FASC). Our strategy of conducting clustering to this factor clustering model (\ref{factor_model}) is to first recover the idiosyncratic components $u_{i}$ in model (\ref{factor_model}) for the unlabeled data $\{\boldsymbol{x}_{i}\}_{i=1}^{n}$. Then by identifying $\boldsymbol{u}_{i}$, we transform the problem from clustering in $\{\boldsymbol{x}_{i}\}_{i=1}^{n}$, which has stretched covariance (large $\text{S}$), to data $\{\boldsymbol{u}_{i}\}_{i=1}^{n}$ with nearly spherical covariance (small $\text{S}$). Therefore, we can then conduct methods such as spectral clustering on $\{\boldsymbol{u}_{i}\}_{i=1}^{n}$ to achieve the optimal misclassification rate with optimal sample complexity $\tilde{\Omega}(d)$.

% In the rest of this paper, we will first introduce the basic settings and preliminaries. Then we will introduce our methodology in detail. After that we will give our theoretical results, which certifies our method, FASC, have both optimal sample complexity and optimal misclassification rate. In order to prove our main results, we introduce a new "cross-validation" type of spectral clustering algorithm together with a simpler proof strategy then the standard spectral clustering literature. Finally we will give some numerical evidence to justify our theory, and compare FASC with vanilla spectral clustering.







==> texfiles/old/main_results.tex <==
\section{Theoretical results}
In this section, we will analyze the FASC algorithm (\prettyref{algo:1}) and provide theoretical guarantees under three different spectral conditions of the factor loading $\bB$. Our results require basic regularity assumptions on our model. The first assumption is that the size of each cluster can not be too small. Also, we need that the true cluster centers should really lie on a $k$ dimensional subspace, and two centers can not be too close. These regularity assumptions are standard in related works (e.g., \cite{abbe2022ellp,zhang2022leaveoneout,loffler2021optimality}). 
% To be specific, recall that in our model (\ref{factor_cluster}), we have $\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K.$ Here we further require the following holds:
To be specific, we make the following assumptions to our model:
\begin{myassumption}[Regularity]\label{regularity}
1. There exists a constant $c$ such that $p_{j}\geq c$, for $j=1,\cdots, K.$\\
2. $\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]$ is rank $k$ and there exist constants $C_3, c_3>0$ such that $C_3 \geq \lambda_{1} (\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) \geq \lambda_{k} (\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) \geq c_3$. \\
3. There exist constants $c_4,c_5>0$ such that $c_5 \geq \max_{i\neq j}\|(\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j})\|\geq \min_{i\neq j}\|(\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j})\| \geq c_4$.
\end{myassumption}

\subsection{Factor model with pervasiveness condition}
In this subsection, we will assume the factor loading matrix $\bB$ has the following “pervasiveness" condition. This condition is common in the related literature (see \cite{fan2021robust} for discussions), since it facilitates the learning of the factors.

\begin{myassumption} \label{pervasiveness}[Pervasiveness]
there exist constants $c,C$, such that $c\sqrt{d} \leq \sigma_{\min}(\bB) \leq\sigma_{\max}(\bB) \leq C\sqrt{d}$.  \end{myassumption}
\paragraph{Approximate perpendicularity}
Besides the above assumptions, we further need a critical assumption that the span of $\{\bmu_{j}\}_{j=1}^{K}$ is approximately perpendicular to the column span of $\bB$. 
% Recall that in our section of signal-to-noise ratio, we mentioned that when $\{\bmu_{j}\}_{j=1}^{K}$ is approximately perpendicular to the column span of $\bB$, SNR is in fact close to $\overline{\text{SNR}}$, and we can achieve the optimal misclassification rate $e^{-\Omega(\overline{\text{SNR}})}$ in term of $\overline{\text{SNR}}$. 
Notice that this "perpendicular" assumption is necessary for our Algorithm \ref{alg1} to work well, as illustrated by the following example: let $\bff_i \sim \cN(0,\bI_r)$ and $\bepsilon_i \sim \cN(0,\sigma^2 \bI_d)$, taking $\sigma^{2}=1,$
$\bB = (100,0)^{T}$, $\bmu_{1}=(3,0)^{T}$, $\bmu_{2}=(-3,0)^{T}$, $p_1=p_2=1/2$. Then $\bx_{i} \sim  
\frac{1}{2}\mathcal{N}((3,0)^{T}, \bSigma) + \frac{1}{2}\mathcal{N}((-3,0)^{T}, \bSigma)$
 where $\bSigma = \begin{pmatrix}
 10001 & 0 \\
 0 & 1 
 \end{pmatrix}$.
Under this model, $\hat{\bV}_{r}$ in (\ref{hat_V_r}) will approximately be $(1,0)^{T}$, since this is the column space of $\bB$. Then when computing $\hat{\bu}_{i}$ as in (\ref{hat_u_i}), we get
 \begin{align*}
    \hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i}\\
    & \approx \begin{pmatrix}
 0 & 0 \\
 0 & 1 
 \end{pmatrix} \bx_{i},
 \end{align*}
 which means $\hat{\bu}_{i}$ will only be a function of the second coordinate of $ \bx_{i}$. However, in this model, the true cluster centers lie in $span\{(1,0)^{T}\}$.
 % Therefore when applying Algorithm \ref{alg1}, two $\bx_i$s that are in different clusters (their first coordinates have much difference), may have $\hat{\bu}_i$s that are close to each other.  
 Therefore when applying Algorithm \ref{alg1}, after the first phase, the computed $\hat{\bu}_{i}$ loses the information of clusters (which are on the first coordinate).
% \shange{do not write strict perp in assumption, use language to discribe. By Davis kahan, it should be small?}
%  \begin{assumption}[Strict perpendicularity]\label{strict_perpendicularity}
% Let $\Sigma := \mathbb{E}[\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{T}]$, and $V_{r}$ be its top $r$ eigenvectors. We assume the following holds:
% \begin{align} 
%     &(I-V_{r}V_{r}^{T})B=0 \notag \\
%     &(I-V_{r}V_{r}^{T})\boldsymbol{\mu}_{j}=\boldsymbol{\mu}_{j}, \quad \forall j \in [K].
% \end{align}
% \end{assumption}
% This assumption indicates that when we calculate the $\hat{\boldsymbol{u}}_{i}$ in the first phase, the clustering structure is preserved. However, this strict perpendicularity is in fact too restricted. 
Motivated by this observation, for our Algorithm \ref{alg1} to achieve the optimal misclassification rate, we will require "approximate perpendicularity" to hold, as the following:

\shange{this $\bV$ here is not the same as $\bV_r$. It's confusing! change the notation. Also, put the definition of $\bV_r$ in some obvious places}


\begin{myassumption}[Approximate perpendicularity]\label{approximate_perpendicularity}
Let the eigen-decomposition of $\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]$ be 
$\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]=\bM\bV\bM^{T}$. This decomposition indicates that the subspace spanned by $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ can be represented by an matrix $\bM \in \mathbb{R}^{d \times k}$ with orthogonal columns. Similarly, let the eigen-decomposition of $\bB\bB^{T}$ be $\bB\bB^{T}=\bU\bLambda \bU^{T}$, which indicates that the column space of $\bB$ can be represented by an matrix $\bU \in \mathbb{R}^{d \times r}$ with orthogonal columns. Then we assume the following holds: 
 \begin{equation*} 
     \|\bU^{T}\bM\| \leq \min \{\sqrt{d \sigma^2}, \frac{c_3}{9C_3}\},
 \end{equation*}
where $c_3,C_3$ first appear in Assumption \ref{regularity}.
\end{myassumption}

% \r{Q: This may not needed if the goal is to show that misclassification rates using $\bu_i$ and $\hat{\bu}_i$ are similar.}

% \begin{remark}
%     ss
% \end{remark}

\noindent \textbf{Remark 1}: Assumption \ref{approximate_perpendicularity}  indicates the following results which is important in proving the guarantee for Algorithm \ref{alg1}:
% that after the first phase of FASC, the structure of clustering is preserved. To be specific, 
let $\bSigma := \mathbb{E}[\bx_{i}\bx_{i}^{T}]$, and $\bV_{r}$ be its top $r$ eigenvectors, we have
\begin{align} \label{strict_perpendicularity}
    &(\bI-\bV_{r}\bV_{r}^{T})\bB\approx0 \notag \\
    &\|(\bI-\bV_{r}\bV_{r}^{T})(\bmu_i - \bmu_j)\|\approx \|\bmu_i - \bmu_j\|, \quad \forall i,j \in [K].
\end{align}
See Lemma \ref{approx_per_lemma} for details.\\

We claim that Assumption \ref{approximate_perpendicularity} is natural and easy to hold in the high dimensional setting, since a randomly uniformly chosen unit vector will be nearly perpendicular to a given vector with a very high probability, as the following lemma shows:
\begin{lemma} \label{justify_approx_perp_lemma}
Let $\bB \in \RR^{d\times r}$ be a fixed matrix, $\bU \in \RR^{d\times r}$ be its left singular vectors. Consider the Grassmannian manifold $G_{d,k}$ that consists of all $k$-dimensional subspaces of $\mathbb{R}^{d}$. Let $\bM \sim \text{Unif} (G_{d,k})$ (see \cite{vershynin2018high} for detailed discussion of the measure on Grassmannian manifold), which means $\bM$ represents a uniformly randomly chosen $k$-dimensional subspace of $\mathbb{R}^{d}$. Suppose $d \geq c_1 (\log n \vee \frac{1}{\sigma^2})$ for some sufficiently large constant $c_1$. Then for sufficiently large $n$ with probability $1-n^{-9}$, 
 \begin{equation*} 
     \|\bU^{T}\bM\| \leq \min \{\sqrt{d \sigma^2}, \frac{c_3}{9C_3}\}.
 \end{equation*}
\end{lemma}

The proof of Lemma \ref{justify_approx_perp_lemma} is provided in Appendix \ref{justify_approx_perp_lemma_proof}. By this lemma, we show that when $d \geq \Omega (\log n)$, if we choose $\bM$ uniformly at random, the Assumption \ref{approximate_perpendicularity} holds with high probability. With the above assumptions, we are now able to state the main theoretical result.
\begin{theorem}\label{main_thm}
Consider the model (\ref{factor_cluster}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg1}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumptions \ref{regularity}, \ref{pervasiveness} and \ref{approximate_perpendicularity} hold, and $d \leq O ( \frac{n}{(\log n)^{2}})$, then there exist constants $C$ and $c$ such that the following hold: \\
1. If $\overline{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \overline{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \overline{\text{SNR}})}$ for sufficiently large $n$.
\end{theorem}


% \r{Q:  The result is somewhat thin.  Do you assume SubGaussian or Gaussian data?}

% \shange{emphasize again, if do not use factor adjustment, what is the result?}
Theorem \ref{main_thm} shows that Algorithm \ref{alg1} achieves the optimal misclassification rate and near linear sample complexity at the same time. For the misclassification rate, by Theorem \ref{main_thm} it is bounded by $\exp{(-c \cdot \overline{\text{SNR}})}$. Recall that vanilla spectral clustering (without factor-adjustment) can only achieve a misclassification rate $\exp{(- \Omega (\text{S}))}$ (e.g., \cite{abbe2022ellp,zhang2022leaveoneout}), which can be much worse than our result (recall Figure \ref{SNR vs barSNR vs S} for a numerical comparison of $\overline{\text{SNR}}$ and S). The performance difference between FASC and spectral clustering will be further demonstrated by simulation studies. It is worth noting that our bound is optimal in $\text{SNR}$, since $\text{SNR} \leq \overline{\text{SNR}}$. For the sample size of FASC, $d \leq O (\frac{n}{(\log n)^{2}})$ is required for Theorem \ref{main_thm} to hold, which means the sample complexity required is $n \geq \tilde{\Omega} (d)$, which is linear in $d$ up to log factors. 
% If further considering when Assumption \ref{approximate_perpendicularity}
% is reasonable (Lemma \ref{justify_approx_perp_lemma}), then FASC (Algorithm \ref{alg1}) is appealing under the scenario that $\Omega(\log n) \leq d \leq O( n/(\log n)^{2})$.
In addition, when $\Omega(\log n) \leq d \leq O( n/(\log n)^{2})$, then Lemma \ref{justify_approx_perp_lemma} shows that Assumption \ref{approximate_perpendicularity} holds in many reasonable scenarios. As a result FASC (Algorithm \ref{alg1}) will achieve the desired bound of misclassification rate. However, similar gurantees for spectral clustering  does not exist.


% \paragraph{Downstream Task Learning}
% We upper bound the prediction error of Algorithm \ref{mle+erm} as follows.

\subsubsection{Proof sketch}
In this subsection, we briefly characterize the intuition of proving Theorem \ref{main_thm}. For simplicity, we assume Assumption \ref{regularity} and (\ref{strict_perpendicularity}) hold "strictly". The detailed proof under Assumption \ref{approximate_perpendicularity} will be presented in the Appendix. Our proof strategy has two phases: in the first phase, we show that our estimator $\hat{\bu}_{i}$ can be written as $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$,
where $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise; in the second phase, we apply the result for spectral clustering with small sub-Gaussian noise.
\paragraph{First phase: decomposing the estimator}
For the first phase, 
\begin{align*}
    \hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i}  \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) (\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})  \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{y_{i}} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &:= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{align*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}$. Let $\bDelta:=\bV_{r}\bV_{r}^{T} -\hat{\bV}_{r}\hat{\bV}_{r}^{T}$, by matrix perturbation theory, we have $\|\bDelta\| \leq O (\sqrt{\frac{\log n}{n}})$ with a high probability (Proposition \ref{matrix_perturbation_proposition}). Then we have for $j_{1} \neq j_{2}$, 
\begin{align*}
   \|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\| &= \| (I-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \|  \\
   & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \\
   &= \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \quad (\text{By (\ref{strict_perpendicularity})}) \\
   & \geq \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta\| \| \boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| \notag \\
   & \geq \frac{1}{2} \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\|.
\end{align*}
 For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
    \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}  \\
    &= 0 + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \quad (\text{By (\ref{strict_perpendicularity})}) 
\end{align*}
Notice that $\bff_{i} \sim \text{SG}_{r} (c_1^2) $, $\bepsilon_{i} \sim \text{SG}_{d} (\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
    \|\bDelta \bB\|^{2} + \sigma^{2} & \leq \|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
    & \leq O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \quad (\text{By proposition \ref{matrix_perturbation_proposition}}) \notag \\
    & \leq  O(\frac{d \log n}{n}) + \sigma^{2} \quad (\text{By Assumption \ref{pervasiveness}}) \notag \\
    & \leq O(\frac{1 }{\log n}) + \sigma^{2}  \quad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{2}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq O (\frac{1}{\log n})$, we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\sigma^{2})$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (O (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$. Which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise.

\paragraph{Second phase: general results for spectral clustering}
For the second phase, we apply the general results for spectral clustering. Suppose we now have data from the following model: 
\begin{align} \label{spectral_clustering_model}
    &\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
    &\bx_{i} = \btheta_{y_{i}} + \bepsilon_{i},
\end{align}
where $y_{i}$ is the true label, $\{\btheta_{j}\}_{j=1}^{K}$ is the set of true clustering centers, and $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$ is independent from all other quantities. The signal-to-noise ratio in this model is defined as 
\begin{equation*}
    \widetilde{\text{SNR}} := \frac{\min_{i\neq j}\|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\|^{2}}{\sigma^2}.
\end{equation*}
We have the following theoretical guarantee for spectral clustering (Algorithm \ref{alg2}), which is a direct consequence of Corollary 3.1 in \cite{zhang2022leaveoneout} with a slight modification (here we use $(1+\epsilon)$-approximate $K$-means).
% (Theorem 3.1 in \cite{abbe2022ellp}): 
\begin{lemma}\label{spectral_clustering_lemma}
Consider the model defined in (\ref{spectral_clustering_model}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg2}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumption \ref{regularity} holds, and $d \leq O (n)$, then there exist constant $C$ and $c$ such that the following hold: \\
1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$.
\end{lemma}
% See the appendix for the proof of Lemma \ref{spectral_clustering_lemma}. Notice that similar results are already given in many spectral clustering literature, but their proof is usually complicated, due to the fact that $\hat{V}$ is not independent with $\boldsymbol{x}_{i}$. Here we resolve this problem by using the "cross-validation" type algorithm, thus our analysis is much simpler.
Applying Lemma \ref{spectral_clustering_lemma} on $\{\hat{\boldsymbol{u}}_{i}\}_{i=1}^{n}$ will finish the proof for Theorem \ref{main_thm}.  

\noindent \textbf{Remark}: Notice that the proofs for Lemma \ref{spectral_clustering_lemma} or similar results are very complicated (see \cite{abbe2022ellp,zhang2022leaveoneout}), due to the fact that $\hat{\bV}$ is not independent with $\bx_{i}$. We can resolve this problem by splitting the data to facilitate an easier analysis of spectral clustering algorithm. See Appendix \ref{cv} for further details.

\subsection{Factor model with weak factors}
In this subsection, we will explore the theoretical properties of FASC without "pervasiveness" condition. An alternative setting is called ``weak factor":
\begin{myassumption} \label{weak_factor1}
There exist constants $C$, such that $3\|\bSigma_u\| \leq \sigma_{\min}^{2}(\bB) \leq \sigma_{\max}^{2}(\bB) \leq C$.
\end{myassumption}
Under this scenario, we will need a slightly stronger "approximate perpendicularity" to hold for FASC to perform well.
\begin{myassumption}[Approximate perpendicularity]\label{approximate_perpendicularity2}
Let the eigen-decomposition of $\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]$ be 
$\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]=\bM\bV\bM^{T}$, the eigen-decomposition of $\bB\bB^{T}$ be $\bB\bB^{T}=\bU\bLambda \bU^{T}$. We assume the following holds:
 \begin{equation*} 
     \|\bU^{T}\bM\| \leq \min \{\sigma, \frac{c_3}{9C_3}\}.
 \end{equation*}
\end{myassumption}
Under the ``weak factor" scenario, theoretical guarantees for FASC can also be provided.
\begin{theorem}\label{thm2}
Consider the model (\ref{factor_cluster}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg1}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumptions \ref{regularity}, \ref{weak_factor1} and \ref{approximate_perpendicularity2} hold, and $d \leq O ( \frac{n}{(\log n)^{3}})$, then there exist constants $C$ and $c$ such that the following hold: \\
1. If $\overline{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \overline{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \overline{\text{SNR}})}$ for sufficiently large $n$.
\end{theorem}
Theorem \ref{thm2} shows that FASC still achieves the optimal misclassification rate in the aforementioned weak factor case with the linear sample complexity. The only difference between Theorem \ref{main_thm} and \ref{thm2} is 
the necessity of a slightly stronger "approximate perpendicularity" to ensure the clustering structure is correctly specified, under the "weak factor" scenario.

Another possible scenario is that the eigen gap between the factor component and $\bu_i$ is small compared to the scale of $\bB$, under which the learning of the factor model is even harder. 
\begin{myassumption} \label{weak_factor2}
There exist constants $C$, such that $3\|\bSigma_u\| \leq \sigma_{\min}^{2}(\bB) \leq \sigma_{\max}^{2}(\bB) \leq C d$.
\end{myassumption}
Under this scenario, an even stronger perpendicularity assumption is needed to ensure FASC achieves the optimal misclassification rate.
\begin{myassumption}[Approximate perpendicularity]\label{approximate_perpendicularity3}
Let the eigen-decomposition of $\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]$ be $\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]=\bM\bV\bM^{T}$, the eigen-decomposition of $\bB\bB^{T}$ be $\bB\bB^{T}=\bU\bLambda \bU^{T}$. We assume the following holds:
 \begin{equation*} 
     \|\bU^{T}\bM\| \leq \min \{\frac{\sigma}{\sqrt{d}}, \frac{c_3}{9C_3}\}.
 \end{equation*}
\end{myassumption}

\begin{theorem}\label{thm3}
Consider the model (\ref{factor_cluster}) with $\bepsilon_i \sim \cN (0,\sigma^2 \bI_d)$.  Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg1}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumptions \ref{regularity}, \ref{weak_factor2} and \ref{approximate_perpendicularity3} hold, and $d^3 \leq O ( \frac{n}{(\log n)^{2}})$, then there exist constants $C$ and $c$ such that the following hold: \\
1. If $\overline{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \overline{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \overline{\text{SNR}})}$ for sufficiently large $n$.
\end{theorem}
Theorem \ref{thm3} shows that under this scenario, when a strong version of "approximate perpendicularity" (Assumption \ref{approximate_perpendicularity3}) holds, FASC can still achieve the optimal misclassification rate. However, the sample complexity needed is $n=\tilde{\Omega} (d^3)$, which is much worse than the counterpart in Theorem \ref{main_thm} and \ref{thm2}.

==> texfiles/old/method.tex <==
\section{Methodology}
If $\bu_{i}$ is observable, instead of applying spectral clustering on $\bx_{i}$, we can directly apply spectral clustering on $\bu_{i}$. Notice that applying spectral clustering on $\bu_{i}$ rather than $\bx_i$ is beneficial. The guarantee of the spectral clustering algorithm improves when the quantity ``S" gets larger. However the quantity ``S" corresponds to $\bu_{i}$ is $\overline{\text{SNR}}$, which is much larger than the counter part to $\bx_i$, since the covariance of $\bu_i$ does not have the spiked component induced by $\bB \boldsymbol f_i$. Motivated by this observation, the general procedure for FASC (Algorithm \ref{algo:1}) will be the following: we will first estimate $\bu_{i}$ with $\hat{\bu_i}$ using PCA. Then we will apply spectral clustering on the estimated $\{\hat{\bu}_i\}_{i=1}^{n}$.

% If $\bu_{i}$ is observable, instead of applying spectral clustering on $\bx_{i}$, we can directly apply spectral clustering on $\bu_{i}$. Notice that spectral clustering is a S-based \shange{S-based?} algorithm, which performs better \shange{say something exact} when S gets larger. The quantity ``S" corresponds to $\bu_{i}$ is $\overline{\text{SNR}}$ which is much larger than the counter part to $\bx_i$, since the covariance of $\bu_i$ does not have the spiked component induced by $\bB \bff_i$. Motivated by this observation, the general procedure for FASC (Algorithm \ref{algo:1}) is the following. We will first produce an estimate $\hat{\bu_i}$ of $\bu_{i}$ using PCA and then apply spectral clustering on the estimated $\{\hat{\bu}_i\}_{i=1}^{n}$.






\paragraph{First phase: estimating \texorpdfstring{$\bu_{i}$}{TEXT}}
Recall the model (\ref{factor_cluster}). The covariance matrix of $\bx_{i}$ is given as
\begin{equation*}
    \bSigma:=\text{cov}(\bx_{i}) = \text{cov} (\bB\bff_{i}+\bu_{i})=\bB\bB^{T} + \text{cov}(\bu_{i}) :=\bB \bB^{T} + \bSigma_u.
\end{equation*}
Notice that the operator norm of $\bSigma_u$ is small compared to the operator norm of $\bB\bB^{T}$ and hence $\text{cov}(\bx_{i})$ can be view as a low-rank matrix $\bB\bB^{T}$ plus a small matrix $\bSigma_u$. In this case, the column span of $\bB$ is close to the span of top $r$ eigenvectors of $\text{cov}(\bx_{i})$. Motivated by this observation, we compute the sample covariance matrix $\hat{\bSigma}:=\frac{1}{n}\bX^{T}\bX = \frac{1}{n}\sum_{i=1}^{n} \bx_{i} \bx_{i}^{T}$, and write its eigen-decomposition $\hat{\bSigma}=\sum_{j=1}^{d}\hat{\lambda}_{j}\hat{\bv}_{j}\hat{\bv}_{j}^{T}$,
% \begin{equation*}
% \hat{\Sigma}=\sum_{j=1}^{d}\hat{\lambda}_{j}\hat{\boldsymbol{v}}_{j}\hat{\boldsymbol{v}}_{j}^{T},
% \end{equation*}
where $\hat{\lambda}_{1} \geq \hat{\lambda}_{2} \geq \cdots \geq \hat{\lambda}_{d} \geq 0$. Then $\hat{\bV}_{r}:= (\hat{\bv}_{1},\cdots,\hat{\bv}_{r})$ is an estimation of the subspace spanned by $\bB$'s column. Therefore $\hat{\bV}_{r}\hat{\bV}_{r}^{T}\bx_{i}$, the projection of $\bx_{i}$ onto the subspace, is approximately $\bB\bff_{i}$, the factor component of $\bx_{i}$. 
% Therefore naturally we have the estimator of $\boldsymbol{u}_{i} = \boldsymbol{x}_{i} - B\boldsymbol{f}_{i}$ that is
The estimator of $\bu_{i}$ is then given by $\hat{\bu}_{i} = (\bI - \hat{\bV}_{r}\hat{\bV}_{r}^{T})\bx_{i}$.
% \begin{equation}\label{hat_u}
% \hat{\boldsymbol{u}}_{i} = (I - \hat{V}_{r}\hat{V}_{r}^{T})\boldsymbol{x}_{i}
% \end{equation}

\paragraph{Second phase: spectral clustering on \texorpdfstring{$\hat{\bu}_{i}$}{TEXT}}


After obtaining estimator $\hat{\bu}_{i}$, we can conduct spectral clustering (Algorithm \ref{alg2}) on $\{\hat{\bu}_{i}\}_{i=1}^{n}$ to get the desired estimated labels. $\{\hat{y}_{i}\}_{i=1}^{n}$. 

% Let $\hat{U}:= (\hat{\boldsymbol{u}}_{1},\cdots,\hat{\boldsymbol{u}}_{n})^{T}$. Assume we already know the true cluster centers lie in a $k$ dimensional subspace. Suppose that in each cluster, the data points are strongly concentrated around the center. That is, $\hat{U} \approx (\boldsymbol{\theta}_{y_{1}},\cdots,\boldsymbol{\theta}_{y_{n}})^{T} = F\Theta$, where $\Theta = (\boldsymbol{\theta}_{1},\cdots,\boldsymbol{\theta}_{k})^{T}\in \mathbb{R}^{k \times d} $ represents the cluster centers;
% $F \in \mathbb{R}^{n \times k}$ is defined as $F_{ij}=1$ if and only if $y_{i}=j$, else $F_{ij}=0$, represents the true label of each data point. Then we can see that, the row space of $\Theta$ is the span of the cluster centers. Therefore, finding the $k$ dimensional subspace that the cluster centers lie in is equivalent to finding the top $k$ right singular vectors of $F \Theta$. 

% Motivated by this observation, the algorithm of spectral clustering can be stated as the following. We first consider the singular value decomposition of $\hat{U}$:
% \begin{equation*}
%     \hat{U} = \sum_{j=1}^{d} \hat{\sigma}_{j} \boldsymbol{\eta}_{j} \boldsymbol{\xi}_{j}^{T}
% \end{equation*}
% where $\hat{\sigma}_{1} \geq \hat{\sigma}_{2} \geq \cdots \geq \hat{\sigma}_{d} \geq0$ are the singular values of $\hat{U}$. We take $\hat{V}:=(\boldsymbol{\xi}_{1},\cdots,\boldsymbol{\xi}_{k})\in \mathbb{R}^{d \times k}$, then $\hat{V}$ is the desired projection matrix that approximately finds the $k$ dimensional subspace. Then we project the data points onto this $k$ dimensional subspace and conduct $K$-means algorithm to these projected data points to find the estimated labels. Notice that exact $K$-means is not computationally efficient, here we instead use $(1+\epsilon)$-approximate $K$-means where a linear-time algorithm exists for solving it  \citep{Kumar2004ASL}. That is, we get $\{\hat{y}_{i}\}_{i=1}^{n}$ and $\{\hat{\boldsymbol{\mu}}_{j}\}_{j=1}^{K}$ such that
% \begin{equation*}
%     \sum_{i=1}^n\|(\hat{U}\hat{V})_i-\hat{\boldsymbol{\mu}}_{\hat{y}_i}\|_2^2 \leq(1+\epsilon) \min _{\substack{\{\widetilde{\boldsymbol{\mu}}_j\}_{j=1}^K \subseteq \mathbb{R}^k \\\left\{\widetilde{y}_i\right\}_{i=1}^n \subseteq[K]}}\{\sum_{i=1}^n\|(\hat{U}\hat{V})_i-\widetilde{\boldsymbol{\mu}}_{\tilde{y}_i}\|_2^2\} .
% \end{equation*}
% $\{\hat{y}_{i}\}_{i=1}^{n}$ are our desired estimated labels.

% \noindent \textbf{Remark}: The procedure of estimating $\{\hat{y}_{i}\}_{i=1}^{n}$ we described in this subsection is slightly different from the actual algorithm we will use. We actually use a "cross-fitting" type of spectral clustering, which allows for easier theoretical analysis. We will discuss this in detail later.

\subsection{The Factor-Adjusted Spectral Clustering (FASC)} 
In this subsection, we will formally state Factor-Adjusted Spectral Clustering (FASC). For simplicity of theoretical analysis, the formal algorithm we used is slightly different from the previous section: we split the data into two halves. Then we use the second half of data to compute $\hat{\bV}_{r}$, and estimate the corresponding $\hat{\bu}_{i}$ in the first half using the $\hat{\bV}_{r}$ which comes from the second half. And vice versa. In the second phase, we apply spectral clustering on $\hat{\bu}_{i}$. The algorithm is stated as follows. For simplicity, we assume the number of data is $2n$.
\begin{algorithm}[H]
\caption{Factor-Adjusted Spectral Clustering (FASC)}\label{algo:1}
\begin{algorithmic}[1]
\State {\bf Input:} Dataset $\{\bx_i\}^{2n}_{i=1}$. The number of factors $r$,  the number of clusters $K$,  target dimension of embedding $k$.
\State Split the data $\{\bx_i\}^{2n}_{i=1}$ into two halves, and use the second half of data to compute $\hat{\bV}_{r}$: Let $\hat{\bSigma}:= \frac{1}{n}\sum_{i=n+1}^{2n} \bx_{i} \bx_{i}^{T}$. Then we write the eigen-decomposition of $\hat{\bSigma}$:
\begin{equation*}
\hat{\bSigma}=\sum_{j=1}^{d}\hat{\lambda}_{j}\hat{\bv}_{j}\hat{\bv}_{j}^{T},
\end{equation*}
where $\hat{\lambda}_{1} \geq \hat{\lambda}_{2} \geq \cdots \geq \hat{\lambda}_{d} \geq 0$. Let 
\begin{equation} \label{hat_V_r}
    \hat{\bV}_{r}:= (\hat{\bv}_{1},\cdots,\hat{\bv}_{r}) \in \mathbb{R}^{d \times r}.
\end{equation}
\State Compute $\hat{\bu}_{i}$ for $i=1,\cdots,n$:
\begin{equation} \label{hat_u_i}
\hat{\bu}_{i} = \bx_{i} - \hat{\bV}_{r}\hat{\bV}_{r}^{T}\bx_{i}, \quad i=1,\cdots,n.
\end{equation}

\State Compute 
\begin{equation*}
    \hat{\bV}:=(\bxi_{1},\cdots,\bxi_{k}),
\end{equation*}
where $\bxi_{1},\cdots,\bxi_{k}$ are the top $k$ right singular vectors of the data matrix $(\hat{\bu}_{1},\cdots,\hat{\bu}_{n})^{T} $.

\State Conduct $(1+\epsilon)$-approximate $K$-means on $\{\hat{\bV}^{T}\hat{\bu}_{i}\}_{i=1}^{n}$, getting $\{\hat{y}_{i}\}_{i=1}^{n}$ and $\{\hat{\bmu}_{j}\}_{j=1}^{K}$ such that:
\begin{equation*}
    \sum_{i=1}^n\|\hat{\bV}^{T}\hat{\bu}_{i}-\hat{\bmu}_{\hat{y}_i}\|_2^2 \leq(1+\epsilon) \min _{\substack{\{\widetilde{\bmu}_j\}_{j=1}^K \subseteq \mathbb{R}^k \\\left\{\widetilde{y}_i\right\}_{i=1}^n \subseteq[K]}}\{\sum_{i=1}^n\|\hat{\bV}^{T}\hat{\bu}_{i}-\widetilde{\bmu}_{\tilde{y}_i}\|_2^2\} .
\end{equation*}


\State {\bf Output:} $\{\hat{y}_{i}\}_{i=1}^{n}$.
\end{algorithmic}
\end{algorithm}

\begin{remark} In this algorithm we get $\{\hat{y}_{i}\}_{i=1}^{n}$. For $i=n+1,\cdots, 2n$, we can get the corresponding $\{\hat{y}_{i}\}_{i=n+1}^{2n}$ in a similar way at the same time (learning $\hat{\bV}_r$ using the first half, then apply spectral clustering on the second half).
\end{remark}
% \r{Q:  Why the splitting is needed?  We can learn $\bB \bff_i$ using all the data and subtract them from the observed data.}


==> texfiles/old/proof_lemma.tex <==
\section{A cross-fitting type spectral clustering algorithm and the corresponding guarantee} \label{cv}


Consider the following "cross-fitting" type spectral clustering algorithm: 

\begin{algorithm}[H]
\caption{Spectral clustering}\label{alg3}
\begin{algorithmic}[1]
\State {\bf Input:} $\{\bx_i\}^{2n}_{i=1}$. The number of clusters $K$, target dimension of embedding $k$.
\State Split the data $\{\bx_i\}^{2n}_{i=1}$ into two halves, and use the second half to compute $\hat{V}$: 
\begin{equation*}
    \hat{\bV}:=(\bxi_{1},\cdots,\bxi_{k}),
\end{equation*}
where $\bxi_{1},\cdots,\bxi_{k}$ are the top $k$ right singular vectors of $(\hat{\bx}_{n+1},\cdots,\hat{\bx}_{2n})^{T} $.

\State Conduct $(1+\epsilon)$-approximate $K$-means on $\{\hat{\bV}^{T}\hat{\bx}_{i}\}_{i=1}^{n}$, getting $\{\hat{y}_{i}\}_{i=1}^{n}$ and $\{\hat{\bmu}_{j}\}_{j=1}^{K}$ such that:
\begin{equation*}
    \sum_{i=1}^n\|\hat{V}^{T}\bx_{i}-\hat{\bmu}_{\hat{y}_i}\|_2^2 \leq(1+\epsilon) \min _{\substack{\{\widetilde{\bmu}_j\}_{j=1}^K \subseteq \mathbb{R}^k \\\left\{\widetilde{y}_i\right\}_{i=1}^n \subseteq[K]}}\{\sum_{i=1}^n\|\hat{\bV}^{T}\bx_{i}-\widetilde{\bmu}_{\tilde{y}_i}\|_2^2\} .
\end{equation*}


\State {\bf Output:} $\{\hat{y}_{i}\}_{i=1}^{n}$.
\end{algorithmic}
\end{algorithm}


We have the following theoretical guarantee for Algorithm \ref{alg3} : 


\begin{lemma}\label{spectral_clustering_lemma_cv}
Consider the model defined in (\ref{spectral_clustering_model}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg3}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumption \ref{regularity} holds, and $d \leq O (n)$, then there exist constant $C$ and $c$ such that the following hold: \\
1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$.
\end{lemma}



In this section, we provide proofs for Lemma \ref{spectral_clustering_lemma_cv}. Consider the model defined in (\ref{spectral_clustering_model}). Let $\bX:= (\bx_{n+1}, \cdots, \bx_{2n})^{T}$.  We can write $\bX= \bF\bTheta + \bE$, where $\bTheta = (\btheta_{1},\cdots,\btheta_{K})^{T}\in \mathbb{R}^{K \times d} $ represents the cluster centers;
$\bF \in \mathbb{R}^{n \times k}$ is defined as $\bF_{ij}=1$ if and only if $y_{n+i}=j$, else $\bF_{ij}=0$, represents the true label of each data point, $\bE = (\bepsilon_{n+1}, \cdots, \bepsilon_{2n})^{T}$ be the noise matrix. In Algorithm \ref{alg3}, we compute $\hat{V}$ which is the top $K$ right singular vectors of $\bX$.  Let $V$ be the top $K$ right singular vectors of $\bF\bTheta$, which represents the subspace that contains the span of $\{\btheta_{j}\}_{j=1}^{K}$. The idea of proving Lemma \ref{spectral_clustering_lemma} is as the following. Notice that, since $\bV$ represents the subspace that contains the span of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$, and when $\hat{\bV}$ is close to $\bV$, then \\
1. $\bm_{j}:= \hat{\bV}^{T} \boldsymbol{\theta}_{j} $ should preserve the distance structure of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$. \\
2. For the $d$ dimensional sub-Gaussian noise $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$, when we project it onto $K$ dimensional subspace using $\hat{\bV}$, its norm becomes much smaller. Therefore, with these observations, we can use the following lemma (Lemma D.1 in \cite{abbe2022ellp}) to guarantee the success of approximate $K$-means:
\begin{lemma}[Approximate $K$-means] \label{approx_K_means} Let $\left\{\bx_i\right\}_{i=1}^n \subseteq \mathbb{R}^d$ and define
\begin{equation*}
L\left(\left\{\boldsymbol{\mu}_j\right\}_{j=1}^K,\left\{y_i\right\}_{i=1}^n\right)=\sum_{i=1}^n\left\|\bx_i-\boldsymbol{\mu}_{y_i}\right\|_2^2, \quad \forall\left\{\boldsymbol{\mu}_j\right\}_{j=1}^K \subseteq \mathbb{R}^d, \quad\left\{y_i\right\}_{i=1}^n \subseteq[K].
\end{equation*}
Let $\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{\hat{\boldsymbol{\mu}}_j\right\}_{j=1}^K \subseteq \mathbb{R}^d$, $\left\{y_i^{\star}\right\}_{i=1}^n,\left\{\hat{y}_i\right\}_{i=1}^n \subseteq[K]$, $s=\min _{j \neq k}\|\boldsymbol{\mu}_j^{\star}-\boldsymbol{\mu}_k^{\star}\|_2$ and $n_{\min}=\min_{j \in[K]} |\{i: y_i^{\star}=j\} |$. Suppose that the followings hold for some $C>0$ and $\delta \in(0, s / 2)$ :\\
1. (Near-optimality) $L\left(\left\{\hat{\boldsymbol{\mu}}_j\right\}_{j=1}^K,\left\{\hat{y}_i\right\}_{i=1}^n\right) \leq C \cdot L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right)$ and $\hat{y}_i \in \operatorname{argmin}_{j \in[K]}\left\|\bx_i-\hat{\boldsymbol{\mu}}_j\right\|_2$ for all $i \in[n]$;\\
2. (Low-noise condition) $L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) \leq \delta^2 n_{\min } /\left[(1+\sqrt{C})^2 K\right]$.\\
Then, there exists a permutation $\tau:[K] \rightarrow[K]$ such that
\begin{align*}
& \sum_{j=1}^K\left\|\boldsymbol{\mu}_j^{\star}-\hat{\boldsymbol{\mu}}_{\tau(j)}\right\|_2^2 \leq \frac{(1+\sqrt{C})^2 K}{n_{\min }} L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right), \notag \\
& \left\{i: \hat{y}_i \neq \tau\left(y_i^{\star}\right)\right\} \subseteq\left\{i:\left\|\bx_i-\boldsymbol{\mu}_{y_i^{\star}}^{\star}\right\|_2 \geq s / 2-\delta\right\}, \notag \\
& \left|\left\{i: \hat{y}_i \neq \tau\left(y_i^{\star}\right)\right\}\right| \leq\left|\left\{i:\left\|\bx_i-\boldsymbol{\mu}_{y_i^{\star}}^{\star}\right\|_2 \geq s / 2-\delta\right\}\right| .
\end{align*}
\end{lemma}
We also need the following lemma for bounding the distance between $\bV$ and $\hat{\bV}$: 
\begin{lemma} \label{lemma_3}
With probability greater than $1-O(1/n)$,
\begin{equation*}
\text{dist}(\bV,\hat{\bV}) := \min_{R \in \mathcal{O}^{r \times r}}\|\bV\bR-\hat{\bV}\| \leq O(\frac{8 \sigma (\sqrt{n}+\sqrt{d})}{\sqrt{n}}) \leq O(\sigma).
\end{equation*}
\end{lemma}
The proof of this lemma is deferred to the next subsection. We also need the following two lemmas from \cite{zhang2022leaveoneout}: 

\begin{lemma} [Lemma D.1 in \cite{zhang2022leaveoneout}] \label{Lemma_D.1_leave_one_out}
Let $\bA= (\ba_{1}, \cdots, \ba_{n}) \in \mathbb{R}^{k \times n}$ be a random matrix with each column $\ba_{i} \sim \text{SG}_{k}(\sigma^{2}) $ independently for every $i \in [n]$. Then 
\begin{equation*}
    \mathbb{P}(\|\bA\| \geq 4t\sigma (\sqrt{n}+ \sqrt{k})) \leq \exp \left(-\frac{(t^{2}-3)n}{2}\right)
\end{equation*}
for any $t \geq 2$.
\end{lemma}

\begin{lemma} [Lemma D.2 in \cite{zhang2022leaveoneout}] \label{Lemma_D.2_leave_one_out}
Let $\boldsymbol{X} \sim \text{SG}_{d}(\sigma^{2}))$ be a $d$ dimensional sub-Gaussian random vector. Then for any $k \leq d$, for any matrix $\bU = (\bu_{1}, \cdots, \bu_{k}) \in \mathbb{R}^{d\times k}$ with orthogonal columns. We have  
\begin{equation*}
    \mathbb{P}(\|\bU^{T}\bX\|^{2} \geq \sigma^{2} (k +2\sqrt{kt} + 2t)) \leq e^{-t}.
\end{equation*}
\end{lemma}

Intuitively, Lemma \ref{Lemma_D.1_leave_one_out} controls the norm of our noise matrix $E$. Lemma \ref{Lemma_D.2_leave_one_out} shows that when we project a sub-Gaussian random vector on to low dimensional subspace, its norm becomes much smaller. With these lemmas, we are now able to prove Lemma \ref{spectral_clustering_lemma}. Let 
\begin{align*}
    \bz_{i} := \hat{\bV}^{T} \bx_{i}, \\
    \bm_{j}:= \hat{\bV}^{T} \btheta_{j}.
\end{align*}
Since $\hat{\bV}$ is the top $K$ right singular vectors of $X:= (\bx_{n+1}, \cdots, \bx_{2n})^{T}$, it's independent from $\{\bx_{i}\}_{i=1}^{n}$ which we will perform spectral clustering on. By Lemma \ref{lemma_3}, with high probability (our following analysis will on this event), there exists $\bR \in \mathcal{O}^{r \times r}$ such that $\|\bV\bR-\hat{\bV}\| \leq O(\sigma).$ Then
\begin{align*}
    \|\bm_{i}-\bm_{j}\| &= \|\hat{\bV}^{T}(\btheta_{i}-\btheta_{j})\| \notag \\ 
    & \geq \|(\bV\bR)^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|((\bV\bR)^{T}-\hat{\bV}^{T})(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| \notag \\
    & \geq \|\bR^{T}\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|((\bV\bR)^{T}-\hat{\bV}^{T})\|\|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| \notag \\
    & = \|\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|\bV\bR-\hat{\bV}\| \|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\|.
\end{align*}
Since $\bV$ represents the subspace that contains the span of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$, there exists $\bbeta$ such that $\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j} = \bV\boldsymbol{\beta}$, and $\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| = \|\boldsymbol{\beta}\|$. Then $\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}) = \bV^{T}\bV\boldsymbol{\beta} = \boldsymbol{\beta}$, therefore $\|\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| = \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|$. Also, $\|\bV\bR-\hat{\bV}\| \leq O(\sigma).$ Combine these together we have 
$\|\bm_{i}-\bm_{j}\| \geq (1-O(\sigma))\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| \geq \frac{1}{2}\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|$. The last inequality holds when $\sigma \ll 1$, which holds because we assume $1 \ll \tilde{\text{SNR}}$ in the assumption of Lemma \ref{spectral_clustering_lemma} .

Now we can use Lemma \ref{approx_K_means} to prove our main result. In this lemma, take $\bx_{i}$ to be our $\bz_{i}$,  $\bmu_{j}^{\star}$ to be our $\bm_{j}$, and $y_{i}^{\star}$ to be our $y_{i}$. First we check the "near-optimality" condition in Lemma \ref{approx_K_means}: this holds with $C=1+\epsilon$ because we use $K$-means in our Algorithm \ref{alg2}. Second, we check the "low-noise" condition. 
\begin{align*}
    L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) &= \sum_{i=1}^{n} \|\bz_{i} - \bm_{y_{i}}\|^{2} \notag \\
    &= \sum_{i=1}^{n} \|\hat{\bV}^{T} \bx_{i} - \hat{\bV}^{T} \boldsymbol{\theta}_{y_{i}} \|^{2} \notag \\
    &= \sum_{i=1}^{n} \|\hat{\bV}^{T} \bepsilon_{i}  \|^{2} \notag \\
    &= \|\tilde{\bE}\|_{F}^{2},
\end{align*}
where we define $\tilde{\bE} := (\hat{\bV}^{T} \bepsilon_{1}, \cdots, \hat{\bV}^{T} \bepsilon_{n} ) \in \mathbb{R}^{k \times n}$. Notice that each column of $\tilde{\bE}$ is $\hat{\bV}^{T} \bepsilon_{i}$, which is independent from each other. Since we have $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$, $\hat{\bV} \in \mathbb{R}^{d \times k}$ is an projection matrix independent of those $\bepsilon_{i}$, we have $\hat{\bV}^{T} \bepsilon_{i} \sim \text{SG}_{k}(\sigma^{2})$. Therefore by Lemma \ref{Lemma_D.1_leave_one_out}, take $t=2$, we have with probability greater than $1-\exp (-\frac{1}{2}n)$, $\|\tilde{\bE}\| \leq 8 \sigma (\sqrt{n}+ \sqrt{k})$.
Then on this event, 
\begin{align*}
   L\left(\left\{\bmu_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) &= \|\tilde{\bE}\|_{F}^{2} \notag \\
   & \leq k\|\tilde{\bE}\|^{2} \notag \\
   & \leq k (8 \sigma (\sqrt{n}+ \sqrt{k}))^{2} \notag \\
   & \leq O(n\sigma^{2}). 
\end{align*}
where the last ineqaulity holds since $k=O(1)$. Therefore the low noise condition holds for $\delta = O(\sigma)$ (notice that we have regularity assumptions, so that $n_{\min }$ can not be very close to zero, with high probability). Thus, we can apply Lemma \ref{approx_K_means}, which gives 
\begin{align*}
    \left\{i: \hat{y}_i \neq \tau\left(y_i\right)\right\} &\subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq \frac{1}{2} \min_{i \neq j} \|\bm_{i}-\bm_{j}\|-\delta\right\}  \notag \\
    & \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq \frac{1}{4} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|-\delta\right\}  \notag \\
    & \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|\right\} 
\end{align*}
where the last inequality holds for some constant $c_5 >0$ since we assume $1 \ll \tilde{\text{SNR}}$  so that $\sigma \leq o(\min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|)$. Finally, since $\hat{\bV} \in \mathbb{R}^{d \times k}$ is an projection matrix independent of those $\bepsilon_{i}$, by Lemma \ref{Lemma_D.2_leave_one_out}, we have 
\begin{equation*}
    \mathbb{P}(\|\hat{\bV}^{T}\bepsilon_{i}\|^{2} \geq \sigma^{2} (k +2\sqrt{kt} + 2t)) \leq e^{-t}.
\end{equation*}
Take $t = \frac{c_6}{\sigma^{2}} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}$ for some sufficiently small constant $c_6>0$, then we have 
\begin{equation*}
    \mathbb{P}(\|\hat{\bV}^{T}\bepsilon_{i}\|^{2} \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}) \leq \exp (-\frac{c_6}{\sigma^{2}} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}) = \exp (- c_6 \tilde{\text{SNR}}) .
\end{equation*}
Since 
\begin{equation*}
    \left\{i: \hat{y}_i \neq \tau\left(y_i\right)\right\} \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|\right\} ,
\end{equation*}
we have 
\begin{align*}
    \mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) &\leq \mathbb{P} \left( \left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| \right) \notag \\
    & \leq \exp (- c_6 \tilde{\text{SNR}}) .
\end{align*}
Therefore there exist some constant $C$, such that when $\tilde{\text{SNR}} \geq C \log n$, $\mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) \leq e^{- \alpha \log n} = n^{-\alpha}$ for some $\alpha >2$. Then by union bound (notice that all the "high probability event" in our previous analysis will have probability converges to 1 when $n \rightarrow \infty$"), 
\begin{equation*}
\mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0] \geq 1 - n \cdot n^{-\alpha} - o(1) = 1- o(1) - n^{1-\alpha} \rightarrow 1,
\end{equation*}
when $n \rightarrow \infty$. 

On the other hand, for $C \log n \geq \tilde{\text{SNR}} \gg 1$, we have $\mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) \leq e^ {- c_6 \tilde{\text{SNR}}}$. This implies
\begin{equation*}
    \mathbb{E} [\mathcal{M}(\hat{\by}, \by)] = \mathbb{E} [\frac{1}{n}\sum_{i=1}^{n} \mathbb{I}_{(\hat{y}_i \neq \tau\left(y_i\right))}] \leq e^ {- c_6 \tilde{\text{SNR}}}
\end{equation*} 
which is what we want (again, the "high probability event" in previous analysis are negligible) .

\subsection{Proof for Lemma \ref{lemma_3}}
We give the proof of Lemma \ref{lemma_3} in this subsection. By Wedin's sin$\Theta$ theorem (see \cite{MAL-079} Theorem 2.9), 
\begin{equation*}
\text{dist} (\bV, \hat{\bV}) \leq \frac{2\|\bX-\bF\bTheta\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})} = \frac{2\|\bE\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})},
\end{equation*}
where $\sigma_{k}(\bF\bTheta)$ and $\sigma_{k+1}({\bF\bTheta})$ denote the $k$-th and $(k+1)$-th singular value of $\bF\bTheta$ respectively. By Lemma \ref{Lemma_D.1_leave_one_out}, take $t=2$, we have with probability greater than $1-\exp (-\frac{1}{2}n)$, $\|\bE\| \leq 8 \sigma (\sqrt{n}+ \sqrt{d})$.

For $\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})$, notice that $\sigma_{k+1}(\bF\bTheta) = 0$ (since $\bTheta$ is rank $k$), and 
\begin{align*}
    \sigma_{k}(\bF\bTheta) = \sqrt{\lambda_{k}((\bF\bTheta)^{T}(\bF\bTheta))} = \sqrt{n} \cdot \sqrt{\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta))}.
\end{align*}
Since $(\bF\bTheta)^{T}(\bF\bTheta) = \sum_{j=1}^{K}n_{j}\btheta_{j}\btheta_{j}^{T}$, where $n_{j} = |\{i \in [n]: y_{i}=j\}|$, we have 
\begin{equation*}
\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta) = \frac{1}{n} \sum_{j=1}^{K}n_{j}\btheta_{j}\btheta_{j}^{T} \rightarrow \sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}.
\end{equation*}
To be more specific, by Weyl's inequality (see \cite{MAL-079} Lemma 2.2), 
\begin{align*}
    |\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta)) - \lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T})| &\leq \|\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta) - \sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}\| \notag \\
&\leq \sum_{j=1}^{k}|\frac{n_{j}}{n} -p_{j}| \|\btheta_{j}\btheta_{j}^{T}\| \notag \\
& \leq O(\frac{\log n}{\sqrt{n}})
\end{align*}
with probability greater than $1-O(1/n)$, because $n_{j}$ is a binomial random variable (so that it has sub-Gaussian tail bound), and $\btheta_{j}\btheta_{j}^{T}$ is $O(1)$.

Also notice that by our regularity assumptions (Assumption \ref{regularity}), $\lambda_{k} (\mathbb{\bE}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) \geq c_3$, which is equivalent to $\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) \geq c_3$. Then
\begin{align*}
  \sigma_{k}(\bF\bTheta) &= \sqrt{n} \cdot \sqrt{\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta))}  \notag \\
  &=\sqrt{n} \cdot  \sqrt {\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) - (\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta)) - \lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}))} \notag \\
& = \sqrt{n} \cdot  \sqrt {\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) + O(\frac{\log n}{\sqrt{n}})} \notag \\
&\geq  c_7 \sqrt{n}
\end{align*}
for some constant $c_7>0$. Therefore
\begin{align*}
\text{dist} (\bV, \hat{\bV}) &\leq \frac{2\|\bE\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})} \notag \\
& \leq \frac{2 \cdot 8 \sigma (\sqrt{n}+ \sqrt{d})}{c_7 \sqrt{n}} \notag \\
& \leq O(\sigma).
\end{align*}
The last line follows from our assumption that $d = O(n)$.



\section{Proof for Lemma \ref{justify_approx_perp_lemma}}
\label{justify_approx_perp_lemma_proof}
Since $\bU$ and $\bM$ have orthogonal columns, it is trivial that $\|\bU^{T}\bM\| \leq 1 \leq \sqrt{\frac{d}{\log n}}$. For the assumption $\|\bU^{T}\bM\| \leq \frac{c_3}{9C_3}$, suppose $\bB$ is already given and fixed. Thus $\bU$ is also fixed. Consider the Grassmannian manifold $G_{d,k}$ that consists of all $k$-dimensional subspaces of $\mathbb{R}^{d}$. Let $\bM \sim \text{Unif} (G_{d,k})$ (see \cite{vershynin2018high} for detailed discussion of the measure on Grassmannian manifold), which means $M$ represents a uniformly randomly chosen $k$-dimensional subspace of $\mathbb{R}^{d}$. Let the columns of $\bU$ be $(\bw_{1},\cdots,\bw_{r})$, then by Lemma 5.3.2 in \cite{vershynin2018high}, for each $\bw_{i}$,

\begin{equation*}
    \mathbb{P} \left( \left|\|\bw_{i}^{T} \bM \|- \sqrt{\frac{K}{d}}\right| \geq t \right) \leq 2e^{-cdt^{2}} 
\end{equation*}
for some constant $c$. Take $t=(100C_3\sqrt{r}/c_3)^{-1}$, then with probability no less than $1-2\exp{(-cdt^{2})}$,
\begin{equation*}
    \|\bw_{i}^{T} \bM\| \leq t + \sqrt{\frac{k}{d}} \leq (100C_3\sqrt{r}/c_3)^{-1} + \sqrt{\frac{K}{c_1 \log n}} \leq (50C_3\sqrt{r}/c_3)^{-1}
\end{equation*}
for sufficiently large $n$ (since $k$ and $r$ are assumed to be $\Omega(1)$.)

Take $c_1$ sufficiently large (recall $d \geq c_1 \log n$) such that 
$ct^{2}d\geq ct^{2}c_1 \log n \geq 10 \log n$. Then $1-2\exp{(-cdt^{2})} \geq 1-2n^{-10}$. Therefore we have, with probability no less than $1-2n^{-10}$, $\|\bw_{i}^{T} \bM\| \leq (50C_3\sqrt{r}/c_3)^{-1}$. Take the union bound, we have with probability greater than $ 1- 2r n^{-10} \geq 1-n^{-9}$ (for sufficiently large $n$), for every $i\in [r]$, $\|\bw_{i}^{T} \bM\| \leq (50C_3\sqrt{r}/c_3)^{-1}$. Thus, under this very high probability event,
$\|\bU^{T}\bM\| \leq \sqrt{\sum_{i=1}^{r} \|\bw_{i}^{T} \bM\|^{2}} \leq \frac{c_3}{9C_3}$.


==> texfiles/old/proof_main_result.tex <==
\section{Proofs for Theorem \ref{main_thm}}
In this appendix, we will show how to prove Theorem \ref{main_thm}. As in the proof sketch section, for the first phase,
\begin{align*}
    \hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i} \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) (\bB \bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})    \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{y_{i}} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i}  \\
    &:= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{align*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. We will first introduce several technical lemmas for analyzing $\tilde{\bmu}_{y_i}$  and $\tilde{\bepsilon}_{i}$.

\subsection{Technical lemmas for factor model estimation}


Let $\bDelta:=\bV_{r}\bV_{r}^{T} -\hat{\bV}_{r}\hat{\bV}_{r}^{T}$. We have the following lemmas for bounding $\|\bDelta\|$.
\begin{lemma}\label{matrix_perturbation_lemma}
Consider the model defined in (\ref{factor_cluster}). Let $\bSigma := \EE{\bx_{i}\bx_{i}^{T}}$ be the population covariance matrix, and $\hat{\bSigma}:= \frac{1}{n}\sum_{i=1}^{n} \bx_{i} \bx_{i}^{T}$ be the empirical covariance matrix. When $n \geq d$, for sufficiently large $n$ ("sufficiently large" means $n$ greater than some absolute constant), we have
\begin{equation*}
    \|\hat{\bSigma}- \bSigma\| \lesssim \lambda_{1}^{*} \sqrt{\frac{\log n}{n}} + \sqrt{\frac{\lambda_{1}^{*}d \log n}{n}} + \sqrt{\frac{d \log n}{n}} + \frac{d \log^2 n}{n}
\end{equation*}
with probability greater than $1-O(n^{-10})$. Here $\lambda_{1}^{*} = \lambda_{max}(\bB \bB^{T})$. 
\end{lemma}
% \begin{lemma}\label{matrix_perturbation_lemma}
% Consider the model defined in (\ref{factor_cluster}). Let $\Sigma := \mathbb{E}{\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{T}}$ be the population covariance matrix, and $\hat{\Sigma}:= \frac{1}{2n}\sum_{i=2n+1}^{4n} \boldsymbol{x}_{i} \boldsymbol{x}_{i}^{T}$ be the empirical covariance matrix. Let $A:=\mathbb{E}{\boldsymbol{u}_{i}\boldsymbol{u}_{i}^{T}}$, then we have
% \begin{equation*}
%     \|\hat{\Sigma}- \Sigma\| \leq C (\lambda_{1}^{*} \sqrt{\frac{r}{n}} + \sqrt{\frac{\|A\| \lambda_{1}^{*}d}{n}} +  \|A\| \sqrt{\frac{d}{n}} + \frac{\|A\| d (\log (n+d))^{\frac{3}{2}}}{n}  ) (\log (n+d))^{\frac{1}{2}}
% \end{equation*}
% with probability greater than $1-O((n+d)^{-10})$, when $n\geq cr (\log (n+d))^{3}$ for some constant $c,C$. Here $\lambda_{1}^{*} = \lambda_{max}(BB^{T})$. 
% \end{lemma}
% In fact, this is just the Lemma 3.5 in \cite{MAL-079}, where we replaced the $\boldsymbol{\eta}_{i} \sim \mathcal{N}(0,\sigma^{2} I_{d})$ in this book by $\boldsymbol{u}_{i} \sim \mathcal{N}(0,A)$. Notice that $\lambda_{1}^{*} = \Omega (d)$ by pervasiveness condition, and $\|A\|= O(1)$ by assumption. Therefore by Davis-Kahan Theorem, we can easily get the following proposition, which is standard in matrix perturbation theory: 
Lemma \ref{matrix_perturbation_lemma} is a generalized version of Lemma 3.5 in \cite{MAL-079}. By Davis-Kahan Theorem (see \cite{MAL-079}), since $\hat{V}_{r}$ is the top $r$ eigenvectors of $\hat{\Sigma}$, $V_{r}$ is the top $r$ eigenvectors of $\Sigma$, we have
\begin{equation*}
    \|\bDelta\| \leq \frac{\|\hat{\bSigma}- \bSigma\|}{\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)},
\end{equation*}
where $\lambda_{r}(\bSigma)$ and $\lambda_{r+1}(\bSigma)$ are the $r$-th and $(r+1)$-th largest eigenvalues of $\bSigma$ respectively. Under the conditions of Theorem \ref{main_thm}, i.e., by pervasiveness condition, $\bSigma = \bB \bB^{T} + \EE \bu_i\bu_i^{T}$, all the $r$ non-zero eigenvalues of $\bB\bB^{T}$ scales as $\Omega(d)$, $\|\EE \bu_i\bu_i^{T}\| = O(1)$, we have $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) = \Omega (d)$. Therefore from Lemma \ref{matrix_perturbation_lemma} we get the following proposition for controlling $\|\bDelta\|$.

\begin{proposition} \label{matrix_perturbation_proposition}
Under the conditions of Theorem \ref{main_thm}, we have
\begin{equation*}
\| \bDelta \| \leq O (\sqrt{\frac{\log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}


\subsection{Technical lemma for phase 1}
The next lemma shows why Assumption \ref{approximate_perpendicularity} is important in our analysis, and why it can indicate (\ref{strict_perpendicularity}) .

\begin{lemma} \label{approx_per_lemma}
Under Assumption \ref{regularity}, \ref{pervasiveness} and \ref{approximate_perpendicularity}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma}
This lemma shows that when Assumption \ref{approximate_perpendicularity} holds, we have  (\ref{strict_perpendicularity}), and the Assumption \ref{regularity} still holds after projection, which will facilitate our analysis. 

% \begin{proof} [Proof for Lemma \ref{approx_per_lemma}]
%     Under Assumption \ref{approximate_perpendicularity}, 
% \begin{align*}
%     \Sigma &:= \mathbb{E} [{\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{T}}] \notag \\
%     & =  \mathbb{E} [(B\boldsymbol{f}_{i}+ \boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i})(B\boldsymbol{f}_{i}+ \boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i})^{T}] \notag \\
%     & = BB^{T} + \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] + \sigma^{2} I_{d} \notag \\
%     &= U \Lambda U^{T} + MVM^{T} + \sigma^{2} I_{d}. \notag \\
% \end{align*}
% We consider $\tilde{\Sigma} := U \Lambda U^{T} + (I-UU^{T})MVM^{T}(I-UU^{T})^{T} + \sigma^{2} I_{d}.$ Notice that 
% \begin{equation*}
% U^{T} (I-UU^{T})M = (U^{T}- U^{T}UU^{T}) M = (U^{T}-U^{T})M = 0.   
% \end{equation*}
% This means the column space of $(I-UU^{T})MVM^{T}(I-UU^{T})^{T}$ (which belongs to the column space of $(I-UU^{T})M$) is orthogonal to the column space of $U$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%     (I-UU^{T})MVM^{T}(I-UU^{T})^{T} = U_{\perp} \bar{V} U_{\perp}^{T}
% \end{equation*}
% for some $U_{\perp}$ that $U_{\perp}U^{T}=0$. Thus, we have 
% \begin{equation*}
%     \tilde{\Sigma} = (U, U_{\perp},U_0)\begin{pmatrix}
%  \Lambda & &  \\
%   & \bar{V} & \\
%  & & 0
%  \end{pmatrix} (U, U_{\perp},U_0)^{T} + \sigma^{2} I_{d}
% \end{equation*}
% where $U_{0}$ is the orthogonal complement of $(U, U_{\perp})$. Since by pervasiveness condition, $\lambda_{r}(\Lambda) = \sigma_{min}(B)^{2} = \Omega(d)$, $\|\bar{V}\| \leq \|\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]\| = O(1)$, $\sigma^{2} = O(1)$, we have the top $r$ eigenvectors of $\tilde{\Sigma}$ is just $U$. Since $V_{r}$ is the top $r$ eigenvectors of $\Sigma$, by Davis-Kahan theorem, 
% \begin{equation} \label{dist_U_Vr}
% \text{dist} (U, V_{r}) := \|UU^{T}- V_{r}V_{r}^{T}\| \leq \frac{\|\Sigma- \tilde{\Sigma}\|}{\lambda_{r}(\tilde{\Sigma})}.
% \end{equation}
% It is obvious that $\lambda_{r}(\tilde{\Sigma}) = \lambda_{r}(\Lambda) = \Omega (d)$. For $\|\Sigma- \tilde{\Sigma}\|$, we have 
% \begin{align*}
%     \Sigma- \tilde{\Sigma} & = (U\Lambda U^{T} + MVM^{T} +\sigma^{2}I_{d}) - (U \Lambda U^{T} + (I-UU^{T})MVM^{T}(I-UU^{T})^{T} + \sigma^{2} I_{d}) \notag \\
%     &= UU^{T} MVM^{T} +MVM^{T}UU^{T} - UU^{T} MVM^{T} UU^{T}.
% \end{align*}
% Therefore 
% \begin{align*}
%     \|\Sigma- \tilde{\Sigma} \|& \leq  \|UU^{T} MVM^{T}\| +\|MVM^{T}UU^{T}\| + \|UU^{T} MVM^{T} UU^{T}\| \notag \\
%     &\leq 2\|U\|\|U^{T}M\|\|V\|\|M^{T}\| + \|U\|\|U^{T} M\|\|V\|M^{T} U\|\|U^{T}\| \notag \\
%     & \leq O(\|U^{T}M\|).
% \end{align*}
% Therefore by Davis-Kahan (\ref{dist_U_Vr}), $\text{dist} (U, V_{r})  \leq O(\|U^{T}M\|/d).$ With this in mind, we are able to get the desired result. For the first claim,
% \begin{align*}
%     \|(I-V_{r}V_{r}^{T})B\| &\leq \|(I-UU^{T})B\|  +  \|(UU^{T}- V_{r}V_{r}^{T})B\| \notag \\
%     &= 0 + \|(UU^{T}- V_{r}V_{r}^{T})B\| \notag \\
%     &\leq  \text{dist} (U,V_{r})\|B\| \notag \\
%     &\leq  O(\|U^{T}M\|/d) \times \Omega(\sqrt{d}) \notag \\
%     & \leq O(\frac{\|U^{T}M\|}{\sqrt{d}}) \notag \\
%     & \leq O(\sqrt{\frac{1}{\log n}}),
% \end{align*}
% where the last line follows from Assumption \ref{approximate_perpendicularity}. 

% For the second claim,
% \begin{align*}
%     &\| (I-V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| \notag \\
%     &\geq \|(I-UU^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| - \|(UU^{T}- V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     &\geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \text{dist} (U,V_{r})\|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|.
% \end{align*}
% Notice that $\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2} \in \text{Col} (M)$, then there exists $\boldsymbol{\alpha}$ such that $\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2} = M \boldsymbol{\alpha}$, and $\|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| = \|\boldsymbol{\alpha}\|$. Then we have 
% \begin{align*}
%    \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| & = \|UU^{T}M \boldsymbol{\alpha}\| \notag \\
%    &\leq \|U^{T}M \boldsymbol{\alpha}\| \notag \\
%    & \leq \|U^{T}M\| \|\boldsymbol{\alpha}\| \notag \\
%    &\leq \frac{1}{2} \|\boldsymbol{\alpha}\| = \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity}. Therefore 
% \begin{align*}
%     &\| (I-V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| \notag \\
%     &\geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \text{dist} (U,V_{r})\|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|- \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - O(\|U^{T}M\|/d) \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - O(\sqrt{\frac{1}{d \log n}}) \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq c_2 \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})) \\ \notag 
%      &\geq  \lambda_{k} ((I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T})) - \|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\| \\ \notag 
%      & \geq \lambda_{k} (\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) - \| \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] -
%      (I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) \| \notag \\
%      &- \|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] -
%      (I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) \| \notag \\
%     & = \|UU^{T} MVM^{T} +MVM^{T}UU^{T} - UU^{T} MVM^{T} UU^{T}\| \notag \\
%     & \leq 2 \|U^{T}M\|\|V\| + \|U^{T}M\|^{2}\|V\| \notag \\
%     & \leq C_3 (2\|U^{T}M\| + \|U^{T}M\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \notag \\
%     & \leq 3C_3 \|U^{T}M\| \quad (\text{Since} \|U^{T}M\| \leq 1) \notag \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\| \notag \\
%     & = \|(UU^{T}MVM^{T}UU^{T} - UU^{T}MVM^{T} - MVM^{T}UU^{T})  \notag \\
%     &- (V_{r}V_{r}^{T}MVM^{T}V_{r}V_{r}^{T}  - V_{r}V_{r}^{T}MVM^{T} - MVM^{T}V_{r}V_{r}^{T})\|  \notag \\
%     & \leq \|UU^{T}MVM^{T}UU^{T} - V_{r}V_{r}^{T}MVM^{T}V_{r}V_{r}^{T}\| \notag \\
%     &+ 2\|UU^{T}MVM^{T} - V_{r}V_{r}^{T}MVM^{T}\| \notag \\
%     & \leq 2 \|V\| \|UU^{T} - V_{r}V_{r}^{T} \| + 2 \|V\| \|UU^{T} - V_{r}V_{r}^{T} \| \notag \\
%     & \leq 4 C_3 O(\frac{\|U^{T}M\|}{d}) \notag \\
%     & \leq O (\sqrt{\frac{1}{d \log n}}) \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
% \end{align*}
% Combine the above three inequalities, we have 
% $\lambda_{k} ((I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})) \geq \frac{1}{2}c_3$. 





% Therefore we proved Lemma \ref{approx_per_lemma}.
% \end{proof}

\subsection{Proofs for Theorem \ref{main_thm}}

 As in the proof sketch section, we have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (\sqrt{\frac{\log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by Proposition \ref{matrix_perturbation_proposition}). For $j_{1} \neq j_{2}$, 
\begin{equation*}
    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
\end{equation*}
On the other hand,
\begin{align*}
   \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
   & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
   &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma}}) \\
   & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (\sqrt{\frac{\log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Proposition \ref{matrix_perturbation_proposition}})\notag \\
   & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
    \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
\end{align*}
\shange{$\Delta$ is a random quantity. Do not write it in this way! Directly claim $\Delta$ is small with high prob,  and then jump to the result you want, see later}Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Proposition \ref{matrix_perturbation_proposition}}) \\
    & \leq O (\sigma^2) +O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma}}) \\
    & \leq  O (\sigma^2) +O(\frac{d \log n}{n}) + \sigma^{2} \qquad (\text{By pervasiveness condition})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{2}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. 

From the above analysis, we know that after our first phase, with probability greater than $1-O(n^{-10})$, we have $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$, where $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$ and  $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$. \shange{directly jump to this result!}In our Algorithm \ref{alg1}, after obtaining $\hat{\bu}_{i}$, we actually conduct Algorithm \ref{alg2} with input $\{\bx_i\}^{n}_{i=1} := \{\hat{\boldsymbol{u}}_{i}\}^{n}_{i=1}$, the number of clusters $K$, and target dimension of embedding $k$. We now verify that Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$: the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
\begin{align*}
    & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
     &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
     &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
     & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
     & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
     & \geq \frac{1}{2}c_3 - O(\sqrt{\frac{\log n}{n}}) \notag \\
     &\geq  \frac{1}{3}c_3.
\end{align*}
Then by Lemma \ref{spectral_clustering_lemma}, there exist constant $C$ and $c$ such that the following hold: \\
1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
\begin{equation*}
    \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
\end{equation*}
Recall our definition for $\overline{\text{SNR}}$:  
\begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
\end{equation*}
Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{main_thm}.

\subsection{Proofs for Lemma \ref{matrix_perturbation_lemma} and \ref{approx_per_lemma}}

\paragraph{Proof for Lemma \ref{matrix_perturbation_lemma}}
\begin{proof}
Recall the model defined in (\ref{factor_cluster}): 
\begin{align*}
    &\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
    &\bx_{i}=\bB\bff_{i}+\bu_{i},  \quad \mbox{and} \quad    \bu_{i}=\bmu_{y_{i}} + \bepsilon_{i}.
\end{align*}
Here $\EE\bff_i=0$, $\EE \bmu_{y_{i}}=0$, $\EE \bepsilon_{i}=0$, $\cov(\bff_i)=\EE \bff_i\bff_i^{T}=\bI_r$. We also assume sub-Gaussian and boundedness properties: $\bff_i \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_i \sim \text{SG}_{d}(\sigma^2)$, $\|\bmu_j\| \leq c_2$ for any $j \in [K]$. Since $\sigma^2 \leq O(1)$, we conclude that $\bu_i$ is also sub-Gaussian with parameter $c_3^2$. 
To deal with matrix concentration, we will need the following lemma (Corollary 3.2 in \cite{MAL-079}), which is a truncated version of matrix Bernstein inequality:
\begin{lemma}[Truncated matrix Bernstein inequality]\label{matrix_Bernstein}
Let $\bZ, \bZ_1, \cdots, \bZ_n$ be i.i.d. random matrices with dimension $m_1\times m_2$. Suppose the followings hold: 
\begin{equation}\label{Bernstein_condition}
\PP(\|\bZ - \EE[\bZ]\| \geq L) \leq q_0 \quad \mbox{and} \quad  \| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}   ]   \|  \leq q_1 .
\end{equation}
Define the matrix variance statistic $V$ as $V= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \}$. Set $m:=\max\{m_1,m_2\}$. For any $a \geq 2$, with probability at least $1-2m^{-a+1}-nq_0$, 
\begin{align*}
\|\frac{1}{n}\sum_{i=1}^{n} ( \bZ_i - \EE \bZ_i )\| \leq V \sqrt{\frac{2a \log m}{n}} + L  \frac{2a \log m}{3 n}  + q_1,    
\end{align*}
where $m=m_1+m_2$.
\end{lemma}
Back to the proof of \ref{matrix_perturbation_lemma}, we have the following decomposition: 
\begin{align} \label{matrix_perturbation_ineq1}
    \|\hat{\bSigma}- \bSigma\| &= \|\frac{1}{n}\sum_{i=1}^{n}\bx_i\bx_i^{T} - \EE \bx_i\bx_i^{T}\| \notag \\
    &= \|\frac{1}{n}\sum_{i=1}^{n}(\bB \bff_i + \bu_i)(\bB \bff_i + \bu_i)^{T} - \EE (\bB \bff_i + \bu_i)(\bB \bff_i + \bu_i)^{T}\| \notag \\
    & \leq \|\bB\|^{2} \|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\| + 2\|\bB\| \|\frac{1}{n}\sum_{i=1}^{n}\bff_i \bu_i^{T}\| + \|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\|.
\end{align}
We will then bound each of the three terms by matrix Bernstein inequality. For $\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bff_i\bff_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall that $\bff_i \sim \text{SG}_{r} (c_1^2)$ implies $\|\bff_i\| \sim \text{SG} (r c^2)$ (see \cite{jin2019short} Lemma 1). Therefore 
\begin{align*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) & = \PP(\|\bff_i \bff_i^{T} - \EE[\bff_i \bff_i^{T}]\| \geq L) \\
&\leq \PP(\|\bff_i \bff_i^{T}\| +\| \EE[\bff_i \bff_i^{T}]\| \geq L) \\
&= \PP(\|\bff_i \bff_i^{T}\| \geq L-1) \\
&\leq \PP(\|\bff_i\|^2 \geq L-1) \\
&= \PP(\|\bff_i\| \geq \sqrt{L-1})
\end{align*}
Take $L= 22c^2 r \log n + 2$, by sub-Gaussian tail bound, we have $\PP(\|\bff_i\| \geq \sqrt{L-1}) \leq 2 n^{-11} :=q_0$. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bff_i\bff_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bff_i\bff_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty}  \PP(\|\bff_i\|^2 \geq y) \mathrm{d} y + L \PP (\|\bff_i\|^2 \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2rc^2}}\mathrm{d} y + 2Le^{-\frac{L}{2rc^2}} \\
&= (4rc^2+2L) e^{-\frac{L}{2rc^2}}\\
& \leq 3L e^{-\frac{L}{2rc^2}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T} - (\EE \bff_i \bff_i^{T})^2\|^{1/2} \\
& \leq \|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}\|^{1/2}.
\end{align*}
The last inequality is due to the fact that $\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}-(\EE \bff_i \bff_i^{T})^2$ and $(\EE \bff_i \bff_i^{T})^2$ are both positive semidefinite. For $\|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}\|$, notice that for any $\bv \in \RR^r$ such that $\|\bv\|=1$, 
\begin{align*}
    \bv^{T} (\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}) \bv &= \EE [(\bff_i^{T} \bv)^2 \bff_i^{T} \bff_i] \\
    & \leq \sqrt{\EE (\bff_i^{T} \bv)^4 \EE (\bff_i^{T} \bff_i)^2 }  \qquad \text{(by Cauchy inequality)} \\
    & \leq c \sqrt{\EE \|\bff_i\|^4} \qquad \text{(since $\bff_i^{T} \bv \sim \text{SG}(c_1^2)$)} \\
    & \leq C r \qquad \text{(since $\|\bff_i\| \sim \text{SG}(c^2r)$)} 
\end{align*}
which implies $V \leq c \sqrt{r}$ for some absolute constant $c$. Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log r} $,
\begin{equation} \label{matrix_perturbation_ineq2}
\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\| \leq C (\sqrt{\frac{\log n}{n}} + \frac{\log^2 n}{n})\leq C \sqrt{\frac{\log n}{n}}
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$. Here we use the fact that $r =O(1)$. 

For $\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bu_i^{T} \|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bff_i \bu_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall $\|\bff_i\| \sim \text{SG} (r c^2)$, and $\bu_i \sim \text{SG}_{d} (c_3^2)$ implies $\|\bu_i\| \sim \text{SG} (d c^2)$. Therefore $\|\bff_i \bu_i^{T}\|$ is sub-exponential with parameter $c^2\sqrt{dr}$, thus
\begin{equation*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) = \PP(\|\bff_i \bu_i^{T}\| \geq L) \leq 2n^{-11} :=q_0
\end{equation*}
if we take  $L= 22c^2 \sqrt{dr} \log n $. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bff_i\bu_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bff_i\bu_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2c^2\sqrt{dr}}}\mathrm{d} y + 2Le^{-\frac{L}{2c^2\sqrt{dr}}} \\
&= (4c^2\sqrt{dr}+2L) e^{-\frac{L}{2c^2\sqrt{dr}}}\\
& \leq 3L e^{-\frac{L}{2c^2\sqrt{dr}}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \max \{ \|\EE \bff_i \bu_i^{T} \bu_i \bff_i^{T} \|^{1/2} , \|\EE \bu_i \bff_i^{T} \bff_i \bu_i^{T} \|^{1/2} \} \\
&= \max \{ \|\EE  \bu_i^{T} \bu_i \EE \bff_i \bff_i^{T} \|^{1/2} , \|\EE \bu_i \bu_i^{T} \EE \bff_i^{T} \bff_i  \|^{1/2} \} \\
&= \max \{ \|\EE \| \bu_i\|^2 \bI_r \|^{1/2} , \|\EE \bu_i \bu_i^{T} r  \|^{1/2} \} \\
&\lesssim \max\{\sqrt{d}, \sqrt{r}\} \qquad (\|\bu_i\| \sim \text{SG} (d c^2), \|\EE \bu_i \bu_i^{T}\|=O(1))\\
& =\sqrt{d}
\end{align*}
Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log d} $,
\begin{equation} \label{matrix_perturbation_ineq3}
\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bu_i^{T}\| \leq C \sqrt{d} (\sqrt{\frac{ \log n}{n}} + \frac{\log^2 n}{n}) \leq C \sqrt{\frac{ d \log n}{n}}
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$.

For $\|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bu_i\bu_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall $\|\bu_i\| \sim \text{SG} (d c^2)$. Therefore 
\begin{align*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) & = \PP(\|\bu_i \bu_i^{T} - \EE[\bu_i \bu_i^{T}]\| \geq L) \\
&\leq \PP(\|\bu_i \bu_i^{T}\| +\| \EE[\bu_i \bu_i^{T}]\| \geq L) \\
& \leq \PP(\|\bu_i \bu_i^{T}\| \geq L-C) \qquad (\| \EE[\bu_i \bu_i^{T}]\| \leq C) \\
&\leq \PP(\|\bu_i\|^2 \geq L-C) \\
&= \PP(\|\bu_i\| \geq \sqrt{L-C})
\end{align*}
Take $L= 24c^2 d \log n + C$, by sub-Gaussian tail bound, we have $\PP(\|\bu_i\| \geq \sqrt{L-C}) \leq 2 n^{-12} :=q_0$. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bu_i\bu_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bu_i\bu_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty}  \PP(\|\bu_i\|^2 \geq y) \mathrm{d} y + L \PP (\|\bu_i\|^2 \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2dc^2}}\mathrm{d} y + 2Le^{-\frac{L}{2dc^2}} \\
&= (4dc^2+2L) e^{-\frac{L}{2rc^2}}\\
& \leq 3L e^{-\frac{L}{2dc^2}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. Here we use the fact that $n \geq d$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T} - (\EE \bu_i \bu_i^{T})^2\|^{1/2} \\
& \leq \|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}\|^{1/2}.
\end{align*}
The last inequality is due to the fact that $\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}-(\EE \bu_i \bu_i^{T})^2$ and $(\EE \bu_i \bu_i^{T})^2$ are both positive semidefinite. For $\|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}\|$, notice that for any $\bv \in \RR^d$ such that $\|\bv\|=1$, 
\begin{align*}
    \bv^{T} (\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}) \bv &= \EE [(\bu_i^{T} \bv)^2 \bu_i^{T} \bu_i] \\
    & \leq \sqrt{\EE (\bu_i^{T} \bv)^4 \EE (\bu_i^{T} \bu_i)^2 }  \qquad \text{(by Cauchy inequality)} \\
    & \leq c \sqrt{\EE \|\bu_i\|^4} \qquad \text{(since $\bu_i^{T} \bv \sim \text{SG}(c_3^2)$)} \\
    & \leq C d \qquad \text{(since $\|\bu_i\| \sim \text{SG}(c^2d)$)} 
\end{align*}
which implies $V \leq c \sqrt{d}$ for some absolute constant $c$. Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log d} $,
\begin{equation} \label{matrix_perturbation_ineq4}
\|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\| \leq C (\sqrt{\frac{d\log n}{n}} + \frac{d\log^2 n}{n})
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$. 

Finally, combine (\ref{matrix_perturbation_ineq1}), (\ref{matrix_perturbation_ineq2}), (\ref{matrix_perturbation_ineq3}), (\ref{matrix_perturbation_ineq4}), we have with probability $1-O(n^{-10})$
\begin{equation*}
    \|\hat{\bSigma}- \bSigma\| \lesssim \lambda_{1}^{*} \sqrt{\frac{\log n}{n}} + \sqrt{\frac{\lambda_{1}^{*}d \log n}{n}} + \sqrt{\frac{d \log n}{n}} + \frac{d \log^2 n}{n}
\end{equation*}
which is exactly what we want.
\end{proof}
\paragraph{Proof for Lemma \ref{approx_per_lemma}}
\begin{proof}
    Under Assumption \ref{approximate_perpendicularity}, 
\begin{align*}
    \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
    & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
    & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
\end{align*}
We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$. Notice that 
\begin{equation*}
\bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
\end{equation*}
This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
\begin{equation*}
     (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
\end{equation*}
for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$. Thus, we have 
\begin{equation*}
    \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
 \bLambda & &  \\
  & \bar{\bV} & \\
 & & 0
 \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T}
\end{equation*}
where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By pervasiveness condition, $\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} = \Omega(d)$, $\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| = O(1)$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma}) = \lambda_{r}(\bLambda) = \Omega (d)$, and $\lambda_{r+1}(\tilde{\bSigma})=\|\bar{\bV}\|=O(1)$. For $\|\bSigma- \tilde{\bSigma}\|$, we have 
\begin{align*}
    \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}]) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}) \\
    &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}].
\end{align*}
Recall $\bepsilon_i \sim \text{SG}_{d} (\sigma^2)$, which means for any $\bv \in \RR^d$ such that $\|\bv\|=1$, $\bv^{T}\bepsilon_{i} \sim \text{SG} (\sigma^2)$, thus
\begin{equation*}
    \bv^{T} \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \bv = \EE (\bv^{T}\bepsilon_{i})^2 \leq c \sigma^2.
\end{equation*}
Therefore $\|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\| \leq c\sigma^2$. We then have
\begin{align*}
    \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| + \|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\|  \\
    &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| +c\sigma^2 \\
    & \leq O(\|\bU^{T}\bM\| + \sigma^2).
\end{align*}
Therefore by Davis-Kahan (\ref{dist_U_Vr}), $\text{dist} (\bU, \bV_{r})  \leq O(\frac{\|\bU^{T}\bM\| + \sigma^2}{d}).$ By Assumption \ref{approximate_perpendicularity} and $\sigma \leq 1$, we have $O(\frac{\|\bU^{T}\bM\| + \sigma^2}{d}) \leq O ((\sigma/ \sqrt{d})\wedge (1/d))$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma/ \sqrt{d}) \times \Omega(\sqrt{d}) \\
    & \leq O(\sigma).
\end{align*}

For the second claim,
\begin{align*}
    &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
    &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
    &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
\end{align*}
Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, \shange{why this is true? need to mention $\bM$ is orthogonal. or write it in another way.} and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
\begin{align*}
   \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
   &\leq \|\bU^{T}\bM \balpha\| \\
   & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
   &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
\end{align*}
where the last inequality follows from Assumption \ref{approximate_perpendicularity}. Therefore 
\begin{align*}
    &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
    &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(1/ d) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(1/ d) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
\end{align*}
for some constant $c_2 > 0$. 

For the third claim, notice that by Weyl's inequality, 
\begin{align*}
     &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
     &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
     & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
     (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
     &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
\end{align*}
Notice that 
\begin{align*}
    &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
     (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
    & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
    & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
    & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
    & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
    &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
\end{align*}
Also,
\begin{align*}
    &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
    & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
    &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
    & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
    &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
    & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
    & \leq 4 C_3 O(\frac{1}{d}) =O(1)
\end{align*}
for sufficiently large $d$. Combine the above three inequalities, we have 
\begin{align*}
\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
\end{align*}
Therefore we proved Lemma \ref{approx_per_lemma}.
\end{proof}

\subsection{Proof for Lemma \ref{spectral_clustering_lemma}}
In this subsection we will briefly show why Lemma \ref{spectral_clustering_lemma} is a consequence of Corollary 3.1 in \cite{zhang2022leaveoneout}. 

We first claim that, although Theorem 3.1 and Corollary 3.1 in \cite{zhang2022leaveoneout} hold for spectral clustering with exact K-means, the results will actually hold for $(1+\epsilon)$-approximate K-means with only differences in constants. To see this, notice that in the proof of Proposition 3.1, \cite{zhang2022leaveoneout} claims that 
\begin{equation*}
    \|\hat{\Theta}-\hat{P}\|_{F} \leq \|P-\hat{P}\|_{F}
\end{equation*}
since $\hat{\Theta}$ is the solution to the exact K-means. However if $\hat{\Theta}$ is the solution to $(1+\epsilon)$-approximate K-means, we can similarly get 
\begin{equation*}
    \|\hat{\Theta}-\hat{P}\|_{F} \leq (1+\epsilon) \|P-\hat{P}\|_{F}.
\end{equation*}
Using this inequality will not affect the analysis except for several constants. As long as Proposition 3.1 still holds, the proofs of Theorem 3.1 will still remains the same.

Now it remains to show Lemma \ref{spectral_clustering_lemma} is a consequence of Corollary 3.1 in \cite{zhang2022leaveoneout} (with approximate K-means). Recall the definition of several quantities in \cite{zhang2022leaveoneout}: $\Delta=\min_{i \neq j}\|\btheta_i - \btheta_i\|$, $\beta=\frac{K}{n} \min_{j\in[K]} \{i:y_i \neq j\}$, $\lambda_K$ be the $K$-th singular value of data matrix $\bX$. Therefore we can see that, under our model, when $n$ is sufficiently large, with probability $1-o(1)$, $\beta \approx K \min_{j\in[K]}p_j $ which means $\beta=\Theta(1)$. Also $\Delta=\Theta(1)$, and $\lambda_K$ will scale with $\sqrt{n}$. Therefore we can see that when $d \leq O(n)$, the conditions in Corollary 3.1 in \cite{zhang2022leaveoneout} will be satisfied when $n$ is sufficiently large. Therefore Lemma \ref{spectral_clustering_lemma} is immediately implied.

\section{Proofs for Theorem \ref{thm2}}
The proofs for Theorem \ref{thm2} are similar to that of Theorem \ref{main_thm}. We also have $\hat{\bu}_{i}= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$. For the factor model estimation, Lemma \ref{matrix_perturbation_lemma} still applies. Recall Davis-Kahan theorem
\begin{equation*}
    \|\bDelta\| \leq \frac{\|\hat{\bSigma}- \bSigma\|}{\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)},
\end{equation*}
we will need to control $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)$.
We have $\bSigma = \bB \bB^{T} + \bSigma_u$, therefore by Weyl's ineqaulity, $|\lambda_{r}(\bSigma)-\lambda_{r}(\bB \bB^{T})| \leq \|\bSigma-\bB \bB^{T}\| = \|\bSigma_u\|$. Similarly $|\lambda_{r+1}(\bSigma)|= |\lambda_{r+1}(\bSigma)-\lambda_{r+1}(\bB \bB^{T})| \leq \|\bSigma-\bB \bB^{T}\| = \|\bSigma_u\|$. By Assumption \ref{weak_factor1}, $\lambda_{r}(\bB \bB^{T})= \sigma_{\min}^{2} (\bB) \geq 3 \|\bSigma_u\|$. Therefore $\lambda_{r}(\bSigma) \geq 2 \|\bSigma_u\|$, $\lambda_{r+1}(\bSigma) \leq \|\bSigma_u\|$, which implies $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) \geq \|\bSigma_u\| \geq c$ for some absolute constant $c$ (by Assumption \ref{regularity}). Therefore from Lemma \ref{matrix_perturbation_lemma} we get the following proposition for controlling $\|\bDelta\|$.
\begin{proposition} \label{matrix_perturbation_proposition2}
Under the conditions of Theorem \ref{weak_factor1}, we have
\begin{equation*}
\| \bDelta \| \leq O (\sqrt{\frac{d \log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}
Similar to Lemma \ref{approx_per_lemma}, we have the following:
\begin{lemma} \label{approx_per_lemma2}
Under Assumption \ref{regularity}, \ref{weak_factor1} and \ref{approximate_perpendicularity2}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma} 
With this lemma, we can prove Theorem \ref{thm2}. Similar to the proof for Theorem \ref{main_thm}, we have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (\sqrt{\frac{d \log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by Proposition \ref{matrix_perturbation_proposition2}). Similar to the proof for Theorem \ref{main_thm}, for $j_{1} \neq j_{2}$, 
\begin{equation*}
    \frac{c_2}{2} \|\bmu_{j_1} -\bmu_{j_2}\| \leq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \leq \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{equation*}




% For $j_{1} \neq j_{2}$, 
% \begin{equation*}
%     \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
% \end{equation*}

% On the other hand,
% \begin{align*}
%    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%    & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
%    &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma2}}) \\
%    & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (\sqrt{\frac{d \log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Proposition \ref{matrix_perturbation_proposition2}})\notag \\
%    & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
% \end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
    \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
\end{align*}
Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{d\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Proposition \ref{matrix_perturbation_proposition2}}) \\
    & \leq O (\sigma^2) +O(\frac{d\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma2}}) \\
    & \leq  O (\sigma^2) +O(\frac{d \log n}{n}) + \sigma^{2} \qquad (\text{By Assumption \ref{weak_factor1}})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{3}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. Similar to the proofs for Theorem \ref{main_thm}, Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$. Thus by applying Lemma \ref{spectral_clustering_lemma} we get the desired result.


% : the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma2}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
% \begin{align*}
%     & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
%      &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
%      &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
%      & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
%      & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
%      & \geq \frac{1}{2}c_3 - O(\sqrt{\frac{d\log n}{n}}) \notag \\
%      &\geq  \frac{1}{3}c_3.
% \end{align*}
% Then by Lemma \ref{spectral_clustering_lemma}, there exist constant $C$ and $c$ such that the following hold: \\
% 1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
% 2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
% \begin{equation*}
%     \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
% \end{equation*}
% Recall our definition for $\overline{\text{SNR}}$:  
% \begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
% \end{equation*}
% Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{thm2}.

\subsection{Proofs for Lemma \ref{approx_per_lemma2}}
\begin{proof}
We use the same notations as in the proofs for Lemma \ref{approx_per_lemma}. Then
% \begin{align*}
%     \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
%     & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
%     & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
%     &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
% \end{align*}
% We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$. Notice that 
% \begin{equation*}
% \bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
% \end{equation*}
% This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%      (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
% \end{equation*}
% for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$. Thus, we have 
% \begin{equation*}
%     \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
%  \bLambda & &  \\
%   & \bar{\bV} & \\
%  & & 0
%  \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T}
% \end{equation*}
% where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By Assumption \ref{weak_factor1}, $\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} \geq 3 \|\bSigma_u\|$, $\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| \leq \|\bSigma_u\|$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr2}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma})-\lambda_{r+1}(\tilde{\bSigma}) \geq 2 \|\bSigma_u\| \geq c_3$. For $\|\bSigma- \tilde{\bSigma}\|$, as in the proofs for Lemma \ref{approx_per_lemma},
% we have 
% \begin{align*}
%     \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}]) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}) \\
%     &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}].
% \end{align*}
% Recall $\bepsilon_i \sim \text{SG}_{d} (\sigma^2)$, which means for any $\bv \in \RR^d$ such that $\|\bv\|=1$, $\bv^{T}\bepsilon_{i} \sim \text{SG} (\sigma^2)$, thus
% \begin{equation*}
%     \bv^{T} \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \bv = \EE (\bv^{T}\bepsilon_{i})^2 \leq c \sigma^2.
% \end{equation*}
% Therefore $\|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\| \leq c\sigma^2$. We then have
% \begin{align*}
%     \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| + \|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\|  \\
%     &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| +c\sigma^2 \\
%     & \leq O(\|\bU^{T}\bM\| + \sigma^2).
% \end{align*}
$\|\bSigma- \tilde{\bSigma} \| \leq O(\|\bU^{T}\bM\| + \sigma^2)$. Therefore by Davis-Kahan (\ref{dist_U_Vr2}), $\text{dist} (\bU, \bV_{r})  \leq O(\|\bU^{T}\bM\| + \sigma^2).$ By Assumption \ref{approximate_perpendicularity2} and $\sigma \leq 1$, we have $O(\|\bU^{T}\bM\| + \sigma^2) \leq O(\sigma)$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma) \times \Omega(1) \\
    & \leq O(\sigma).
\end{align*}
The proofs for the second and the third claim are similar to that of Lemma \ref{approx_per_lemma}.
\end{proof}
% For the second claim,
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
%     &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
% \end{align*}
% Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
% \begin{align*}
%    \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
%    &\leq \|\bU^{T}\bM \balpha\| \\
%    & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
%    &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity2}. Therefore 
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(\sigma) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(\sigma) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
%      &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
%      & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%      &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%     & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
%     & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
%     & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
%     & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity2}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
%     & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
%     &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
%     & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
%     &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
%     & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
%     & \leq 4 C_3 O(\sigma) =O(1).
% \end{align*}
% Combine the above three inequalities, we have 
% \begin{align*}
% \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
% \end{align*}
% Therefore we proved Lemma \ref{approx_per_lemma2}.
% \end{proof}

\section{Proofs for Theorem \ref{thm3}}
The proofs for Theorem \ref{thm3} are similar to that of Theorem \ref{main_thm}. Under Assumption \ref{weak_factor2}, we also have $\lambda_{r}(\bB \bB^{T})= \sigma_{\min}^{2} (\bB) \geq 3 \|\bSigma_u\|$, therefore  $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) \geq \|\bSigma_u\| \geq c$ still applies. Combining Lemma \ref{matrix_perturbation_lemma}, we get the following proposition for controlling $\|\bDelta\|$.
\begin{proposition} \label{matrix_perturbation_proposition3}
Under the conditions of Theorem \ref{weak_factor2}, we have
\begin{equation*}
\| \bDelta \| \leq O (d\sqrt{\frac{\log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}
Similar to Lemma \ref{approx_per_lemma}, we have the following:
\begin{lemma} \label{approx_per_lemma3}
Under Assumption \ref{regularity}, \ref{weak_factor1} and \ref{approximate_perpendicularity2}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma} 
With this lemma, we can prove Theorem \ref{thm3}. We have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (d\sqrt{\frac{\log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by Proposition \ref{matrix_perturbation_proposition}). For $j_{1} \neq j_{2}$, 
\begin{equation*}
    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
\end{equation*}
On the other hand,
\begin{align*}
   \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
   & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
   &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma3}}) \\
   & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (d\sqrt{\frac{ \log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Proposition \ref{matrix_perturbation_proposition3}})\notag \\
   & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. The last equality use the assumption that $d^3 \leq O(\frac{n}{(\log n)^{3}})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
% \begin{align*}
%     \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
%     &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
% \end{align*}
% Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, 
we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Therefore
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{d^2\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Proposition \ref{matrix_perturbation_proposition3}}) \\
    & \leq O (\sigma^2) +O(\frac{d^2\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma3}}) \\
    & \leq  O (\sigma^2) +O(\frac{d^3 \log n}{n}) + \sigma^{2} \qquad (\text{By Assumption \ref{weak_factor2}})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d^3 \leq O ( \frac{n}{(\log n)^{3}}) )
\end{align*}
% Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. 
Similar to the proofs for Theorem \ref{main_thm}, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. The only thing remains is to verify that Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$: the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma3}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
\begin{align*}
    & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
     &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
     &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
     & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
     & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
     & \geq \frac{1}{2}c_3 - O(d\sqrt{\frac{\log n}{n}}) \notag \\
     &\geq  \frac{1}{3}c_3.
\end{align*}
The last inequality uses the assumption that $d^3 \leq O(\frac{n}{(\log n)^3})$. By Lemma \ref{spectral_clustering_lemma}, we get the desired result.

% there exist constant $C$ and $c$ such that the following hold: \\
% 1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
% 2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
% \begin{equation*}
%     \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
% \end{equation*}
% Recall our definition for $\overline{\text{SNR}}$:  
% \begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
% \end{equation*}
% Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{thm3}.

\subsection{Proofs for Lemma \ref{approx_per_lemma3}}
\begin{proof}
The proof is similar to that of Lemma \ref{approx_per_lemma} with slight differences. Recall
\begin{align*}
    \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
    & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
    & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \sigma^2 \bI_d.
\end{align*}
We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} + \sigma^2 \bI_d$. 
% Notice that 
% \begin{equation*}
% \bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
% \end{equation*}
% This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%      (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
% \end{equation*}
% for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$.
Similar to the proof for Lemma \ref{approx_per_lemma} (with an additional term), we have 
\begin{equation*}
    \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
 \bLambda & &  \\
  & \bar{\bV} & \\
 & & 0
 \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T} + \sigma^2 \bI_d
\end{equation*}
where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By Assumption \ref{weak_factor1}, $\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} \geq 3 \|\bSigma_u\|$, $\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| \leq \|\bSigma_u\|$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr3}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma})-\lambda_{r+1}(\tilde{\bSigma}) \geq 2 \|\bSigma_u\| \geq c_3$. For $\|\bSigma- \tilde{\bSigma}\|$, we have 
\begin{align*}
    \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \sigma^2 \bI_d) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} + \sigma^2 \bI_d) \\
    &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}.
\end{align*}
We then have
\begin{align*}
    \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
    &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| \\
    & \leq O(\|\bU^{T}\bM\|).
\end{align*}
Therefore by Davis-Kahan (\ref{dist_U_Vr3}), $\text{dist} (\bU, \bV_{r})  \leq O(\|\bU^{T}\bM\|).$ By Assumption \ref{approximate_perpendicularity3}, we have $O(\|\bU^{T}\bM\|) \leq O(\sigma/\sqrt{d})$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma/\sqrt{d}) \times \Omega(\sqrt{d}) \\
    & \leq O(\sigma).
\end{align*}
The proofs for the second and the third terms are similar to that of Lemma \ref{approx_per_lemma}.
% For the second claim,
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
%     &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
% \end{align*}
% Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
% \begin{align*}
%    \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
%    &\leq \|\bU^{T}\bM \balpha\| \\
%    & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
%    &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity3}. Therefore 
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(\sigma/\sqrt{d}) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(\sigma/\sqrt{d}) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
%      &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
%      & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%      &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%     & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
%     & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
%     & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
%     & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity3}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
%     & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
%     &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
%     & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
%     &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
%     & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
%     & \leq 4 C_3 O(\sigma/\sqrt{d}) =O(1).
% \end{align*}
% Combine the above three inequalities, we have 
% \begin{align*}
% \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
% \end{align*}
% Therefore we proved Lemma \ref{approx_per_lemma3}.
\end{proof}

==> texfiles/old/proof_sketch_thm_1.tex <==
\section{Proof sketch of \prettyref{thm:2}}
In this subsection, we briefly characterize the intuition of proving Theorem \ref{main_thm}. For simplicity, we assume Assumption \ref{regularity} and (\ref{strict_perpendicularity}) hold "strictly". The detailed proof under Assumption \ref{approximate_perpendicularity} will be presented in the Appendix. Our proof strategy has two phases: in the first phase, we show that our estimator $\hat{\bu}_{i}$ can be written as $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$,
where $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise; in the second phase, we apply the result for spectral clustering with small sub-Gaussian noise.
\paragraph{First phase: decomposing the estimator}
For the first phase, 
\begin{align*}
	\hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i}  \\
	&= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) (\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})  \\
	&= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{y_{i}} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
	&:= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{align*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}$. Let $\bDelta:=\bV_{r}\bV_{r}^{T} -\hat{\bV}_{r}\hat{\bV}_{r}^{T}$, by matrix perturbation theory, we have $\|\bDelta\| \leq O (\sqrt{\frac{\log n}{n}})$ with a high probability (Proposition \ref{matrix_perturbation_proposition}). Then we have for $j_{1} \neq j_{2}$, 
\begin{align*}
	\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\| &= \| (I-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \|  \\
	& \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \\
	&= \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \quad (\text{By (\ref{strict_perpendicularity})}) \\
	& \geq \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta\| \| \boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| \notag \\
	& \geq \frac{1}{2} \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\|.
\end{align*}
For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
	\tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
	&= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}  \\
	&= 0 + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \quad (\text{By (\ref{strict_perpendicularity})}) 
\end{align*}
Notice that $\bff_{i} \sim \text{SG}_{r} (c_1^2) $, $\bepsilon_{i} \sim \text{SG}_{d} (\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
	\|\bDelta \bB\|^{2} + \sigma^{2} & \leq \|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
	& \leq O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \quad (\text{By proposition \ref{matrix_perturbation_proposition}}) \notag \\
	& \leq  O(\frac{d \log n}{n}) + \sigma^{2} \quad (\text{By Assumption \ref{pervasiveness}}) \notag \\
	& \leq O(\frac{1 }{\log n}) + \sigma^{2}  \quad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{2}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq O (\frac{1}{\log n})$, we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\sigma^{2})$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (O (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$. Which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise.

\paragraph{Second phase: general results for spectral clustering}
For the second phase, we apply the general results for spectral clustering. Suppose we now have data from the following model: 
\begin{align} \label{spectral_clustering_model}
	&\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
	&\bx_{i} = \btheta_{y_{i}} + \bepsilon_{i},
\end{align}
where $y_{i}$ is the true label, $\{\btheta_{j}\}_{j=1}^{K}$ is the set of true clustering centers, and $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$ is independent from all other quantities. The signal-to-noise ratio in this model is defined as 
\begin{equation*}
	\widetilde{\text{SNR}} := \frac{\min_{i\neq j}\|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\|^{2}}{\sigma^2}.
\end{equation*}
We have the following theoretical guarantee for spectral clustering (Algorithm \ref{alg2}), which is a direct consequence of Corollary 3.1 in \cite{zhang2022leaveoneout} with a slight modification (here we use $(1+\epsilon)$-approximate $K$-means).
% (Theorem 3.1 in \cite{abbe2022ellp}): 
\begin{lemma}\label{spectral_clustering_lemma}
	Consider the model defined in (\ref{spectral_clustering_model}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg2}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumption \ref{regularity} holds, and $d \leq O (n)$, then there exist constant $C$ and $c$ such that the following hold:
	
	\begin{enumerate}[label=(\alph*)]
		\item If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.
		
		\item If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$.
	\end{enumerate}
\end{lemma}
% See the appendix for the proof of Lemma \ref{spectral_clustering_lemma}. Notice that similar results are already given in many spectral clustering literature, but their proof is usually complicated, due to the fact that $\hat{V}$ is not independent with $\boldsymbol{x}_{i}$. Here we resolve this problem by using the "cross-validation" type algorithm, thus our analysis is much simpler.
Applying Lemma \ref{spectral_clustering_lemma} on $\{\hat{\boldsymbol{u}}_{i}\}_{i=1}^{n}$ will finish the proof for Theorem \ref{main_thm}.  

\begin{remark}
	Notice that the proofs for Lemma \ref{spectral_clustering_lemma} or similar results are very complicated (see \cite{abbe2022ellp,zhang2022leaveoneout}), due to the fact that $\hat{\bV}$ is not independent with $\bx_{i}$. We can resolve this problem by splitting the data to facilitate an easier analysis of spectral clustering algorithm. See Appendix \ref{cv} for further details.
\end{remark} 


==> texfiles/old/realdata.tex <==
\section{Real data analysis}
In this section, we apply FASC on real datasets.
\subsection{Mice protein expression}
We analyze the mice protein expression data from UCI Machine Learning Repository:\\ \url{https://archive.ics.uci.edu/ml/datasets/Mice+Protein+Expression}.\\
The dataset consists of the expression levels of 77 proteins measured in the cerebral cortex of 8 classes of control (which we view as the true class label), containing a total of 1080 measurements per protein. Each measurement can be considered as an independent sample. We first cleaned the missing values by dropping 6 columns “BAD\_N”, “BCL2\_N”, “pCFOS\_N”, “H3AcK18\_N”, “EGR1\_N”, “H3MeK4\_N” and then removing all rows with at least 1 missing value. After data cleaning and centralization, we get a dataset of 1047 samples each having 71 attributes. We then apply the k-means clustering, spectral clustering and FASC to the unlabeled dataset with the number of clusters $K=8$. We compare the clustering results to the true class labels and calculate the misclassification rate. The results of clustering are stated in the second column of Table \ref{table1}, where FASC with $r=1$ or $2$ performs much better than k-means and spectral clustering. However, for larger $r$, the performance of FASC is not better than k-means or spectral clustering.
\begin{table}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|p{5cm}|p{5cm}|p{5cm}|}
    \hline
    \textbf{Clustering algorithm} & \textbf{Misclassification rate for mice protein expression data} & \textbf{Misclassification rate for DNA codon usage frequencies data} \\
    \hline
    k-means & 0.659 & 0.610 \\ 
    \hline
    spectral clustering & 0.657 & 0.608 \\
    \hline
    FASC(r=1) & 0.538 & 0.507  \\
    \hline
    FASC(r=2) & 0.569 & 0.565 \\
    \hline
    FASC(r=3) & 0.666 & 0.630 \\
    \hline
    FASC(r=4) & 0.645 & 0.700 \\
    \hline
    Baseline(random guess) & 0.875 & 0.875 \\
    \hline
  \end{tabular}%
  }
\caption{Misclassification rate for different methods on mice protein expression data and DNA codon usage frequencies data}
  \label{table1}
\end{table}

This phenomenon can be explained by the spectral structure of this dataset. We draw the scree plot Figure \ref{scree_plot_1} which shows the eigenvalues of the dataset arranged in descending order. It is obvious that the first two eigenvalues are significantly larger than others, suggesting that there may exist two significant factors.  Therefore it is appropriate to do factor adjustment on this dataset with the number of factors $r=1$ or $2$, justifying the result that FASC performs well with $r=1$ or $2$.
\begin{figure}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{Scree plot.png}
  \caption{Scree plot of mice protein expression data}
  \label{scree_plot_1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{DNA codon frequency scree plot.png}
  \caption{Scree plot of DNA codon frequency data}
  \label{scree_plot_2}
\end{subfigure}
}
\caption{Scree plot}
\label{scree_plot}
\end{figure}
\subsection{DNA codon usage frequencies}
We analyze the DNA codon usage frequencies data from UCI Machine Learning Repository:\\ \url{https://archive.ics.uci.edu/dataset/577/codon+usage}.\\
The dataset consists of codon usage frequencies in the genomic coding DNA of a large sample of diverse organisms from different taxa tabulated in the CUTG database. Each sample has 64 attributes that are the codon (including 'UUU', 'UUA', 'UUG', 'CUU', etc) frequency. The data are classified by their kingdom (which we view as the true class label): 'bct'(bacteria), 'pln' (plant), 'inv' (invertebrate), 'vrt' (vertebrate), 'mam' (mammal), 'rod' (rodent), 'pri' (primate) and 'vrl'(virus) ('arc','phg','plm' are removed since the number of samples are very small). After data cleaning, we get a dataset of 12135 samples with 64 attributes. We apply the k-means clustering, spectral clustering and FASC to the centralized unlabeled dataset with the number of clusters $K=8$. We compare the clustering results to the true class label and calculate the misclassification rate. The results of clustering are stated in the third column of Table \ref{table1}, where FASC with $r=1$ or $2$ performs much better than k-means and spectral clustering.
% \begin{table}
%   \centering
%   \resizebox{0.8\textwidth}{!}{%
%   \begin{tabular}{|c|c|}
%     \hline
%     \textbf{Method} & \textbf{Misclassification rate}  \\
%     \hline
%     k-means & 0.610  \\
%     \hline
%     spectral clustering & 0.608  \\
%     \hline
%     FASC(r=1) & 0.507  \\
%     \hline
%     FASC(r=2) & 0.565  \\
%     \hline
%     FASC(r=3) & 0.630  \\
%     \hline
%     FASC(r=4) & 0.700  \\
%     \hline
%     Baseline(random guess) & 0.875  \\
%     \hline
%   \end{tabular}%
%   }
% \caption{Misclassification rate for different methods on DNA codon usage frequencies data}
%   \label{table2}
% \end{table}
Similar to the mice protein expression analysis, this phenomenon can also be explained by the spectral structure. In the scree plot Figure \ref{scree_plot_2}, the first two eigenvalues are significantly larger than others. 
% \r{Q: Do we know the true label?  Do we do data splitting?  Do we split data into training and validation part?}


==> texfiles/old/setup.tex <==
\section{Problem setup}
\noindent\textbf{Notation:}  Let $\|\cdot\| $ be the $\ell_2$ norm of a vector or the spectral norm of a matrix. We denote by $\|\cdot\|_{\rF}$ the Frobenius norm of a matrix. For a matrix $\bM\in\R^{m\times n}$, we denote by $\sigma_{\min}(\bM)$ and $\sigma_{\max}(\bM)$ the smallest non-zero singular value and the largest singular value of $\bM$, respectively. Moreover, for a symmetric matrix $\bA \in \R^{m\times m}$,  we denote by $\lambda_{\min}(\bA)$ and $\lambda_{\max}(\bA)$ the smallest non-zero eigenvalue and the largest eigenvalue of $\bA$, respectively.
% $\mathcal{N}(\bmu,\bSigma)$ refers to the normal distribution with mean $\mu$ and covariance matrix $\bSigma$.
For a random variable $X$, we say $X$ is sub-Gaussian with parameter $\sigma^{2}$ (denoted as $X \sim \text{SG}(\sigma^{2})$) if $\mathbb{E}e^{tX} \leq e^{\frac{1}{2}\sigma^{2}t^{2}}$ for any $t \in \mathbb{R}$. For a random vector $\bX \in \mathbb{R}^{d}$, we say $\bX$ is sub-Gaussian with parameter $\sigma^{2}$ (denoted as $\bX \sim \text{SG}_{d}(\sigma^{2})$), if $\bv^{T}\bX \sim \text{SG}(\sigma^{2})$ holds for any unit vector $\bv \in \mathbb{R}^{d}$. We use $c,C$ to denote some absolute constants that may differ from line to line.


% We use $\tilde{\mathcal{O}}(\cdot)$ and $\tilde{\Omega}(\cdot)$ notation to hide polylogarithmic factors. The use of $\mathcal{O}$, $\Omega$ and $\Theta$ is standard.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Mixture model with factor structure} \label{section_factor}

% \shange{rewrite the model!!!}
In this paper, we assume that data $\{(\bx_{i},y_{i})\}_{i=1}^{n}\subset \mathbb{R}^{d} \times \mathbb{R}$  are i.i.d. sampled from the following mixture model:
\begin{align} \label{factor_cluster}
    &\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
    &\bx_{i}= \bmu_{y_{i}} + \be_{i} \quad \mbox{with} \quad \be_{i}=\bB\bff_{i}+\bepsilon_{i}.
\end{align}
where $y_{i}$ is the unobserved true label, $\{\bmu_{j}\}_{j=1}^{K}$ is the set of true cluster centers, $\bB \in \mathbb{R}^{d \times r}$ is a fixed factor loading matrix, $\bff_{i}$ is a mean-zero latent factor independent from $y_{i}$, and $\bepsilon_{i}$ is a mean-zero noise independent from all other quantities. Without a loss of generality, we assume $\cov (\bff_i)=\bI_r$ and $\mathbb{E}[\bx_{i}]=0$, i.e., $\sum_{j=1}^{K}p_{j}\boldsymbol{\mu}_{j} = 0$ (when the mean is not zero, we can first centralize the data, which will not make much difference). We further assume $\bff_i \sim \text{SG}_{r}(c_1^2)$ for some absolute constant $c_1$, and $\bepsilon_i \sim \text{SG}_{d}(\sigma^2)$ where $\sigma^2 \leq 1$ is the noise level.
% We can see that for each $j \in [K]$, $\boldsymbol{x}_{i}$ such that corresponds to $y_{i}=j$ follows a Gaussian distribution $\mathcal{N}(\boldsymbol{\mu}_{j}, \bB\bB^{T}+\sigma^{2}I_{d})$. The marginal distribution $\boldsymbol{x}_{i} \sim \sum_{j=1}^{K} p_{j} \mathcal{N}(\boldsymbol{\mu}_{j}, \bB\bB^{T}+\sigma^{2}I_{d})$ is from a Gaussian Mixture Model with the same stretched covariance for each cluster.
By defining $\bu_{i}=\bmu_{y_{i}} + \bepsilon_{i}$, our model can be equivalently stated as $\bx_{i}=\bB\bff_{i}+\bu_{i}$. 

Throughout this paper, we consider the scenario that the number of factors $r$ and the number of clusters $K$ are constants that do not scale with $n$ or $d$. On the contrary, the number of samples $n$ and the dimension $d$ can go to infinity. 

% As often assumed in related literature(see \cite{fan2021robust} for discussion), we assume our factor model has the so called ``pervasiveness" condition, that is, there exist constants $c,C$, such that
% $c\sqrt{d} \leq \sigma_{\min}(\bB) \leq\sigma_{\max}(\bB) \leq C\sqrt{d}$. And the scaling of $\boldsymbol{u}_{i}$ is $O(1)$, that is, $\max_{i,j\in [K]}\|\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j}\| = O(1)$, $\sigma^2= O(1)$. This condition enable us to learn the factor properly.


\paragraph{Misclassification rate}
For any estimated class labels $\{\hat{y}_{i}\}_{i=1}^{n}$, there are permutation ambituities in estimating the true class labels $\{y_i\}_{i=1}^n$. The misclassification rate is thus defined as
\begin{equation*}
    \mathcal{M}(\hat{\by}, \by)=n^{-1} \min _{\tau \in S_K}\left|\left\{i \in[n]: \hat{y}_i \neq \tau\left(y_i\right)\right\}\right| .
\end{equation*}
where $S_K$ is the set of all permutations of $[K]$. Our goal is to design an efficient algorithm that recovers $\{y_{i}\}_{i=1}^{n}$ from the unlabeled data $\{\bx_{i}\}_{i=1}^{n}$ with a small misclassification rate $\mathcal{M}(\hat{\by}, \by)$. 

\paragraph{Signal-to-noise ratio} \label{signal_to_noise}
\shange{Move this Signal-to-noise ratio section to introduction}
The signal-to-noise ratio (SNR) plays a central role in clustering problems. We define $\text{SNR}:=\min_{i\neq j} (\bmu_{i}-\bmu_{j})^{T} (\bB\bB^T + \sigma^2 \bI_d)^{-1}(\bmu_{i}-\bmu_{j})$. A related quantity is defined as
$\text{S} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\|\bB\bB^T + \sigma^2 \bI_d\|}$. Also, the "S" correspond to $\bu_i$ is defined as $\overline{\text{SNR}}:= \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2}$,  which can also be viewed as a factor-adjusted version of SNR. It then follows that $\text{S} \leq \text{SNR} \leq \overline{\text{SNR}}$. Figure \ref{SNR vs barSNR vs S} plots these quantities with respect to different noise level $\sigma$, showing that SNR and $\overline{\text{SNR}}$ can be significantly larger than S. 
% Our proposed algorithm FASC (Algorithm \ref{alg1}) will achieve a misclassification rate $e^{-\Omega(\overline{\text{SNR}})}$, while spectral clustering (Algorithm \ref{alg2}) can only achieve $e^{-\Omega(\text{S})}$.

% $(\bmu_{1}-\bmu_{2})^{T} (\bB\bB^{T}+\sigma^{2}\bI_{d})^{-1}(\boldsymbol{\mu}_{1}-\boldsymbol{\mu}_{2})$, which is upper bounded by $\|(\boldsymbol{\mu}_{1}-\boldsymbol{\mu}_{2})\|^{2}\lambda_{\min}^{-1}(\bB \bB^{T}+\sigma^{2}\bI_{d})$ and equals to  $\frac{1}{\sigma^{2}}\|(\boldsymbol{\mu}_{1}-\boldsymbol{\mu}_{2})\|^{2}$ when number of factors $r < d$.  For multiple clusters setting, the SNR is naturally generalized to
% \begin{equation} \label{SNR}
%     \text{SNR} :=\min_{i\neq j} (\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j})^{T} (\bB\bB^{T}+\sigma^{2}\bI_{d})^{-1}(\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j}) \leq \frac{\min_{i\neq j}\|(\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j})\|^{2}}{\sigma^2} :=\overline{\text{SNR}}.
% \end{equation}
% When the span of $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ is approximately perpendicular to the column space span of $\bB$ (which is usually true in high dimensional scenarios, as Lemma \ref{justify_approx_perp_lemma} will show), SNR is in fact close to $\overline{\text{SNR}}$, and the optimal misclassification rate $e^{-\Omega(\overline{\text{SNR}})}$ can be achieved. For comparison, we can also define 
% $\text{S} := \frac{\min_{i\neq j}\|(\boldsymbol{\mu}_{i}-\boldsymbol{\mu}_{j})\|^{2}}{\|(\bB\bB^{T}+\sigma^{2}\bI_{d})\|}$.
% It is then follows that $\text{S} \leq \text{SNR} \leq \overline{\text{SNR}}$. Figure \ref{SNR vs barSNR vs S} plots these quantities with respect to different noise level $\sigma$, showing that SNR and $\overline{\text{SNR}}$ can be significantly larger than $S$.
% For a numerical comparison of these quantities, see Figure \ref{SNR vs barSNR vs S}, where we plot SNR, $\overline{\text{SNR}}$ and S with respect to noise level $\sigma$.  In Figure \ref{SNR vs barSNR vs S}, we can see that, S is very close to $0$, while SNR and $\overline{\text{SNR}}$ can be significantly larger than $S$.
\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{SNR vs barSNR vs S.png}
    \caption{Comparison of $\text{S} \leq \text{SNR} \leq \overline{\text{SNR}}$ for two-clusters Gaussian mixture model with  $d=100$, $r=3$. For $t=1,2,\cdots,100$, we generate the factor loading matrix $\bB\in \mathbb{R}^{d \times r}$ whose rows are drawn from i.i.d. $\mathcal{N}(0,I_{r})$; generate the true cluster center $\boldsymbol{\mu}$ by drawing $\boldsymbol{\mu}$ from i.i.d. $\mathcal{N}(0,\frac{1}{d}I_{d})$ ; finally we set the noise level $\sigma= 0.01t$. Therefore we have $100$ different models and  compute its associated SNR, $\overline{\text{SNR}}$ and $S$ for each model. The averages based on 1000 simulations are plotted in the figure.}
    \label{SNR vs barSNR vs S}
\end{figure}
% As discussed in related work, previously mentioned efficient algorithms that have optimal sample complexity $n=\tilde{\Omega}(d)$, can only achieve the sub-optimal misclassification rate $e^{-\Omega(\text{S})}$. The goal of our paper is to develop an efficient algorithm that achieves both optimal misclassification rate and optimal sample complexity at the same time under our structural assumption.
\subsection{Spectral clustering}
Spectral clustering (Algorithm \ref{alg2}) aims to reduce the noise and facilitate the computation by projecting the data onto a low-dimensional subspace spanned by the true cluster centers.
% The idea of spectral clustering is simple. Notice that the number of clusters $K$ is assumed to be $O(1)$, which is much smaller than the dimension $d$. Also, the dimension $k$ of the subspace spanned by cluster centers may be even smaller. Therefore, if we project the data onto the subspace spanned by the true cluster centers, then we can reduce this problem from dimension $d$ to $k$. In this way, the noise will be reduced and the computation will also be easier.In spectral clustering, the projection onto the desired subspace is calculated through singular value decomposition (SVD). 
After projection, $K$-means is conducted to get the estimated labels. Notice that exact $K$-means is not computationally efficient, here we instead use $(1+\epsilon)$-approximate $K$-means where a linear-time algorithm exists for solving it  \citep{Kumar2004ASL}.
\begin{algorithm}[H]
\caption{Spectral clustering}\label{alg2}
\begin{algorithmic}[1]
\State {\bf Input:} $\{\boldsymbol{x}_i\}^{n}_{i=1}$. The number of clusters $K$, target dimension of embedding $k$.
\State Compute
\begin{equation*}
    \hat{\bV}:=(\bxi_{1},\cdots,\bxi_{k}),
\end{equation*}
where $\bxi_{1},\cdots,\bxi_{k}$ are the top $k$ right singular vectors of $(\bx_{1},\cdots,\bx_{n})^{T} $.

\State Conduct $(1+\epsilon)$-approximate $K$-means on $\{\hat{\bV}^{T}\bx_{i}\}_{i=1}^{n}$, getting $\{\hat{y}_{i}\}_{i=1}^{n}$ and $\{\hat{\boldsymbol{\mu}}_{j}\}_{j=1}^{K}$ such that:
\begin{equation*}
    \sum_{i=1}^n\|\hat{\bV}^{T}\bx_{i}-\hat{\boldsymbol{\mu}}_{\hat{y}_i}\|_2^2 \leq(1+\epsilon) \min _{\substack{\{\widetilde{\boldsymbol{\mu}}_j\}_{j=1}^K \subseteq \mathbb{R}^k \\\left\{\widetilde{y}_i\right\}_{i=1}^n \subseteq[K]}}\{\sum_{i=1}^n\|\hat{\bV}^{T}\bx_{i}-\widetilde{\boldsymbol{\mu}}_{\tilde{y}_i}\|_2^2\} .
\end{equation*}


\State {\bf Output:} $\{\hat{y}_{i}\}_{i=1}^{n}$.
\end{algorithmic}
\end{algorithm}
However, this algorithm may fail \shange{give a simulation or reference of proof} when S is small, even when SNR is large, as the following example illustrates. 
% Take $\sigma^{2}=1$, $\bB = (100,0)^{T}$, $\bmu_{1}=(0,3)^{T},$ $\bmu_{2}=(0,-3)^{T}$, and $p_1=p_2=1/2.$ Then
Let $\bx_{i} \sim  
\frac{1}{2}\mathcal{N}((0,3)^{T}, \bSigma) + \frac{1}{2}\mathcal{N}((0,-3)^{T}, \bSigma)$
 where $\bSigma = \begin{pmatrix}
 10001 & 0 \\
 0 & 1 
 \end{pmatrix}$.
In this case, the space spanned by the true clustering centers is $span\{(0,1)^{T}\}$. But when we apply Algorithm \ref{alg2}, the right singular vector corresponding to the largest eigenvalue of $\bX = (\bx_1, \cdots, \bx_n)^{T}$ will approximately be $span\{(1,0)^{T}\}$ and we project the data in a wrong direction, which leads to the failure of spectral clustering.
% The failure of spectral clustering in the above example is that while projection directions are demonated by the singular vector of the covariance matrix $\bSigma$ rather than the subspace spanned by the true cluster centers and these two spaces can even be nearly orthogonal.  As a result, the performance of the traditional spectral clustering algorithm can be very poor.  
This phenomenon will often occurs when the covariance matrix $\bSigma$ has some spiked components which do not align with the subspace spanned by the true cluster centers.
To remedy this, we propose the Factor-Adjusted Spectral Clustering (\prettyref{algo:1}) to remove the spiked component in the covariance matrix.


% $\bB=\begin{pmatrix}
% 1 & 2 & 3\\
% a & b & c
% \end{pmatrix}$

% \r{Q:  I edit up to here, spending a lot of time already.  The writing seems like a student's homework, rather than an expert writing a scientific paper}



==> texfiles/old/simulation.tex <==
\section{Simulation study}

In this section, we are going to justify our theory by several simulation experiments. 

\subsection{GMM with factor structure}

% \shange{for model r=3, do algorithm r=1,2,3,4,5}

% \shange{in experiment, do several times for each sigma}
In the following simulations, we generate samples from the model (\ref{factor_cluster}) with the number of clusters $K=5$, the number of factors $r=3$, and each cluster has equal weight (i.e., $p_{j}=1/K$). To be specific, for $t=1,2,\cdots,100$, we generate the factor
loading matrix $\bB\in \mathbb{R}^{d \times r}$ whose rows are drawn from i.i.d. $\mathcal{N}(0,\bI_{r})$; generate the true cluster centers $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ by drawing $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$ from i.i.d. $\mathcal{N}(0,\frac{1}{d}\bI_{d})$ and let $\boldsymbol{\mu}_{j} = \boldsymbol{\theta}_{j} - \frac{1}{K}\sum_{i=1}^{K}\boldsymbol{\theta}_{i}$; finally we set the noise level $\sigma= 0.01t$. Therefore we have $100$ different models, and for each model, we generate $n$ samples by generating class label $y_{i} \sim \text{Uniform}([K])$, latent factor $\bff_{i} \sim \mathcal{N}(0,\bI_{r})$ and noise $\bepsilon_{i} \sim \mathcal{N}(0,\sigma^{2}\bI_{d})$. We then perform FASC (Algorithm \ref{alg1}) and vanilla spectral clustering (Algorithm \ref{alg2}) on these generated data and compare these two methods.  
% \r{Q: Try to reduce repetitions.  Do you use data splitting?  Probably, we can include both with and without splitting}.

\noindent \textbf{Remark:} The models we randomly generated will satisfy Assumption \ref{regularity} and  \ref{pervasiveness} with high probability. Assumption \ref{approximate_perpendicularity} will be satisfied with high probability for large $d$.

% For the "pervasiveness" condition, the generating process of $B$ will result in $B$ scales with $\sqrt{d}$, and the generating process of $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ will result in each $\|\boldsymbol{\mu}_{j}\|$ scales with $\Omega(1)$. For the "approximate perpendicularity" assumption \ref{approximate_perpendicularity}, notice that we have claimed that Assumption \ref{approximate_perpendicularity} will hold with high probability if we choose the subspace of $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ uniformly and randomly which is what we have done. 
In Figure \ref{FASC VS Spectral clustering}, we plot the misclassification rate of FASC (red points) and spectral clustering (blue points) with respect to $\sigma$. Figure \ref{d=5_n=1000_K=5_r=3}, \ref{d=10_n=1000_K=5_r=3}, \ref{d=20_n=1000_K=5_r=3}, \ref{d=100_n=1000_K=5_r=3}, \ref{d=500_n=1000_K=5_r=3}, \ref{d=1500_n=1000_K=5_r=3} show the result of sample size $n=1000$, and $d=5,10,20,100,500,1500$ respectively.
\begin{figure}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=5, n=1000, K=5, r=3.png}
    \caption{d=5, n=1000, K=5, r=3}
    \label{d=5_n=1000_K=5_r=3}
\end{subfigure}
    \hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=10, n=1000, K=5, r=3.png}
    \caption{d=10, n=1000, K=5, r=3}
    \label{d=10_n=1000_K=5_r=3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=20, n=1000, K=5, r=3.png}
    \caption{d=20, n=1000, K=5, r=3}
    \label{d=20_n=1000_K=5_r=3}
\end{subfigure} 
}
\vspace{0.1cm}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=100, n=1000, K=5, r=3.png}
    \caption{d=100, n=1000, K=5, r=3}
    \label{d=100_n=1000_K=5_r=3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=500, n=1000, K=5, r=3.png}
    \caption{d=500, n=1000, K=5, r=3}
    \label{d=500_n=1000_K=5_r=3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=1500, n=1000, K=5, r=3.png}
    \caption{d=1500, n=1000, K=5, r=3}
    \label{d=1500_n=1000_K=5_r=3}
\end{subfigure}}


\caption{FASC VS Spectral clustering}
\label{FASC VS Spectral clustering}
\end{figure}
From Figure \ref{FASC VS Spectral clustering}, it can be seen that vanilla spectral clustering performs like a random guess with a misclassification rate close to $0.8$, regardless of the noise level, justifying the failure of spectral clustering for highly correlated data. On the contrary, in Figure \ref{d=20_n=1000_K=5_r=3}, \ref{d=100_n=1000_K=5_r=3}, \ref{d=500_n=1000_K=5_r=3}, \ref{d=1500_n=1000_K=5_r=3}, FASC achieves exact recovery (misclassification rate is $0$) when $\sigma$ is small. When $\sigma$ grows, the misclassification rate of FASC grows until it reaches the benchmark of spectral clustering. The simulation results justify Theorem \ref{main_thm}: when $\overline{\text{SNR}}$ exceeds some constant multiple of $\log n$, Algorithm \ref{alg1} is able to recover all the labels with high probability; when $\overline{\text{SNR}}$ is not that large, we have the bound $\exp{(-c \cdot \overline{\text{SNR}})}$ for the misclassification rate.

\noindent \textbf{Remark:} It's worthy to point out that, in Figure \ref{d=5_n=1000_K=5_r=3} and \ref{d=10_n=1000_K=5_r=3}, FASC does not perform as well as it does when $d$ is larger, since Assumption \ref{approximate_perpendicularity} may not hold when $d$ is very small. This can be justified through further experiments: in the following experiments, we perform spectral clustering on $\bu_i$. In this case, spectral clustering should be optimal. We compare the results of FASC on $\bx_{i}$ and spectral clustering on $\bu_{i}$ in Figure \label{SC no factor} with $d=5,20,100$ respectively. 
\begin{figure}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{FASC_VS_Spectral_clustering_w_o_factor_d5_n1000_K5_r3.png}
    \caption{d=5, n=1000, K=5, r=3, SC no factor}
    \label{d=5, n=1000, K=5, r=3, SC no factor}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{FASC_VS_Spectral_clustering_w_o_factor_d20_n1000_K5_r3.png}
    \caption{d=20, n=1000, K=5, r=3, SC no factor}
    \label{d=20, n=1000, K=5, r=3, SC no factor}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{FASC_VS_Spectral_clustering_w_o_factor_d100_n1000_K5_r3.png}
    \caption{d=100, n=1000, K=5, r=3, SC no factor}
    \label{d=100, n=1000, K=5, r=3, SC no factor}
\end{subfigure}}
\label{SC no factor}
\caption{FASC on $\boldsymbol{x}_i$ VS Spectral clustering on $\boldsymbol{u}_i$}
\end{figure}
In Figure \ref{d=5, n=1000, K=5, r=3, SC no factor} (where $d=5$), FASC performs poorly compared to spectral clustering. 
% This justifies that Assumption \ref{approximate_perpendicularity} does not hold when $d$ is small, therefore Theorem \ref{main_thm} can not be applied. 
On the other hand, in Figure \ref{d=100, n=1000, K=5, r=3, SC no factor} (where $d=100$), FASC performs optimally. These phenomenons justify the correctness of our theory and show the effectiveness of Algorithm \ref{alg1} under relatively high-dimension scenario.

\paragraph{Different number of factors in algorithm} 
In real datasets, the exact number $r$ of factors may be unknown. The following simulation study suggest that When applying \prettyref{algo:1}, choosing an $r$ slightly larger than the real number of factors is also efficient. In Figure \ref{FASC with  different r, model: d=100, n=1000, K=5, r=3}, the actual number of underlying factors is 3, and we apply FASC with $r=1,2,3,4,5$ relatively and plot the misclassification rate with respect to $\sigma$.When the chosen number of factors in the algorithm is smaller than the actual number of factors (i.e., $r=1,2$), FASC performs poorly. However, when the chosen number of factors in the algorithm is larger than the actual number of factors (i.e., $r=4,5$), FASC still shows quite good performance. 
% This phenomenon suggests that in practical applications, we can first estimate the number of factors, (e.g., draw a scree plot) and then choose a slightly larger $r$. 
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{FASC with different r, model- d=100, n=1000, K=5, r=3.png}
    \caption{FASC with different r, model: d=100, n=1000, K=5, r=3}
    \label{FASC with different r, model: d=100, n=1000, K=5, r=3}
\end{figure}

\subsubsection{High dimensional cases}
% In the previous section, we justify our theory through several experiments. Another interesting finding is that, it seems that FASC performs well even when $d>n$ (see Figure \ref{d=1500_n=1000_K=5_r=3}). However, it is known that the optimal sample size needed for Gaussian clustering problems we considered is $n=\Omega(d)$.
Some experiments are also provided for the scenario that $d$ is large compared to $n$ with the same data-generating process. We choose $n=100$, and $d=100,500,3000$ respectively. The results are shown in Figure \ref{FASC VS Spectral clustering, high dimension}, where FASC still performs much better than spectral clustering. However, in Figure \ref{d=3000, n=100, K=5, r=3}, FASC can only achieve exact recovery when $\sigma \leq 0.1$, while in the previous section, e.g. Figure \ref{d=100_n=1000_K=5_r=3}, FASC can achieve exact recovery for some $\sigma \geq 0.2$. This phenomenon suggests that when $d$ gets larger, the performance for FASC deteriorates. 
\begin{figure}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=100, n=100, K=5, r=3.png}
    \caption{d=100, n=100, K=5, r=3}
    \label{d=100, n=100, K=5, r=3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=500, n=100, K=5, r=3.png}
    \caption{d=500, n=100, K=5, r=3}
    \label{d=500, n=100, K=5, r=3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=3000, n=100, K=5, r=3.png}
    \caption{d=3000, n=100, K=5, r=3}
    \label{d=3000, n=100, K=5, r=3}
\end{subfigure}}
\caption{FASC VS Spectral clustering, high dimension}
\label{FASC VS Spectral clustering, high dimension}
\end{figure}
% We further perform vanilla spectral clustering on $\boldsymbol{u}_{i}= \boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i}$ and compare the results of FASC on $\boldsymbol{x}_{i}$ and spectral clustering on $\boldsymbol{u}_{i}$ in Figure \ref{d=500, n=100, K=5, r=3, SC no factor} where $n=100$, $d=500$. We can see that FASC have the same performance as spectral clustering even when $d$ is large (spectral clustering also gets worse in high dimension).

% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=500, n=100, K=5, r=3, SC no factor.png}
%     \caption{d=500, n=100, K=5, r=3, SC no factor}
%     \label{d=500, n=100, K=5, r=3, SC no factor}
% \end{figure}
% \begin{figure}
%   \centering

%   \begin{minipage}{1\textwidth}
%     \begin{subfigure}{\linewidth}
%       \centering
%       \includegraphics[width=0.8\linewidth]{d=20, n=1000, K=5, r=3.png}
%       \caption{Caption for Figure 1}
%       \label{d=20, n=1000, K=5, r=3}
%     \end{subfigure}
%     \vspace{\baselineskip}

%     \begin{subfigure}{\linewidth}
%       \centering
%       \includegraphics[width=0.8\linewidth]{d=100, n=1000, K=5, r=3.png}
%       \caption{Caption for Figure 2}
%       \label{d=100, n=1000, K=5, r=3}
%     \end{subfigure}

%     \vspace{\baselineskip}
    
%     \begin{subfigure}{\linewidth}
%       \centering
%       \includegraphics[width=0.8\linewidth]{d=500, n=1000, K=5, r=3.png}
%       \caption{Caption for Figure 2}
%       \label{d=500, n=1000, K=5, r=3}
%     \end{subfigure}
%   \end{minipage}

%   \caption{Overall Caption}
%   \label{fig:overall}
% \end{figure}

% \begin{figure}
%   \centering

%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=10, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 1}
%     \label{fig:figure1}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=20, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 2}
%     \label{fig:figure2}
%   \end{subfigure}

%   \caption{Overall Caption}
%   \label{fig:overall}
% \end{figure}



% \begin{figure}
%   \centering

%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=5, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 1}
%     \label{fig:figure1}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=500, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 2}
%     \label{fig:figure2}
%   \end{subfigure}

%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=100, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 3}
%     \label{fig:figure3}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{d=1500, n=1000, K=5, r=3.png}
%     \caption{Caption for Figure 4}
%     \label{fig:figure4}
%   \end{subfigure}

%   \caption{Overall Caption}
%   \label{fig:overall}
% \end{figure}

\subsection{Weak factor cases}
In the previous sections, we generate data from models that satisfy the "pervasiveness" Assumption \ref{pervasiveness}. In this section, we will investigate the "weak factor" cases. The data generating process remains the same, except that we generate the factor loading matrix $B\in \mathbb{R}^{d \times r}$ whose rows are drawn from i.i.d. $\frac{1}{\sqrt{d}}\mathcal{N}(0,I_{r})$.
% In the following simulations, we generate samples from the model (\ref{factor_cluster}) with the number of clusters $K=5$, the number of factors $r=3$, and each cluster has equal weight (i.e., $P_{j}=1/K$). To be specific, for $t=1,2,\cdots,100$, we generate the factor
% loading matrix $B\in \mathbb{R}^{d \times r}$ whose rows are drawn from i.i.d. $\frac{1}{\sqrt{d}}\mathcal{N}(0,I_{r})$; generate the true cluster centers $\{\boldsymbol{\mu}_{j}\}_{j=1}^{K}$ by drawing $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$ from i.i.d. $\mathcal{N}(0,\frac{1}{d}I_{d})$ and let $\boldsymbol{\mu}_{j} = \boldsymbol{\theta}_{j} - \frac{1}{K}\sum_{i=1}^{K}\boldsymbol{\theta}_{i}$; finally we set the noise level $\sigma= 0.01t$. Therefore we have $100$ different models, and for each model, we generate $n$ samples by generating class label $y_{i} \sim \text{Uniform}([K])$, latent factor $\boldsymbol{f}_{i} \sim \mathcal{N}(0,I_{r})$ and noise $\boldsymbol{\epsilon}_{i} \sim \mathcal{N}(0,\sigma^{2}I_{d})$. We then perform FASC and vanilla spectral clustering ($K=5$,$r=3$ are used in algorithms) on these generated data and compare these two methods.
The simulation results are performed in Figure \ref{FASC VS Spectral clustering, weak factor} for $n=1000$, $d=20,100,500$. Similar to Figure \ref{FASC VS Spectral clustering}, FASC still performs well under the weak factor scenario, justifying Theorem \ref{thm2}.
\begin{figure}
\makebox[\textwidth][c]{
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=20, n=1000, K=5, r=3, weak factor.png}
    \caption{d=20, n=1000, K=5, r=3, weak factor}
    \label{d=20, n=1000, K=5, r=3, weak factor}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=100, n=1000, K=5, r=3, weak factor.png}
    \caption{d=100, n=1000, K=5, r=3, weak factor}
    \label{d=100, n=1000, K=5, r=3, weak factor}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=1\textwidth, height=8cm, keepaspectratio]{d=500, n=1000, K=5, r=3, weak factor.png}
    \caption{d=500, n=1000, K=5, r=3, weak factor}
    \label{d=500, n=1000, K=5, r=3, weak factor}
\end{subfigure}}
    \caption{FASC VS Spectral clustering, weak factor}
    \label{FASC VS Spectral clustering, weak factor}
\end{figure}



==> texfiles/revised/proof_lemma_revised.tex <==
\section{A cross-fitting type spectral clustering algorithm and the corresponding guarantee} \label{cv}


Consider the following ``cross-fitting" type spectral clustering algorithm: 

\begin{algorithm}[H]
\caption{Spectral clustering}\label{alg3}
\begin{algorithmic}[1]
\State {\bf Input:} $\{\bx_i\}^{2n}_{i=1}$. The number of clusters $K$, target dimension of embedding $k$.
\State Split the data $\{\bx_i\}^{2n}_{i=1}$ into two halves, and use the second half to compute $\hat{V}$: 
\begin{equation*}
    \hat{\bV}:=(\bxi_{1},\cdots,\bxi_{k}),
\end{equation*}
where $\bxi_{1},\cdots,\bxi_{k}$ are the top $k$ right singular vectors of $(\hat{\bx}_{n+1},\cdots,\hat{\bx}_{2n})^{T} $.

\State Conduct $(1+\epsilon)$-approximate $K$-means on $\{\hat{\bV}^{T}\hat{\bx}_{i}\}_{i=1}^{n}$, getting $\{\hat{y}_{i}\}_{i=1}^{n}$ and $\{\hat{\bmu}_{j}\}_{j=1}^{K}$ such that:
\begin{equation*}
    \sum_{i=1}^n\|\hat{V}^{T}\bx_{i}-\hat{\bmu}_{\hat{y}_i}\|_2^2 \leq(1+\epsilon) \min _{\substack{\{\widetilde{\bmu}_j\}_{j=1}^K \subseteq \mathbb{R}^k \\\left\{\widetilde{y}_i\right\}_{i=1}^n \subseteq[K]}}\{\sum_{i=1}^n\|\hat{\bV}^{T}\bx_{i}-\widetilde{\bmu}_{\tilde{y}_i}\|_2^2\} .
\end{equation*}


\State {\bf Output:} $\{\hat{y}_{i}\}_{i=1}^{n}$.
\end{algorithmic}
\end{algorithm}


We have the following theoretical guarantee for Algorithm \ref{alg3} : 


\begin{lemma}\label{spectral_clustering_lemma_cv}
Consider the model defined in (\prettyref{eq:model0}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg3}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumption \ref{regularity} holds, and $d \leq O (n)$, then there exist constant $C$ and $c$ such that the following hold: \\
1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.\\
2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$.
\end{lemma}



In this section, we provide proofs for Lemma \ref{spectral_clustering_lemma_cv}. Consider the model defined in (\ref{spectral_clustering_model}). Let $\bX:= (\bx_{n+1}, \cdots, \bx_{2n})^{T}$.  We can write $\bX= \bF\bTheta + \bE$, where $\bTheta = (\btheta_{1},\cdots,\btheta_{K})^{T}\in \mathbb{R}^{K \times d} $ represents the cluster centers;
$\bF \in \mathbb{R}^{n \times k}$ is defined as $\bF_{ij}=1$ if and only if $y_{n+i}=j$, else $\bF_{ij}=0$, represents the true label of each data point, $\bE = (\bepsilon_{n+1}, \cdots, \bepsilon_{2n})^{T}$ be the noise matrix. In Algorithm \ref{alg3}, we compute $\hat{V}$ which is the top $K$ right singular vectors of $\bX$.  Let $V$ be the top $K$ right singular vectors of $\bF\bTheta$, which represents the subspace that contains the span of $\{\btheta_{j}\}_{j=1}^{K}$. The idea of proving Lemma \ref{spectral_clustering_lemma} is as the following. Notice that, since $\bV$ represents the subspace that contains the span of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$, and when $\hat{\bV}$ is close to $\bV$, then \\
1. $\bm_{j}:= \hat{\bV}^{T} \boldsymbol{\theta}_{j} $ should preserve the distance structure of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$. \\
2. For the $d$ dimensional sub-Gaussian noise $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$, when we project it onto $K$ dimensional subspace using $\hat{\bV}$, its norm becomes much smaller. Therefore, with these observations, we can use the following lemma (Lemma D.1 in \cite{abbe2022ellp}) to guarantee the success of approximate $K$-means:
\begin{lemma}[Approximate $K$-means] \label{approx_K_means} Let $\left\{\bx_i\right\}_{i=1}^n \subseteq \mathbb{R}^d$ and define
\begin{equation*}
L\left(\left\{\boldsymbol{\mu}_j\right\}_{j=1}^K,\left\{y_i\right\}_{i=1}^n\right)=\sum_{i=1}^n\left\|\bx_i-\boldsymbol{\mu}_{y_i}\right\|_2^2, \quad \forall\left\{\boldsymbol{\mu}_j\right\}_{j=1}^K \subseteq \mathbb{R}^d, \quad\left\{y_i\right\}_{i=1}^n \subseteq[K].
\end{equation*}
Let $\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{\hat{\boldsymbol{\mu}}_j\right\}_{j=1}^K \subseteq \mathbb{R}^d$, $\left\{y_i^{\star}\right\}_{i=1}^n,\left\{\hat{y}_i\right\}_{i=1}^n \subseteq[K]$, $s=\min _{j \neq k}\|\boldsymbol{\mu}_j^{\star}-\boldsymbol{\mu}_k^{\star}\|_2$ and $n_{\min}=\min_{j \in[K]} |\{i: y_i^{\star}=j\} |$. Suppose that the followings hold for some $C>0$ and $\delta \in(0, s / 2)$ :\\
1. (Near-optimality) $L\left(\left\{\hat{\boldsymbol{\mu}}_j\right\}_{j=1}^K,\left\{\hat{y}_i\right\}_{i=1}^n\right) \leq C \cdot L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right)$ and $\hat{y}_i \in \operatorname{argmin}_{j \in[K]}\left\|\bx_i-\hat{\boldsymbol{\mu}}_j\right\|_2$ for all $i \in[n]$;\\
2. (Low-noise condition) $L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) \leq \delta^2 n_{\min } /\left[(1+\sqrt{C})^2 K\right]$.\\
Then, there exists a permutation $\tau:[K] \rightarrow[K]$ such that
\begin{align*}
& \sum_{j=1}^K\left\|\boldsymbol{\mu}_j^{\star}-\hat{\boldsymbol{\mu}}_{\tau(j)}\right\|_2^2 \leq \frac{(1+\sqrt{C})^2 K}{n_{\min }} L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right), \notag \\
& \left\{i: \hat{y}_i \neq \tau\left(y_i^{\star}\right)\right\} \subseteq\left\{i:\left\|\bx_i-\boldsymbol{\mu}_{y_i^{\star}}^{\star}\right\|_2 \geq s / 2-\delta\right\}, \notag \\
& \left|\left\{i: \hat{y}_i \neq \tau\left(y_i^{\star}\right)\right\}\right| \leq\left|\left\{i:\left\|\bx_i-\boldsymbol{\mu}_{y_i^{\star}}^{\star}\right\|_2 \geq s / 2-\delta\right\}\right| .
\end{align*}
\end{lemma}
We also need the following lemma for bounding the distance between $\bV$ and $\hat{\bV}$: 
\begin{lemma} \label{lemma_3}
With probability greater than $1-O(1/n)$,
\begin{equation*}
\text{dist}(\bV,\hat{\bV}) := \min_{R \in \mathcal{O}^{r \times r}}\|\bV\bR-\hat{\bV}\| \leq O(\frac{8 \sigma (\sqrt{n}+\sqrt{d})}{\sqrt{n}}) \leq O(\sigma).
\end{equation*}
\end{lemma}
The proof of this lemma is deferred to the next subsection. We also need the following two lemmas from \cite{zhang2022leaveoneout}: 

\begin{lemma} [Lemma D.1 in \cite{zhang2022leaveoneout}] \label{Lemma_D.1_leave_one_out}
Let $\bA= (\ba_{1}, \cdots, \ba_{n}) \in \mathbb{R}^{k \times n}$ be a random matrix with each column $\ba_{i} \sim \text{SG}_{k}(\sigma^{2}) $ independently for every $i \in [n]$. Then 
\begin{equation*}
    \mathbb{P}(\|\bA\| \geq 4t\sigma (\sqrt{n}+ \sqrt{k})) \leq \exp \left(-\frac{(t^{2}-3)n}{2}\right)
\end{equation*}
for any $t \geq 2$.
\end{lemma}

\begin{lemma} [Lemma D.2 in \cite{zhang2022leaveoneout}] \label{Lemma_D.2_leave_one_out}
Let $\boldsymbol{X} \sim \text{SG}_{d}(\sigma^{2}))$ be a $d$ dimensional sub-Gaussian random vector. Then for any $k \leq d$, for any matrix $\bU = (\bu_{1}, \cdots, \bu_{k}) \in \mathbb{R}^{d\times k}$ with orthogonal columns. We have  
\begin{equation*}
    \mathbb{P}(\|\bU^{T}\bX\|^{2} \geq \sigma^{2} (k +2\sqrt{kt} + 2t)) \leq e^{-t}.
\end{equation*}
\end{lemma}

Intuitively, Lemma \ref{Lemma_D.1_leave_one_out} controls the norm of our noise matrix $E$. Lemma \ref{Lemma_D.2_leave_one_out} shows that when we project a sub-Gaussian random vector on to low dimensional subspace, its norm becomes much smaller. With these lemmas, we are now able to prove Lemma \ref{spectral_clustering_lemma}. Let 
\begin{align*}
    \bz_{i} := \hat{\bV}^{T} \bx_{i}, \\
    \bm_{j}:= \hat{\bV}^{T} \btheta_{j}.
\end{align*}
Since $\hat{\bV}$ is the top $K$ right singular vectors of $X:= (\bx_{n+1}, \cdots, \bx_{2n})^{T}$, it's independent from $\{\bx_{i}\}_{i=1}^{n}$ which we will perform spectral clustering on. By Lemma \ref{lemma_3}, with high probability (our following analysis will on this event), there exists $\bR \in \mathcal{O}^{r \times r}$ such that $\|\bV\bR-\hat{\bV}\| \leq O(\sigma).$ Then
\begin{align*}
    \|\bm_{i}-\bm_{j}\| &= \|\hat{\bV}^{T}(\btheta_{i}-\btheta_{j})\| \notag \\ 
    & \geq \|(\bV\bR)^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|((\bV\bR)^{T}-\hat{\bV}^{T})(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| \notag \\
    & \geq \|\bR^{T}\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|((\bV\bR)^{T}-\hat{\bV}^{T})\|\|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| \notag \\
    & = \|\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| - \|\bV\bR-\hat{\bV}\| \|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\|.
\end{align*}
Since $\bV$ represents the subspace that contains the span of $\{\boldsymbol{\theta}_{j}\}_{j=1}^{K}$, there exists $\bbeta$ such that $\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j} = \bV\boldsymbol{\beta}$, and $\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| = \|\boldsymbol{\beta}\|$. Then $\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}) = \bV^{T}\bV\boldsymbol{\beta} = \boldsymbol{\beta}$, therefore $\|\bV^{T}(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\| = \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|$. Also, $\|\bV\bR-\hat{\bV}\| \leq O(\sigma).$ Combine these together we have 
$\|\bm_{i}-\bm_{j}\| \geq (1-O(\sigma))\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| \geq \frac{1}{2}\|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|$. The last inequality holds when $\sigma \ll 1$, which holds because we assume $1 \ll \tilde{\text{SNR}}$ in the assumption of Lemma \ref{spectral_clustering_lemma} .

Now we can use Lemma \ref{approx_K_means} to prove our main result. In this lemma, take $\bx_{i}$ to be our $\bz_{i}$,  $\bmu_{j}^{\star}$ to be our $\bm_{j}$, and $y_{i}^{\star}$ to be our $y_{i}$. First we check the "near-optimality" condition in Lemma \ref{approx_K_means}: this holds with $C=1+\epsilon$ because we use $K$-means in our Algorithm \ref{alg2}. Second, we check the "low-noise" condition. 
\begin{align*}
    L\left(\left\{\boldsymbol{\mu}_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) &= \sum_{i=1}^{n} \|\bz_{i} - \bm_{y_{i}}\|^{2} \notag \\
    &= \sum_{i=1}^{n} \|\hat{\bV}^{T} \bx_{i} - \hat{\bV}^{T} \boldsymbol{\theta}_{y_{i}} \|^{2} \notag \\
    &= \sum_{i=1}^{n} \|\hat{\bV}^{T} \bepsilon_{i}  \|^{2} \notag \\
    &= \|\tilde{\bE}\|_{F}^{2},
\end{align*}
where we define $\tilde{\bE} := (\hat{\bV}^{T} \bepsilon_{1}, \cdots, \hat{\bV}^{T} \bepsilon_{n} ) \in \mathbb{R}^{k \times n}$. Notice that each column of $\tilde{\bE}$ is $\hat{\bV}^{T} \bepsilon_{i}$, which is independent from each other. Since we have $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$, $\hat{\bV} \in \mathbb{R}^{d \times k}$ is an projection matrix independent of those $\bepsilon_{i}$, we have $\hat{\bV}^{T} \bepsilon_{i} \sim \text{SG}_{k}(\sigma^{2})$. Therefore by Lemma \ref{Lemma_D.1_leave_one_out}, take $t=2$, we have with probability greater than $1-\exp (-\frac{1}{2}n)$, $\|\tilde{\bE}\| \leq 8 \sigma (\sqrt{n}+ \sqrt{k})$.
Then on this event, 
\begin{align*}
   L\left(\left\{\bmu_j^{\star}\right\}_{j=1}^K,\left\{y_i^{\star}\right\}_{i=1}^n\right) &= \|\tilde{\bE}\|_{F}^{2} \notag \\
   & \leq k\|\tilde{\bE}\|^{2} \notag \\
   & \leq k (8 \sigma (\sqrt{n}+ \sqrt{k}))^{2} \notag \\
   & \leq O(n\sigma^{2}). 
\end{align*}
where the last ineqaulity holds since $k=O(1)$. Therefore the low noise condition holds for $\delta = O(\sigma)$ (notice that we have regularity assumptions, so that $n_{\min }$ can not be very close to zero, with high probability). Thus, we can apply Lemma \ref{approx_K_means}, which gives 
\begin{align*}
    \left\{i: \hat{y}_i \neq \tau\left(y_i\right)\right\} &\subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq \frac{1}{2} \min_{i \neq j} \|\bm_{i}-\bm_{j}\|-\delta\right\}  \notag \\
    & \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq \frac{1}{4} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|-\delta\right\}  \notag \\
    & \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|\right\} 
\end{align*}
where the last inequality holds for some constant $c_5 >0$ since we assume $1 \ll \tilde{\text{SNR}}$  so that $\sigma \leq o(\min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|)$. Finally, since $\hat{\bV} \in \mathbb{R}^{d \times k}$ is an projection matrix independent of those $\bepsilon_{i}$, by Lemma \ref{Lemma_D.2_leave_one_out}, we have 
\begin{equation*}
    \mathbb{P}(\|\hat{\bV}^{T}\bepsilon_{i}\|^{2} \geq \sigma^{2} (k +2\sqrt{kt} + 2t)) \leq e^{-t}.
\end{equation*}
Take $t = \frac{c_6}{\sigma^{2}} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}$ for some sufficiently small constant $c_6>0$, then we have 
\begin{equation*}
    \mathbb{P}(\|\hat{\bV}^{T}\bepsilon_{i}\|^{2} \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}) \leq \exp (-\frac{c_6}{\sigma^{2}} \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|^{2}) = \exp (- c_6 \tilde{\text{SNR}}) .
\end{equation*}
Since 
\begin{equation*}
    \left\{i: \hat{y}_i \neq \tau\left(y_i\right)\right\} \subseteq \left\{i:\left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\|\right\} ,
\end{equation*}
we have 
\begin{align*}
    \mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) &\leq \mathbb{P} \left( \left\|\hat{\bV}^{T} \bepsilon_{i}\right\|_2 \geq c_5 \min_{i \neq j} \|\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j}\| \right) \notag \\
    & \leq \exp (- c_6 \tilde{\text{SNR}}) .
\end{align*}
Therefore there exist some constant $C$, such that when $\tilde{\text{SNR}} \geq C \log n$, $\mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) \leq e^{- \alpha \log n} = n^{-\alpha}$ for some $\alpha >2$. Then by union bound (notice that all the "high probability event" in our previous analysis will have probability converges to 1 when $n \rightarrow \infty$"), 
\begin{equation*}
\mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0] \geq 1 - n \cdot n^{-\alpha} - o(1) = 1- o(1) - n^{1-\alpha} \rightarrow 1,
\end{equation*}
when $n \rightarrow \infty$. 

On the other hand, for $C \log n \geq \tilde{\text{SNR}} \gg 1$, we have $\mathbb{P} (\hat{y}_i \neq \tau\left(y_i\right)) \leq e^ {- c_6 \tilde{\text{SNR}}}$. This implies
\begin{equation*}
    \mathbb{E} [\mathcal{M}(\hat{\by}, \by)] = \mathbb{E} [\frac{1}{n}\sum_{i=1}^{n} \mathbb{I}_{(\hat{y}_i \neq \tau\left(y_i\right))}] \leq e^ {- c_6 \tilde{\text{SNR}}}
\end{equation*} 
which is what we want (again, the "high probability event" in previous analysis are negligible) .

\subsection{Proof for Lemma \ref{lemma_3}}
We give the proof of Lemma \ref{lemma_3} in this subsection. By Wedin's sin$\Theta$ theorem (see \cite{MAL-079} Theorem 2.9), 
\begin{equation*}
\text{dist} (\bV, \hat{\bV}) \leq \frac{2\|\bX-\bF\bTheta\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})} = \frac{2\|\bE\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})},
\end{equation*}
where $\sigma_{k}(\bF\bTheta)$ and $\sigma_{k+1}({\bF\bTheta})$ denote the $k$-th and $(k+1)$-th singular value of $\bF\bTheta$ respectively. By Lemma \ref{Lemma_D.1_leave_one_out}, take $t=2$, we have with probability greater than $1-\exp (-\frac{1}{2}n)$, $\|\bE\| \leq 8 \sigma (\sqrt{n}+ \sqrt{d})$.

For $\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})$, notice that $\sigma_{k+1}(\bF\bTheta) = 0$ (since $\bTheta$ is rank $k$), and 
\begin{align*}
    \sigma_{k}(\bF\bTheta) = \sqrt{\lambda_{k}((\bF\bTheta)^{T}(\bF\bTheta))} = \sqrt{n} \cdot \sqrt{\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta))}.
\end{align*}
Since $(\bF\bTheta)^{T}(\bF\bTheta) = \sum_{j=1}^{K}n_{j}\btheta_{j}\btheta_{j}^{T}$, where $n_{j} = |\{i \in [n]: y_{i}=j\}|$, we have 
\begin{equation*}
\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta) = \frac{1}{n} \sum_{j=1}^{K}n_{j}\btheta_{j}\btheta_{j}^{T} \rightarrow \sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}.
\end{equation*}
To be more specific, by Weyl's inequality (see \cite{MAL-079} Lemma 2.2), 
\begin{align*}
    |\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta)) - \lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T})| &\leq \|\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta) - \sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}\| \notag \\
&\leq \sum_{j=1}^{k}|\frac{n_{j}}{n} -p_{j}| \|\btheta_{j}\btheta_{j}^{T}\| \notag \\
& \leq O(\frac{\log n}{\sqrt{n}})
\end{align*}
with probability greater than $1-O(1/n)$, because $n_{j}$ is a binomial random variable (so that it has sub-Gaussian tail bound), and $\btheta_{j}\btheta_{j}^{T}$ is $O(1)$.

Also notice that by our regularity assumptions (Assumption \ref{regularity}), $\lambda_{k} (\mathbb{\bE}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) \geq c_3$, which is equivalent to $\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) \geq c_3$. Then
\begin{align*}
  \sigma_{k}(\bF\bTheta) &= \sqrt{n} \cdot \sqrt{\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta))}  \notag \\
  &=\sqrt{n} \cdot  \sqrt {\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) - (\lambda_{k}(\frac{1}{n}(\bF\bTheta)^{T}(\bF\bTheta)) - \lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}))} \notag \\
& = \sqrt{n} \cdot  \sqrt {\lambda_{k}(\sum_{j=1}
^{K}p_{j}\btheta_{j}\btheta_{j}^{T}) + O(\frac{\log n}{\sqrt{n}})} \notag \\
&\geq  c_7 \sqrt{n}
\end{align*}
for some constant $c_7>0$. Therefore
\begin{align*}
\text{dist} (\bV, \hat{\bV}) &\leq \frac{2\|\bE\|}{\sigma_{k}(\bF\bTheta) -\sigma_{k+1}({\bF\bTheta})} \notag \\
& \leq \frac{2 \cdot 8 \sigma (\sqrt{n}+ \sqrt{d})}{c_7 \sqrt{n}} \notag \\
& \leq O(\sigma).
\end{align*}
The last line follows from our assumption that $d = O(n)$.





==> texfiles/revised/proof_main_result_revised.tex <==
\section{Proofs for \prettyref{thm:pervasive}}
As mentioned in \prettyref{sec:proof_sketch}, for the first phase,
\begin{align*}
    \hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i} \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) (\bB \bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})    \\
    &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{y_{i}} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i}  \\
    &:= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{align*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. We will first introduce several technical lemmas for analyzing $\tilde{\bmu}_{y_i}$  and $\tilde{\bepsilon}_{i}$.

\subsection{Technical lemmas for factor model estimation}


Let $\bDelta:=\bV_{r}\bV_{r}^{T} -\hat{\bV}_{r}\hat{\bV}_{r}^{T}$. We have the following lemmas for bounding $\|\bDelta\|$.
\begin{lemma}\label{matrix_perturbation_lemma}
Consider the model defined in (\ref{factor_cluster}). Let $\bSigma := \EE{\bx_{i}\bx_{i}^{T}}$ be the population covariance matrix, and $\hat{\bSigma}:= \frac{1}{n}\sum_{i=1}^{n} \bx_{i} \bx_{i}^{T}$ be the empirical covariance matrix. When $n \geq d$, for sufficiently large $n$ ("sufficiently large" means $n$ greater than some absolute constant), we have
\begin{equation*}
    \|\hat{\bSigma}- \bSigma\| \lesssim \lambda_{1}^{*} \sqrt{\frac{\log n}{n}} + \sqrt{\frac{\lambda_{1}^{*}d \log n}{n}} + \sqrt{\frac{d \log n}{n}} + \frac{d \log^2 n}{n}
\end{equation*}
with probability greater than $1-O(n^{-10})$. Here $\lambda_{1}^{*} = \lambda_{max}(\bB \bB^{T})$. 
\end{lemma}
% \begin{lemma}\label{matrix_perturbation_lemma}
% Consider the model defined in (\ref{factor_cluster}). Let $\Sigma := \mathbb{E}{\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{T}}$ be the population covariance matrix, and $\hat{\Sigma}:= \frac{1}{2n}\sum_{i=2n+1}^{4n} \boldsymbol{x}_{i} \boldsymbol{x}_{i}^{T}$ be the empirical covariance matrix. Let $A:=\mathbb{E}{\boldsymbol{u}_{i}\boldsymbol{u}_{i}^{T}}$, then we have
% \begin{equation*}
%     \|\hat{\Sigma}- \Sigma\| \leq C (\lambda_{1}^{*} \sqrt{\frac{r}{n}} + \sqrt{\frac{\|A\| \lambda_{1}^{*}d}{n}} +  \|A\| \sqrt{\frac{d}{n}} + \frac{\|A\| d (\log (n+d))^{\frac{3}{2}}}{n}  ) (\log (n+d))^{\frac{1}{2}}
% \end{equation*}
% with probability greater than $1-O((n+d)^{-10})$, when $n\geq cr (\log (n+d))^{3}$ for some constant $c,C$. Here $\lambda_{1}^{*} = \lambda_{max}(BB^{T})$. 
% \end{lemma}
% In fact, this is just the Lemma 3.5 in \cite{MAL-079}, where we replaced the $\boldsymbol{\eta}_{i} \sim \mathcal{N}(0,\sigma^{2} I_{d})$ in this book by $\boldsymbol{u}_{i} \sim \mathcal{N}(0,A)$. Notice that $\lambda_{1}^{*} = \Omega (d)$ by pervasiveness condition, and $\|A\|= O(1)$ by assumption. Therefore by Davis-Kahan Theorem, we can easily get the following proposition, which is standard in matrix perturbation theory: 
Lemma \ref{matrix_perturbation_lemma} is a generalized version of Lemma 3.5 in \cite{MAL-079}. By Davis-Kahan Theorem (see \cite{MAL-079}), since $\hat{V}_{r}$ is the top $r$ eigenvectors of $\hat{\Sigma}$, $V_{r}$ is the top $r$ eigenvectors of $\Sigma$, we have
\begin{equation*}
    \|\bDelta\| \leq \frac{\|\hat{\bSigma}- \bSigma\|}{\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)},
\end{equation*}
where $\lambda_{r}(\bSigma)$ and $\lambda_{r+1}(\bSigma)$ are the $r$-th and $(r+1)$-th largest eigenvalues of $\bSigma$ respectively. Under the conditions of \prettyref{thm:pervasive}, i.e., by pervasiveness condition, $\bSigma = \bB \bB^{T} + \EE \bu_i\bu_i^{T}$, all the $r$ non-zero eigenvalues of $\bB\bB^{T}$ scales as $\Omega(d)$, $\|\EE \bu_i\bu_i^{T}\| = O(1)$, we have $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) = \Omega (d)$. Therefore from Lemma \ref{matrix_perturbation_lemma} we get the following proposition for controlling $\|\bDelta\|$.

\begin{proposition} \label{prop:matrix_perturbation_proposition}
Under the conditions of \prettyref{thm:pervasive}, we have
\begin{equation*}
\| \bDelta \| \leq O (\sqrt{\frac{\log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}


\subsection{Technical lemma for phase 1}
The next lemma shows why Assumption \ref{approximate_perpendicularity} is important in our analysis, and why it can indicate (\ref{strict_perpendicularity}) .

\begin{lemma} \label{approx_per_lemma}
Under Assumption \ref{regularity}, \ref{pervasiveness} and \ref{approximate_perpendicularity}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma}
This lemma shows that when Assumption \ref{approximate_perpendicularity} holds, we have  (\ref{strict_perpendicularity}), and the Assumption \ref{regularity} still holds after projection, which will facilitate our analysis. 

% \begin{proof} [Proof for Lemma \ref{approx_per_lemma}]
%     Under Assumption \ref{approximate_perpendicularity}, 
% \begin{align*}
%     \Sigma &:= \mathbb{E} [{\boldsymbol{x}_{i}\boldsymbol{x}_{i}^{T}}] \notag \\
%     & =  \mathbb{E} [(B\boldsymbol{f}_{i}+ \boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i})(B\boldsymbol{f}_{i}+ \boldsymbol{\mu}_{y_{i}} + \boldsymbol{\epsilon}_{i})^{T}] \notag \\
%     & = BB^{T} + \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] + \sigma^{2} I_{d} \notag \\
%     &= U \Lambda U^{T} + MVM^{T} + \sigma^{2} I_{d}. \notag \\
% \end{align*}
% We consider $\tilde{\Sigma} := U \Lambda U^{T} + (I-UU^{T})MVM^{T}(I-UU^{T})^{T} + \sigma^{2} I_{d}.$ Notice that 
% \begin{equation*}
% U^{T} (I-UU^{T})M = (U^{T}- U^{T}UU^{T}) M = (U^{T}-U^{T})M = 0.   
% \end{equation*}
% This means the column space of $(I-UU^{T})MVM^{T}(I-UU^{T})^{T}$ (which belongs to the column space of $(I-UU^{T})M$) is orthogonal to the column space of $U$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%     (I-UU^{T})MVM^{T}(I-UU^{T})^{T} = U_{\perp} \bar{V} U_{\perp}^{T}
% \end{equation*}
% for some $U_{\perp}$ that $U_{\perp}U^{T}=0$. Thus, we have 
% \begin{equation*}
%     \tilde{\Sigma} = (U, U_{\perp},U_0)\begin{pmatrix}
%  \Lambda & &  \\
%   & \bar{V} & \\
%  & & 0
%  \end{pmatrix} (U, U_{\perp},U_0)^{T} + \sigma^{2} I_{d}
% \end{equation*}
% where $U_{0}$ is the orthogonal complement of $(U, U_{\perp})$. Since by pervasiveness condition, $\lambda_{r}(\Lambda) = \sigma_{min}(B)^{2} = \Omega(d)$, $\|\bar{V}\| \leq \|\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]\| = O(1)$, $\sigma^{2} = O(1)$, we have the top $r$ eigenvectors of $\tilde{\Sigma}$ is just $U$. Since $V_{r}$ is the top $r$ eigenvectors of $\Sigma$, by Davis-Kahan theorem, 
% \begin{equation} \label{dist_U_Vr}
% \text{dist} (U, V_{r}) := \|UU^{T}- V_{r}V_{r}^{T}\| \leq \frac{\|\Sigma- \tilde{\Sigma}\|}{\lambda_{r}(\tilde{\Sigma})}.
% \end{equation}
% It is obvious that $\lambda_{r}(\tilde{\Sigma}) = \lambda_{r}(\Lambda) = \Omega (d)$. For $\|\Sigma- \tilde{\Sigma}\|$, we have 
% \begin{align*}
%     \Sigma- \tilde{\Sigma} & = (U\Lambda U^{T} + MVM^{T} +\sigma^{2}I_{d}) - (U \Lambda U^{T} + (I-UU^{T})MVM^{T}(I-UU^{T})^{T} + \sigma^{2} I_{d}) \notag \\
%     &= UU^{T} MVM^{T} +MVM^{T}UU^{T} - UU^{T} MVM^{T} UU^{T}.
% \end{align*}
% Therefore 
% \begin{align*}
%     \|\Sigma- \tilde{\Sigma} \|& \leq  \|UU^{T} MVM^{T}\| +\|MVM^{T}UU^{T}\| + \|UU^{T} MVM^{T} UU^{T}\| \notag \\
%     &\leq 2\|U\|\|U^{T}M\|\|V\|\|M^{T}\| + \|U\|\|U^{T} M\|\|V\|M^{T} U\|\|U^{T}\| \notag \\
%     & \leq O(\|U^{T}M\|).
% \end{align*}
% Therefore by Davis-Kahan (\ref{dist_U_Vr}), $\text{dist} (U, V_{r})  \leq O(\|U^{T}M\|/d).$ With this in mind, we are able to get the desired result. For the first claim,
% \begin{align*}
%     \|(I-V_{r}V_{r}^{T})B\| &\leq \|(I-UU^{T})B\|  +  \|(UU^{T}- V_{r}V_{r}^{T})B\| \notag \\
%     &= 0 + \|(UU^{T}- V_{r}V_{r}^{T})B\| \notag \\
%     &\leq  \text{dist} (U,V_{r})\|B\| \notag \\
%     &\leq  O(\|U^{T}M\|/d) \times \Omega(\sqrt{d}) \notag \\
%     & \leq O(\frac{\|U^{T}M\|}{\sqrt{d}}) \notag \\
%     & \leq O(\sqrt{\frac{1}{\log n}}),
% \end{align*}
% where the last line follows from Assumption \ref{approximate_perpendicularity}. 

% For the second claim,
% \begin{align*}
%     &\| (I-V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| \notag \\
%     &\geq \|(I-UU^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| - \|(UU^{T}- V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     &\geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \text{dist} (U,V_{r})\|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|.
% \end{align*}
% Notice that $\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2} \in \text{Col} (M)$, then there exists $\boldsymbol{\alpha}$ such that $\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2} = M \boldsymbol{\alpha}$, and $\|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| = \|\boldsymbol{\alpha}\|$. Then we have 
% \begin{align*}
%    \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| & = \|UU^{T}M \boldsymbol{\alpha}\| \notag \\
%    &\leq \|U^{T}M \boldsymbol{\alpha}\| \notag \\
%    & \leq \|U^{T}M\| \|\boldsymbol{\alpha}\| \notag \\
%    &\leq \frac{1}{2} \|\boldsymbol{\alpha}\| = \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity}. Therefore 
% \begin{align*}
%     &\| (I-V_{r}V_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| \notag \\
%     &\geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \|UU^{T}(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - \text{dist} (U,V_{r})\|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|- \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - O(\|U^{T}M\|/d) \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq \frac{1}{2} \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| - O(\sqrt{\frac{1}{d \log n}}) \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \notag \\
%     & \geq c_2 \|(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})) \\ \notag 
%      &\geq  \lambda_{k} ((I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T})) - \|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\| \\ \notag 
%      & \geq \lambda_{k} (\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}]) - \| \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] -
%      (I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) \| \notag \\
%      &- \|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}] -
%      (I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) \| \notag \\
%     & = \|UU^{T} MVM^{T} +MVM^{T}UU^{T} - UU^{T} MVM^{T} UU^{T}\| \notag \\
%     & \leq 2 \|U^{T}M\|\|V\| + \|U^{T}M\|^{2}\|V\| \notag \\
%     & \leq C_3 (2\|U^{T}M\| + \|U^{T}M\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \notag \\
%     & \leq 3C_3 \|U^{T}M\| \quad (\text{Since} \|U^{T}M\| \leq 1) \notag \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(I-UU^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-UU^{T}) - (I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})\| \notag \\
%     & = \|(UU^{T}MVM^{T}UU^{T} - UU^{T}MVM^{T} - MVM^{T}UU^{T})  \notag \\
%     &- (V_{r}V_{r}^{T}MVM^{T}V_{r}V_{r}^{T}  - V_{r}V_{r}^{T}MVM^{T} - MVM^{T}V_{r}V_{r}^{T})\|  \notag \\
%     & \leq \|UU^{T}MVM^{T}UU^{T} - V_{r}V_{r}^{T}MVM^{T}V_{r}V_{r}^{T}\| \notag \\
%     &+ 2\|UU^{T}MVM^{T} - V_{r}V_{r}^{T}MVM^{T}\| \notag \\
%     & \leq 2 \|V\| \|UU^{T} - V_{r}V_{r}^{T} \| + 2 \|V\| \|UU^{T} - V_{r}V_{r}^{T} \| \notag \\
%     & \leq 4 C_3 O(\frac{\|U^{T}M\|}{d}) \notag \\
%     & \leq O (\sqrt{\frac{1}{d \log n}}) \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
% \end{align*}
% Combine the above three inequalities, we have 
% $\lambda_{k} ((I-V_{r}V_{r}^{T})\mathbb{E}[\boldsymbol{\mu}_{y_{i}}\boldsymbol{\mu}_{y_{i}}^{T}](I-V_{r}V_{r}^{T})) \geq \frac{1}{2}c_3$. 





% Therefore we proved Lemma \ref{approx_per_lemma}.
% \end{proof}

\subsection{Proofs for \prettyref{thm:pervasive}}

 As in the proof sketch section, we have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (\sqrt{\frac{\log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by \prettyref{prop:matrix_perturbation_proposition}). For $j_{1} \neq j_{2}$, 
\begin{equation*}
    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
\end{equation*}
On the other hand,
\begin{align*}
   \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
   & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
   &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma}}) \\
   & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (\sqrt{\frac{\log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By \prettyref{prop:matrix_perturbation_proposition}})\notag \\
   & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
    \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
\end{align*}
\shange{$\Delta$ is a random quantity. Do not write it in this way! Directly claim $\Delta$ is small with high prob,  and then jump to the result you want, see later}Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By \prettyref{prop:matrix_perturbation_proposition}}) \\
    & \leq O (\sigma^2) +O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma}}) \\
    & \leq  O (\sigma^2) +O(\frac{d \log n}{n}) + \sigma^{2} \qquad (\text{By pervasiveness condition})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{2}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. 

From the above analysis, we know that after our first phase, with probability greater than $1-O(n^{-10})$, we have $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$, where $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$ and  $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$. \shange{directly jump to this result!}In our Algorithm \ref{alg1}, after obtaining $\hat{\bu}_{i}$, we actually conduct Algorithm \ref{alg2} with input $\{\bx_i\}^{n}_{i=1} := \{\hat{\boldsymbol{u}}_{i}\}^{n}_{i=1}$, the number of clusters $K$, and target dimension of embedding $k$. We now verify that Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$: the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
\begin{align*}
    & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
     &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
     &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
     & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
     & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
     & \geq \frac{1}{2}c_3 - O(\sqrt{\frac{\log n}{n}}) \notag \\
     &\geq  \frac{1}{3}c_3.
\end{align*}
Then by Lemma \ref{spectral_clustering_lemma}, there exist constant $C$ and $c$ such that the following hold: \\
1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
\begin{equation*}
    \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
\end{equation*}
Recall our definition for $\overline{\text{SNR}}$:  
\begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
\end{equation*}
Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{thm:pervasive}.

\subsection{Proofs for Lemma \ref{matrix_perturbation_lemma} and \ref{approx_per_lemma}}

\paragraph{Proof for Lemma \ref{matrix_perturbation_lemma}}
\begin{proof}
Recall the model defined in (\ref{factor_cluster}): 
\begin{align*}
    &\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
    &\bx_{i}=\bB\bff_{i}+\bu_{i},  \quad \mbox{and} \quad    \bu_{i}=\bmu_{y_{i}} + \bepsilon_{i}.
\end{align*}
Here $\EE\bff_i=0$, $\EE \bmu_{y_{i}}=0$, $\EE \bepsilon_{i}=0$, $\cov(\bff_i)=\EE \bff_i\bff_i^{T}=\bI_r$. We also assume sub-Gaussian and boundedness properties: $\bff_i \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_i \sim \text{SG}_{d}(\sigma^2)$, $\|\bmu_j\| \leq c_2$ for any $j \in [K]$. Since $\sigma^2 \leq O(1)$, we conclude that $\bu_i$ is also sub-Gaussian with parameter $c_3^2$. 
To deal with matrix concentration, we will need the following lemma (Corollary 3.2 in \cite{MAL-079}), which is a truncated version of matrix Bernstein inequality:
\begin{lemma}[Truncated matrix Bernstein inequality]\label{matrix_Bernstein}
Let $\bZ, \bZ_1, \cdots, \bZ_n$ be i.i.d. random matrices with dimension $m_1\times m_2$. Suppose the followings hold: 
\begin{equation}\label{Bernstein_condition}
\PP(\|\bZ - \EE[\bZ]\| \geq L) \leq q_0 \quad \mbox{and} \quad  \| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}   ]   \|  \leq q_1 .
\end{equation}
Define the matrix variance statistic $V$ as $V= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \}$. Set $m:=\max\{m_1,m_2\}$. For any $a \geq 2$, with probability at least $1-2m^{-a+1}-nq_0$, 
\begin{align*}
\|\frac{1}{n}\sum_{i=1}^{n} ( \bZ_i - \EE \bZ_i )\| \leq V \sqrt{\frac{2a \log m}{n}} + L  \frac{2a \log m}{3 n}  + q_1,    
\end{align*}
where $m=m_1+m_2$.
\end{lemma}
Back to the proof of \ref{matrix_perturbation_lemma}, we have the following decomposition: 
\begin{align} \label{matrix_perturbation_ineq1}
    \|\hat{\bSigma}- \bSigma\| &= \|\frac{1}{n}\sum_{i=1}^{n}\bx_i\bx_i^{T} - \EE \bx_i\bx_i^{T}\| \notag \\
    &= \|\frac{1}{n}\sum_{i=1}^{n}(\bB \bff_i + \bu_i)(\bB \bff_i + \bu_i)^{T} - \EE (\bB \bff_i + \bu_i)(\bB \bff_i + \bu_i)^{T}\| \notag \\
    & \leq \|\bB\|^{2} \|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\| + 2\|\bB\| \|\frac{1}{n}\sum_{i=1}^{n}\bff_i \bu_i^{T}\| + \|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\|.
\end{align}
We will then bound each of the three terms by matrix Bernstein inequality. For $\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bff_i\bff_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall that $\bff_i \sim \text{SG}_{r} (c_1^2)$ implies $\|\bff_i\| \sim \text{SG} (r c^2)$ (see \cite{jin2019short} Lemma 1). Therefore 
\begin{align*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) & = \PP(\|\bff_i \bff_i^{T} - \EE[\bff_i \bff_i^{T}]\| \geq L) \\
&\leq \PP(\|\bff_i \bff_i^{T}\| +\| \EE[\bff_i \bff_i^{T}]\| \geq L) \\
&= \PP(\|\bff_i \bff_i^{T}\| \geq L-1) \\
&\leq \PP(\|\bff_i\|^2 \geq L-1) \\
&= \PP(\|\bff_i\| \geq \sqrt{L-1})
\end{align*}
Take $L= 22c^2 r \log n + 2$, by sub-Gaussian tail bound, we have $\PP(\|\bff_i\| \geq \sqrt{L-1}) \leq 2 n^{-11} :=q_0$. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bff_i\bff_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bff_i\bff_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty}  \PP(\|\bff_i\|^2 \geq y) \mathrm{d} y + L \PP (\|\bff_i\|^2 \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2rc^2}}\mathrm{d} y + 2Le^{-\frac{L}{2rc^2}} \\
&= (4rc^2+2L) e^{-\frac{L}{2rc^2}}\\
& \leq 3L e^{-\frac{L}{2rc^2}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T} - (\EE \bff_i \bff_i^{T})^2\|^{1/2} \\
& \leq \|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}\|^{1/2}.
\end{align*}
The last inequality is due to the fact that $\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}-(\EE \bff_i \bff_i^{T})^2$ and $(\EE \bff_i \bff_i^{T})^2$ are both positive semidefinite. For $\|\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}\|$, notice that for any $\bv \in \RR^r$ such that $\|\bv\|=1$, 
\begin{align*}
    \bv^{T} (\EE \bff_i \bff_i^{T} \bff_i \bff_i^{T}) \bv &= \EE [(\bff_i^{T} \bv)^2 \bff_i^{T} \bff_i] \\
    & \leq \sqrt{\EE (\bff_i^{T} \bv)^4 \EE (\bff_i^{T} \bff_i)^2 }  \qquad \text{(by Cauchy inequality)} \\
    & \leq c \sqrt{\EE \|\bff_i\|^4} \qquad \text{(since $\bff_i^{T} \bv \sim \text{SG}(c_1^2)$)} \\
    & \leq C r \qquad \text{(since $\|\bff_i\| \sim \text{SG}(c^2r)$)} 
\end{align*}
which implies $V \leq c \sqrt{r}$ for some absolute constant $c$. Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log r} $,
\begin{equation} \label{matrix_perturbation_ineq2}
\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bff_i^{T} - \EE \bff_i \bff_i^{T}\| \leq C (\sqrt{\frac{\log n}{n}} + \frac{\log^2 n}{n})\leq C \sqrt{\frac{\log n}{n}}
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$. Here we use the fact that $r =O(1)$. 

For $\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bu_i^{T} \|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bff_i \bu_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall $\|\bff_i\| \sim \text{SG} (r c^2)$, and $\bu_i \sim \text{SG}_{d} (c_3^2)$ implies $\|\bu_i\| \sim \text{SG} (d c^2)$. Therefore $\|\bff_i \bu_i^{T}\|$ is sub-exponential with parameter $c^2\sqrt{dr}$, thus
\begin{equation*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) = \PP(\|\bff_i \bu_i^{T}\| \geq L) \leq 2n^{-11} :=q_0
\end{equation*}
if we take  $L= 22c^2 \sqrt{dr} \log n $. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bff_i\bu_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bff_i\bu_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2c^2\sqrt{dr}}}\mathrm{d} y + 2Le^{-\frac{L}{2c^2\sqrt{dr}}} \\
&= (4c^2\sqrt{dr}+2L) e^{-\frac{L}{2c^2\sqrt{dr}}}\\
& \leq 3L e^{-\frac{L}{2c^2\sqrt{dr}}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \max \{ \|\EE \bff_i \bu_i^{T} \bu_i \bff_i^{T} \|^{1/2} , \|\EE \bu_i \bff_i^{T} \bff_i \bu_i^{T} \|^{1/2} \} \\
&= \max \{ \|\EE  \bu_i^{T} \bu_i \EE \bff_i \bff_i^{T} \|^{1/2} , \|\EE \bu_i \bu_i^{T} \EE \bff_i^{T} \bff_i  \|^{1/2} \} \\
&= \max \{ \|\EE \| \bu_i\|^2 \bI_r \|^{1/2} , \|\EE \bu_i \bu_i^{T} r  \|^{1/2} \} \\
&\lesssim \max\{\sqrt{d}, \sqrt{r}\} \qquad (\|\bu_i\| \sim \text{SG} (d c^2), \|\EE \bu_i \bu_i^{T}\|=O(1))\\
& =\sqrt{d}
\end{align*}
Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log d} $,
\begin{equation} \label{matrix_perturbation_ineq3}
\|\frac{1}{n}\sum_{i=1}^{n} \bff_i \bu_i^{T}\| \leq C \sqrt{d} (\sqrt{\frac{ \log n}{n}} + \frac{\log^2 n}{n}) \leq C \sqrt{\frac{ d \log n}{n}}
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$.

For $\|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\|$, we apply Lemma \ref{matrix_Bernstein} by setting $\bZ_i=\bu_i\bu_i^{T}$. We first choose proper $L$, $q_0$ and $q_1$ for (\ref{Bernstein_condition}) to hold. Recall $\|\bu_i\| \sim \text{SG} (d c^2)$. Therefore 
\begin{align*}
\PP(\|\bZ - \EE[\bZ]\| \geq L) & = \PP(\|\bu_i \bu_i^{T} - \EE[\bu_i \bu_i^{T}]\| \geq L) \\
&\leq \PP(\|\bu_i \bu_i^{T}\| +\| \EE[\bu_i \bu_i^{T}]\| \geq L) \\
& \leq \PP(\|\bu_i \bu_i^{T}\| \geq L-C) \qquad (\| \EE[\bu_i \bu_i^{T}]\| \leq C) \\
&\leq \PP(\|\bu_i\|^2 \geq L-C) \\
&= \PP(\|\bu_i\| \geq \sqrt{L-C})
\end{align*}
Take $L= 24c^2 d \log n + C$, by sub-Gaussian tail bound, we have $\PP(\|\bu_i\| \geq \sqrt{L-C}) \leq 2 n^{-12} :=q_0$. For $q_1$, 
\begin{align*}
\| \EE[\bZ]-\EE[ \bZ \11 \{ \|\bZ\| <L  \}  ]  \|  &=  \|\EE[ \bZ \11 \{ \|\bZ\| \geq L \} ] \| \\
& \leq \EE[ \|\bZ\| \11 \{ \|\bZ\| \geq L \} ]  \\
&= \EE[ (\|\bZ\|-L) \11 \{ \|\bZ\|-L \geq 0 \} ] + L \PP (\|\bZ\| \geq L ) \\
& =  \int_{0}^{\infty}  \PP(\|\bZ\|-L \geq x) \mathrm{d} x + L \PP (\|\bZ\| \geq L ) \\
& = \int_{L}^{\infty}  \PP(\|\bu_i\bu_i^{T}\| \geq y) \mathrm{d} y + L \PP (\|\bu_i\bu_i^{T}\| \geq L ) \\
& \leq \int_{L}^{\infty}  \PP(\|\bu_i\|^2 \geq y) \mathrm{d} y + L \PP (\|\bu_i\|^2 \geq L ) \\
& \leq \int_{L}^{\infty} 2e^{-\frac{y}{2dc^2}}\mathrm{d} y + 2Le^{-\frac{L}{2dc^2}} \\
&= (4dc^2+2L) e^{-\frac{L}{2rc^2}}\\
& \leq 3L e^{-\frac{L}{2dc^2}} \\
&\leq n^{-10} :=q_1
\end{align*}
for sufficiently large $n$. Here we use the fact that $n \geq d$. For the variance statistic $V$, by definition we have 
\begin{align*}
V &= \max \{ \|\EE (\bZ - \EE \bZ )(\bZ - \EE \bZ )^{T}\|^{1/2}, \|\EE(\bZ - \EE \bZ )^{T} (\bZ - \EE \bZ )\|^{1/2} \} \\
&= \|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T} - (\EE \bu_i \bu_i^{T})^2\|^{1/2} \\
& \leq \|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}\|^{1/2}.
\end{align*}
The last inequality is due to the fact that $\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}-(\EE \bu_i \bu_i^{T})^2$ and $(\EE \bu_i \bu_i^{T})^2$ are both positive semidefinite. For $\|\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}\|$, notice that for any $\bv \in \RR^d$ such that $\|\bv\|=1$, 
\begin{align*}
    \bv^{T} (\EE \bu_i \bu_i^{T} \bu_i \bu_i^{T}) \bv &= \EE [(\bu_i^{T} \bv)^2 \bu_i^{T} \bu_i] \\
    & \leq \sqrt{\EE (\bu_i^{T} \bv)^4 \EE (\bu_i^{T} \bu_i)^2 }  \qquad \text{(by Cauchy inequality)} \\
    & \leq c \sqrt{\EE \|\bu_i\|^4} \qquad \text{(since $\bu_i^{T} \bv \sim \text{SG}(c_3^2)$)} \\
    & \leq C d \qquad \text{(since $\|\bu_i\| \sim \text{SG}(c^2d)$)} 
\end{align*}
which implies $V \leq c \sqrt{d}$ for some absolute constant $c$. Therefore by Lemma \ref{matrix_Bernstein}, take $a=\frac{11 \log n}{\log d} $,
\begin{equation} \label{matrix_perturbation_ineq4}
\|\frac{1}{n}\sum_{i=1}^{n} \bu_i \bu_i^{T} - \EE \bu_i \bu_i^{T}\| \leq C (\sqrt{\frac{d\log n}{n}} + \frac{d\log^2 n}{n})
\end{equation}
with probability at least $1-3n^{-10}$ for sufficiently large $n$. 

Finally, combine (\ref{matrix_perturbation_ineq1}), (\ref{matrix_perturbation_ineq2}), (\ref{matrix_perturbation_ineq3}), (\ref{matrix_perturbation_ineq4}), we have with probability $1-O(n^{-10})$
\begin{equation*}
    \|\hat{\bSigma}- \bSigma\| \lesssim \lambda_{1}^{*} \sqrt{\frac{\log n}{n}} + \sqrt{\frac{\lambda_{1}^{*}d \log n}{n}} + \sqrt{\frac{d \log n}{n}} + \frac{d \log^2 n}{n}
\end{equation*}
which is exactly what we want.
\end{proof}
\paragraph{Proof for Lemma \ref{approx_per_lemma}}
\begin{proof}
    Under Assumption \ref{approximate_perpendicularity}, 
\begin{align*}
    \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
    & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
    & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
\end{align*}
We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$. Notice that 
\begin{equation*}
\bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
\end{equation*}
This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
\begin{equation*}
     (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
\end{equation*}
for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$. Thus, we have 
\begin{equation*}
    \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
 \bLambda & &  \\
  & \bar{\bV} & \\
 & & 0
 \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T}
\end{equation*}
where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By pervasiveness condition,
\shange{this is where I use $\sigma_{min}$. Actually I should replace all of this by $\sigma_r$.}$\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} = \Omega(d)$, 
$\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| = O(1)$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma}) = \lambda_{r}(\bLambda) = \Omega (d)$, and $\lambda_{r+1}(\tilde{\bSigma})=\|\bar{\bV}\|=O(1)$. For $\|\bSigma- \tilde{\bSigma}\|$, we have 
\begin{align*}
    \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}]) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}) \\
    &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}].
\end{align*}
Recall $\bepsilon_i \sim \text{SG}_{d} (\sigma^2)$, which means for any $\bv \in \RR^d$ such that $\|\bv\|=1$, $\bv^{T}\bepsilon_{i} \sim \text{SG} (\sigma^2)$, thus
\begin{equation*}
    \bv^{T} \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \bv = \EE (\bv^{T}\bepsilon_{i})^2 \leq c \sigma^2.
\end{equation*}
Therefore $\|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\| \leq c\sigma^2$. We then have
\begin{align*}
    \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| + \|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\|  \\
    &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| +c\sigma^2 \\
    & \leq O(\|\bU^{T}\bM\| + \sigma^2).
\end{align*}
Therefore by Davis-Kahan (\ref{dist_U_Vr}), $\text{dist} (\bU, \bV_{r})  \leq O(\frac{\|\bU^{T}\bM\| + \sigma^2}{d}).$ By Assumption \ref{approximate_perpendicularity} and $\sigma \leq 1$, we have $O(\frac{\|\bU^{T}\bM\| + \sigma^2}{d}) \leq O ((\sigma/ \sqrt{d})\wedge (1/d))$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma/ \sqrt{d}) \times \Omega(\sqrt{d}) \\
    & \leq O(\sigma).
\end{align*}

For the second claim,
\begin{align*}
    &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
    &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
    &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
\end{align*}
Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, \shange{why this is true? need to mention $\bM$ is orthogonal. or write it in another way.} and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
\begin{align*}
   \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
   &\leq \|\bU^{T}\bM \balpha\| \\
   & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
   &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
\end{align*}
where the last inequality follows from Assumption \ref{approximate_perpendicularity}. Therefore 
\begin{align*}
    &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
    &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(1/ d) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(1/ d) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
    & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
\end{align*}
for some constant $c_2 > 0$. 

For the third claim, notice that by Weyl's inequality, 
\begin{align*}
     &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
     &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
     & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
     (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
     &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
\end{align*}
Notice that 
\begin{align*}
    &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
     (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
    & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
    & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
    & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
    & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
    &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity}}).
\end{align*}
Also,
\begin{align*}
    &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
    & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
    &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
    & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
    &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
    & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
    & \leq 4 C_3 O(\frac{1}{d}) =O(1)
\end{align*}
for sufficiently large $d$. Combine the above three inequalities, we have 
\begin{align*}
\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
\end{align*}
Therefore we proved Lemma \ref{approx_per_lemma}.
\end{proof}

\subsection{Proof for Lemma \ref{spectral_clustering_lemma}}
In this subsection we will briefly show why Lemma \ref{spectral_clustering_lemma} is a consequence of Corollary 3.1 in \cite{zhang2022leaveoneout}. 

We first claim that, although Theorem 3.1 and Corollary 3.1 in \cite{zhang2022leaveoneout} hold for spectral clustering with exact K-means, the results will actually hold for $(1+\epsilon)$-approximate K-means with only differences in constants. To see this, notice that in the proof of Proposition 3.1, \cite{zhang2022leaveoneout} claims that 
\begin{equation*}
    \|\hat{\Theta}-\hat{P}\|_{F} \leq \|P-\hat{P}\|_{F}
\end{equation*}
since $\hat{\Theta}$ is the solution to the exact K-means. However if $\hat{\Theta}$ is the solution to $(1+\epsilon)$-approximate K-means, we can similarly get 
\begin{equation*}
    \|\hat{\Theta}-\hat{P}\|_{F} \leq (1+\epsilon) \|P-\hat{P}\|_{F}.
\end{equation*}
Using this inequality will not affect the analysis except for several constants. As long as Proposition 3.1 still holds, the proofs of Theorem 3.1 will still remains the same.

Now it remains to show Lemma \ref{spectral_clustering_lemma} is a consequence of Corollary 3.1 in \cite{zhang2022leaveoneout} (with approximate K-means). Recall the definition of several quantities in \cite{zhang2022leaveoneout}: $\Delta=\min_{i \neq j}\|\btheta_i - \btheta_i\|$, $\beta=\frac{K}{n} \min_{j\in[K]} \{i:y_i \neq j\}$, $\lambda_K$ be the $K$-th singular value of data matrix $\bX$. Therefore we can see that, under our model, when $n$ is sufficiently large, with probability $1-o(1)$, $\beta \approx K \min_{j\in[K]}p_j $ which means $\beta=\Theta(1)$. Also $\Delta=\Theta(1)$, and $\lambda_K$ will scale with $\sqrt{n}$. Therefore we can see that when $d \leq O(n)$, the conditions in Corollary 3.1 in \cite{zhang2022leaveoneout} will be satisfied when $n$ is sufficiently large. Therefore Lemma \ref{spectral_clustering_lemma} is immediately implied.

\section{Proofs for \prettyref{thm:2}}
The proofs for \prettyref{thm:2} are similar to that of \prettyref{thm:pervasive}. We also have $\hat{\bu}_{i}= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$. For the factor model estimation, Lemma \ref{matrix_perturbation_lemma} still applies. Recall Davis-Kahan theorem
\begin{equation*}
    \|\bDelta\| \leq \frac{\|\hat{\bSigma}- \bSigma\|}{\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)},
\end{equation*}
we will need to control $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma)$.
We have $\bSigma = \bB \bB^{T} + \bSigma_u$, therefore by Weyl's ineqaulity, $|\lambda_{r}(\bSigma)-\lambda_{r}(\bB \bB^{T})| \leq \|\bSigma-\bB \bB^{T}\| = \|\bSigma_u\|$. Similarly $|\lambda_{r+1}(\bSigma)|= |\lambda_{r+1}(\bSigma)-\lambda_{r+1}(\bB \bB^{T})| \leq \|\bSigma-\bB \bB^{T}\| = \|\bSigma_u\|$. By Assumption \ref{weak_factor1}, $\lambda_{r}(\bB \bB^{T})= \sigma_{\min}^{2} (\bB) \geq 3 \|\bSigma_u\|$. Therefore $\lambda_{r}(\bSigma) \geq 2 \|\bSigma_u\|$, $\lambda_{r+1}(\bSigma) \leq \|\bSigma_u\|$, which implies $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) \geq \|\bSigma_u\| \geq c$ for some absolute constant $c$ (by \prettyref{asmp:regularity}). Therefore from Lemma \ref{matrix_perturbation_lemma} we get the following proposition for controlling $\|\bDelta\|$.
\begin{proposition} \label{matrix_perturbation_proposition2}
Under the conditions of Theorem \ref{weak_factor1}, we have
\begin{equation*}
\| \bDelta \| \leq O (\sqrt{\frac{d \log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}
Similar to Lemma \ref{approx_per_lemma}, we have the following:
\begin{lemma} \label{approx_per_lemma2}
Under \prettyref{asmp:regularity}, \ref{weak_factor1} and \ref{approximate_perpendicularity2}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma} 
With this lemma, we can prove Theorem \ref{thm2}. Similar to the proof for \prettyref{thm:pervasive}, we have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (\sqrt{\frac{d \log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by Proposition \ref{matrix_perturbation_proposition2}). Similar to the proof for \prettyref{thm:pervasive}, for $j_{1} \neq j_{2}$, 
\begin{equation*}
    \frac{c_2}{2} \|\bmu_{j_1} -\bmu_{j_2}\| \leq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \leq \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{equation*}




% For $j_{1} \neq j_{2}$, 
% \begin{equation*}
%     \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
% \end{equation*}

% On the other hand,
% \begin{align*}
%    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%    & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
%    &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma2}}) \\
%    & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (\sqrt{\frac{d \log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Proposition \ref{matrix_perturbation_proposition2}})\notag \\
%    & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
% \end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
    \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
    &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
\end{align*}
Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{d\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Proposition \ref{matrix_perturbation_proposition2}}) \\
    & \leq O (\sigma^2) +O(\frac{d\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma2}}) \\
    & \leq  O (\sigma^2) +O(\frac{d \log n}{n}) + \sigma^{2} \qquad (\text{By Assumption \ref{weak_factor1}})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{3}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. Similar to the proofs for Theorem \ref{thm:pervasive}, Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$. Thus by applying Lemma \ref{spectral_clustering_lemma} we get the desired result.


% : the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma2}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
% \begin{align*}
%     & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
%      &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
%      &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
%      & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
%      & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
%      & \geq \frac{1}{2}c_3 - O(\sqrt{\frac{d\log n}{n}}) \notag \\
%      &\geq  \frac{1}{3}c_3.
% \end{align*}
% Then by Lemma \ref{spectral_clustering_lemma}, there exist constant $C$ and $c$ such that the following hold: \\
% 1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
% 2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
% \begin{equation*}
%     \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
% \end{equation*}
% Recall our definition for $\overline{\text{SNR}}$:  
% \begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
% \end{equation*}
% Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{thm2}.

\subsection{Proofs for Lemma \ref{approx_per_lemma2}}
\begin{proof}
We use the same notations as in the proofs for Lemma \ref{approx_per_lemma}. Then
% \begin{align*}
%     \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
%     & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
%     & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
%     &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
% \end{align*}
% We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$. Notice that 
% \begin{equation*}
% \bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
% \end{equation*}
% This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%      (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
% \end{equation*}
% for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$. Thus, we have 
% \begin{equation*}
%     \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
%  \bLambda & &  \\
%   & \bar{\bV} & \\
%  & & 0
%  \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T}
% \end{equation*}
% where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By Assumption \ref{weak_factor1}, $\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} \geq 3 \|\bSigma_u\|$, $\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| \leq \|\bSigma_u\|$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr2}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma})-\lambda_{r+1}(\tilde{\bSigma}) \geq 2 \|\bSigma_u\| \geq c_3$. For $\|\bSigma- \tilde{\bSigma}\|$, as in the proofs for Lemma \ref{approx_per_lemma},
% we have 
% \begin{align*}
%     \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}]) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}) \\
%     &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}].
% \end{align*}
% Recall $\bepsilon_i \sim \text{SG}_{d} (\sigma^2)$, which means for any $\bv \in \RR^d$ such that $\|\bv\|=1$, $\bv^{T}\bepsilon_{i} \sim \text{SG} (\sigma^2)$, thus
% \begin{equation*}
%     \bv^{T} \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \bv = \EE (\bv^{T}\bepsilon_{i})^2 \leq c \sigma^2.
% \end{equation*}
% Therefore $\|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\| \leq c\sigma^2$. We then have
% \begin{align*}
%     \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| + \|\EE [\bepsilon_{i}\bepsilon_{i}^{T}]\|  \\
%     &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| +c\sigma^2 \\
%     & \leq O(\|\bU^{T}\bM\| + \sigma^2).
% \end{align*}
$\|\bSigma- \tilde{\bSigma} \| \leq O(\|\bU^{T}\bM\| + \sigma^2)$. Therefore by Davis-Kahan (\ref{dist_U_Vr2}), $\text{dist} (\bU, \bV_{r})  \leq O(\|\bU^{T}\bM\| + \sigma^2).$ By Assumption \ref{approximate_perpendicularity2} and $\sigma \leq 1$, we have $O(\|\bU^{T}\bM\| + \sigma^2) \leq O(\sigma)$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma) \times \Omega(1) \\
    & \leq O(\sigma).
\end{align*}
The proofs for the second and the third claim are similar to that of Lemma \ref{approx_per_lemma}.
\end{proof}
% For the second claim,
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
%     &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
% \end{align*}
% Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
% \begin{align*}
%    \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
%    &\leq \|\bU^{T}\bM \balpha\| \\
%    & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
%    &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity2}. Therefore 
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(\sigma) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(\sigma) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
%      &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
%      & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%      &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%     & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
%     & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
%     & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
%     & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity2}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
%     & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
%     &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
%     & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
%     &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
%     & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
%     & \leq 4 C_3 O(\sigma) =O(1).
% \end{align*}
% Combine the above three inequalities, we have 
% \begin{align*}
% \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
% \end{align*}
% Therefore we proved Lemma \ref{approx_per_lemma2}.
% \end{proof}

\section{Proofs for \prettyref{thm:3}}
The proof of \prettyref{thm:3} is similar to that of \prettyref{thm:pervasive}. Under Assumption \ref{weak_factor2}, we also have $\lambda_{r}(\bB \bB^{T})= \sigma_{\min}^{2} (\bB) \geq 3 \|\bSigma_u\|$, therefore  $\lambda_{r}(\bSigma)-\lambda_{r+1}(\bSigma) \geq \|\bSigma_u\| \geq c$ still applies. Combining Lemma \ref{matrix_perturbation_lemma}, we get the following proposition for controlling $\|\bDelta\|$.
\begin{proposition} \label{matrix_perturbation_proposition3}
Under the conditions of Theorem \ref{weak_factor2}, we have
\begin{equation*}
\| \bDelta \| \leq O (d\sqrt{\frac{\log n}{n}})    
\end{equation*}
with probability greater than $1-O(n^{-10})$, for sufficiently large $n$. 
\end{proposition}
Similar to Lemma \ref{approx_per_lemma}, we have the following:
\begin{lemma} \label{approx_per_lemma3}
Under \prettyref{asmp:regularity}, \ref{weak_factor1} and \ref{approximate_perpendicularity2}, the following hold:\\
1. $\|(\bI-\bV_{r}\bV_{r}^{T})\bB\| \leq O (\sigma) $ \\
2. There exist constant $c_2 >0$, such that $\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\|$ for any $j_{1}\neq j_{2}$. \\
3. $C_3 \geq \lambda_{1} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. 
\end{lemma} 
With this lemma, we can prove Theorem \ref{thm3}. We have
\begin{equation*}
    \hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{equation*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB \bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})  \bepsilon_{i} $. In the following, we do the analysis on the event that $\|\bDelta \| \leq O (d\sqrt{\frac{\log n}{n}}) $
which has probability greater than $1-O(n^{-10})$ for sufficiently large $n$ (by \prettyref{prop:matrix_perturbation_proposition}). For $j_{1} \neq j_{2}$, 
\begin{equation*}
    \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| = \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \leq \|\bmu_{j_1} -\bmu_{j_2}\|.
\end{equation*}
On the other hand,
\begin{align*}
   \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| &= \| (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
   & \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|\bDelta (\bmu_{j_1} -\bmu_{j_2})\| \\
   &= c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - \|\bDelta\| \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Lemma \ref{approx_per_lemma3}}) \\
   & \geq c_2 \|\bmu_{j_1} -\bmu_{j_2}\| - O (d\sqrt{\frac{ \log n}{n}}) \| \bmu_{j_1} -\bmu_{j_2}\| \qquad (\text{By Proposition \ref{matrix_perturbation_proposition3}})\notag \\
   & \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|,
\end{align*}
for sufficiently large $n$, with probability greater than $1-O(n^{-10})$. The last equality use the assumption that $d^3 \leq O(\frac{n}{(\log n)^{3}})$. Therefore $\tilde{\bmu}_{y_i}$ preserves the structure of $\bmu_{y_i}$ with high probability. For $\tilde{\bepsilon}_{i}$, 
% \begin{align*}
%     \tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
%     &= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} .
% \end{align*}
% Notice that $\bff_{i} \sim \text{SG}_{r}(c_1^2)$, $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^2)$, 
we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} + \|\bDelta \bB\|^{2} + \sigma^{2}))$. Therefore
\begin{align*}
  & \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \\ 
  & \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +\|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
& \leq \|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +O(\frac{d^2\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Proposition \ref{matrix_perturbation_proposition3}}) \\
    & \leq O (\sigma^2) +O(\frac{d^2\log n}{n}) \|\bB\|^{2} + \sigma^{2} \qquad (\text{By Lemma \ref{approx_per_lemma3}}) \\
    & \leq  O (\sigma^2) +O(\frac{d^3 \log n}{n}) + \sigma^{2} \qquad (\text{By Assumption \ref{weak_factor2}})  \\
    & \leq O (\sigma^2) +O(\frac{1}{\log n}) + \sigma^{2}  \qquad (\text{By the assumption that } d^3 \leq O ( \frac{n}{(\log n)^{3}}) )
\end{align*}
% Therefore, when $\sigma^{2} \leq \frac{c}{\log n}$ for some absolute constant $c$, we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|(\bI-\bV_{r}\bV_{r}^{T}) \bB\|^{2} +  \|\bDelta \bB\|^{2} + \sigma^{2}\leq C\sigma^{2}$ for some absolute constant $C$. 
Similar to the proofs for Theorem \ref{thm:pervasive}, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} ( C' (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$ for some constant $C'$, which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise. The only thing remains is to verify that Assumption \ref{regularity} still holds (for alternative constants) for $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$: the first two conditions in Assumption \ref{regularity} is easy to verify, since we have shown $ \|\bmu_{j_1} -\bmu_{j_2}\| \geq \|\tilde{\bmu}_{j_{1}} - \tilde{\bmu}_{j_2}\| \geq \frac{c_{2}}{2} \|\bmu_{j_1} -\bmu_{j_2}\|$; for verifying the third condition, we use the third claim in Lemma \ref{approx_per_lemma3}, which says $ \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3$. Then by Weyl's inequality, 
\begin{align*}
    & \lambda_{k} (\mathbb{E}[\tilde{\bmu}_{y_{i}}\tilde{\bmu}_{y_{i}}^{T}]) \\
     &=\lambda_{k} ((\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\  
     &\geq  \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\
     & - \|(\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T}) - (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\| \\ 
     & \geq \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) - O(\|\bDelta\|)\\
     & \geq \frac{1}{2}c_3 - O(d\sqrt{\frac{\log n}{n}}) \notag \\
     &\geq  \frac{1}{3}c_3.
\end{align*}
The last inequality uses the assumption that $d^3 \leq O(\frac{n}{(\log n)^3})$. By Lemma \ref{spectral_clustering_lemma}, we get the desired result.

% there exist constant $C$ and $c$ such that the following hold: \\
% 1. If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})=0]=1$.\\
% 2. If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\boldsymbol{y}}, \boldsymbol{y})] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$. Where
% \begin{equation*}
%     \widetilde{\text{SNR}} := \frac{\min_{j_1\neq j_2}\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\|^{2}}{C' (\max \{ \frac{1}{\log n}, \sigma^{2}\})}.
% \end{equation*}
% Recall our definition for $\overline{\text{SNR}}$:  
% \begin{equation*} \overline{\text{SNR}} := \frac{\min_{i\neq j}\|(\bmu_{i}-\bmu_{j})\|^{2}}{\sigma^2} . 
% \end{equation*}
% Then when $\sigma^{2} \leq \frac{1}{\log n}$, $\overline{\text{SNR}} \geq \Omega (\widetilde{\text{SNR}}) > \Omega( \log n) $. When $\sigma^{2} \geq \frac{1}{\log n}$, $\Omega( \log n) \geq \widetilde{\text{SNR}} \geq \Omega( \overline{\text{SNR}} ) $. Therefore the above results give the desired results for Theorem \ref{thm3}.

\subsection{Proofs for Lemma \ref{approx_per_lemma3}}
\begin{proof}
The proof is similar to that of Lemma \ref{approx_per_lemma} with slight differences. Recall
\begin{align*}
    \bSigma &:= \mathbb{E} [{\bx_{i}\bx_{i}^{T}}] \\
    & =  \mathbb{E} [(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})(\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})^{T}] \\
    & = \bB \bB^{T} + \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \EE [\bepsilon_{i}\bepsilon_{i}^{T}] \\
    &= \bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \sigma^2 \bI_d.
\end{align*}
We consider $\tilde{\bSigma} := \bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} + \sigma^2 \bI_d$. 
% Notice that 
% \begin{equation*}
% \bU^{T} (\bI-\bU\bU^{T})\bM = (\bU^{T}- \bU^{T}\bU\bU^{T}) \bM = (\bU^{T}-\bU^{T})\bM = 0.   
% \end{equation*}
% This means the column space of $ (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T}$ (which belongs to the column space of $(\bI-\bU\bU^{T})\bM$) is orthogonal to the column space of $\bU$. Thus we can write the eigendecomposition that 
% \begin{equation*}
%      (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} = \bU_{\perp} \bar{\bV} \bU_{\perp}^{T}
% \end{equation*}
% for some $\bU_{\perp}$ that $\bU_{\perp}\bU^{T}=0$.
Similar to the proof for Lemma \ref{approx_per_lemma} (with an additional term), we have 
\begin{equation*}
    \tilde{\bSigma} = (\bU, \bU_{\perp},\bU_0)\begin{pmatrix}
 \bLambda & &  \\
  & \bar{\bV} & \\
 & & 0
 \end{pmatrix} (\bU, \bU_{\perp},\bU_0)^{T} + \sigma^2 \bI_d
\end{equation*}
where $\bU_{0}$ is the orthogonal complement of $(\bU, \bU_{\perp})$. By Assumption \ref{weak_factor1},\shange{this is where I use $\sigma_{min}$. Actually I should replace all of this by $\sigma_r$.} $\lambda_{r}(\bLambda) = \sigma_{min}(\bB)^{2} \geq 3 \|\bSigma_u\|$, $\|\bar{\bV}\| \leq \|\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]\| \leq \|\bSigma_u\|$. Therefore the top $r$ eigenvectors of $\tilde{\bSigma}$ is just $\bU$. Since $\bV_{r}$ is the top $r$ eigenvectors of $\bSigma$, by Davis-Kahan theorem, 
\begin{equation} \label{dist_U_Vr3}
\text{dist} (\bU, \bV_{r}) := \|\bU\bU^{T}- \bV_{r}\bV_{r}^{T}\| \leq \frac{\|\bSigma- \tilde{\bSigma}\|}{\lambda_{r}(\tilde{\bSigma})- \lambda_{r+1}(\tilde{\bSigma})}.
\end{equation}
It is obvious that $\lambda_{r}(\tilde{\bSigma})-\lambda_{r+1}(\tilde{\bSigma}) \geq 2 \|\bSigma_u\| \geq c_3$. For $\|\bSigma- \tilde{\bSigma}\|$, we have 
\begin{align*}
    \bSigma- \tilde{\bSigma} & = (\bU \bLambda \bU^{T} + \bM\bV\bM^{T} + \sigma^2 \bI_d) - (\bU \bLambda \bU^{T} + (\bI-\bU\bU^{T})\bM\bV\bM^{T}(\bI-\bU\bU^{T})^{T} + \sigma^2 \bI_d) \\
    &= \bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}.
\end{align*}
We then have
\begin{align*}
    \|\bSigma- \tilde{\bSigma} \|& \leq  \|\bU\bU^{T} \bM\bV\bM^{T}\| +\|\bM\bV\bM^{T}\bU\bU^{T}\| + \|\bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
    &\leq 2\|\bU\|\|\bU^{T}\bM\|\|\bV\|\|\bM^{T}\| + \|\bU\|\|\bU^{T} \bM\|\|\bV\|\bM^{T} \bU\|\|\bU^{T}\| \\
    & \leq O(\|\bU^{T}\bM\|).
\end{align*}
Therefore by Davis-Kahan (\ref{dist_U_Vr3}), $\text{dist} (\bU, \bV_{r})  \leq O(\|\bU^{T}\bM\|).$ By Assumption \ref{approximate_perpendicularity3}, we have $O(\|\bU^{T}\bM\|) \leq O(\sigma/\sqrt{d})$.  With this in mind, we are able to get the desired result. For the first claim,
\begin{align*}
    \|(\bI-\bV_{r}\bV_{r}^{T})\bB\| &\leq \|(\bI-\bU\bU^{T})\bB\|  +  \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &= 0 + \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})\bB\| \\
    &\leq  \text{dist} (\bU,\bV_{r})\|\bB\|  \\
    &\leq  O (\sigma/\sqrt{d}) \times \Omega(\sqrt{d}) \\
    & \leq O(\sigma).
\end{align*}
The proofs for the second and the third terms are similar to that of Lemma \ref{approx_per_lemma}.
% For the second claim,
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \|  \\
%     &\geq \|(\bI-\bU\bU^{T})(\bmu_{j_1} -\bmu_{j_2}) \| - \|(\bU\bU^{T}- \bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2})\| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\|.
% \end{align*}
% Notice that $\bmu_{j_1} -\bmu_{j_2} \in \text{Col} (\bM)$, then there exists $\balpha$ such that $\bmu_{j_1} -\bmu_{j_2} = \bM \balpha$, and $\|\bmu_{j_1} -\bmu_{j_2}\| = \|\balpha\|$. Then we have 
% \begin{align*}
%    \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| & = \|\bU\bU^{T}\bM \balpha \| \\
%    &\leq \|\bU^{T}\bM \balpha\| \\
%    & \leq \|\bU^{T}\bM\| \|\balpha \|  \\
%    &\leq \frac{1}{2} \|\balpha\| = \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\|,
% \end{align*}
% where the last inequality follows from Assumption \ref{approximate_perpendicularity3}. Therefore 
% \begin{align*}
%     &\| (\bI-\bV_{r}\bV_{r}^{T})(\bmu_{j_1} -\bmu_{j_2}) \| \\
%     &\geq \|(\bmu_{j_1} -\bmu_{j_2})\| - \|\bU\bU^{T}(\bmu_{j_1} -\bmu_{j_2})\| - \text{dist} (\bU,\bV_{r})\|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \|(\bmu_{j_1} -\bmu_{j_2})\|- \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| - O(\sigma/\sqrt{d}) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq \frac{1}{2} \|(\bmu_{j_1} -\bmu_{j_2})\| -  O(\sigma/\sqrt{d}) \|(\bmu_{j_1} -\bmu_{j_2})\| \\
%     & \geq c_2 \|(\bmu_{j_1} -\bmu_{j_2})\|
% \end{align*}
% for some constant $c_2 > 0$. 

% For the third claim, notice that by Weyl's inequality, 
% \begin{align*}
%      &\lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \\ 
%      &\geq  \lambda_{k} ((\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T})) - \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\ 
%      & \geq \lambda_{k} (\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}]) - \| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%      &- \|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\|.
% \end{align*}
% Notice that 
% \begin{align*}
%     &\| \mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}] -
%      (\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) \| \\
%     & = \|\bU\bU^{T} \bM\bV\bM^{T} +\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T} \bM\bV\bM^{T} \bU\bU^{T}\| \\
%     & \leq 2 \|\bU^{T}\bM\|\|\bV\| + \|\bU^{T}\bM\|^{2}\|\bV\| \\
%     & \leq C_3 (2\|\bU^{T}\bM\| + \|\bU^{T}\bM\|^{2}) \quad (\text{By Assumption \ref{regularity}}) \\
%     & \leq 3C_3 \|\bU^{T}\bM\| \quad (\text{Since} \|\bU^{T}\bM\| \leq 1)  \\
%     &\leq \frac{1}{3} c_3 \quad (\text{By Assumption \ref{approximate_perpendicularity3}}).
% \end{align*}
% Also,
% \begin{align*}
%     &\|(\bI-\bU\bU^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bU\bU^{T}) - (\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})\| \\
%     & = \|(\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bU\bU^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bU\bU^{T}) \\
%     &- (\bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}  - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T} - \bM\bV\bM^{T}\bV_{r}\bV_{r}^{T})\|  \\
%     & \leq \|\bU\bU^{T}\bM\bV\bM^{T}\bU\bU^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\bV_{r}\bV_{r}^{T}\| \\
%     &+ 2\|\bU\bU^{T}\bM\bV\bM^{T} - \bV_{r}\bV_{r}^{T}\bM\bV\bM^{T}\| \\
%     & \leq 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| + 2 \|\bV\| \|\bU\bU^{T} - \bV_{r}\bV_{r}^{T} \| \\
%     & \leq 4 C_3 O(\sigma/\sqrt{d}) =O(1).
% \end{align*}
% Combine the above three inequalities, we have 
% \begin{align*}
% \lambda_{k} ((\bI-\bV_{r}\bV_{r}^{T})\mathbb{E}[\bmu_{y_{i}}\bmu_{y_{i}}^{T}](\bI-\bV_{r}\bV_{r}^{T})) \geq \frac{1}{2}c_3.     
% \end{align*}
% Therefore we proved Lemma \ref{approx_per_lemma3}.
\end{proof}

==> texfiles/revised/proof_sketch_thm_1_old.tex <==
\section{Proof sketch of \prettyref{thm:2}}
In this subsection, we briefly characterize the intuition of proving Theorem \ref{main_thm}. For simplicity, we assume Assumption \ref{regularity} and (\ref{strict_perpendicularity}) hold "strictly". The detailed proof under Assumption \ref{approximate_perpendicularity} will be presented in the Appendix. Our proof strategy has two phases: in the first phase, we show that our estimator $\hat{\bu}_{i}$ can be written as $\hat{\bu}_{i} = \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i}$,
where $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise; in the second phase, we apply the result for spectral clustering with small sub-Gaussian noise.
\paragraph{First phase: decomposing the estimator}
For the first phase, 
\begin{align*}
	\hat{\bu}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bx_{i}  \\
	&= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) (\bB\bff_{i}+ \bmu_{y_{i}} + \bepsilon_{i})  \\
	&= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{y_{i}} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
	&:= \tilde{\bmu}_{y_i} + \tilde{\bepsilon}_{i},
\end{align*}
where $ \tilde{\bmu}_{j}:= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T})\bmu_{j} $, $\tilde{\bepsilon}_{i} := (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}$. Let $\bDelta:=\bV_{r}\bV_{r}^{T} -\hat{\bV}_{r}\hat{\bV}_{r}^{T}$, by matrix perturbation theory, we have $\|\bDelta\| \leq O (\sqrt{\frac{\log n}{n}})$ with a high probability (Proposition \ref{matrix_perturbation_proposition}). Then we have for $j_{1} \neq j_{2}$, 
\begin{align*}
	\|\tilde{\boldsymbol{\mu}}_{j_{1}} - \tilde{\boldsymbol{\mu}}_{j_2}\| &= \| (I-\hat{\bV}_{r}\hat{\bV}_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \|  \\
	& \geq \| (\bI-\bV_{r}\bV_{r}^{T})(\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}) \| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \\
	&= \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta (\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2})\| \quad (\text{By (\ref{strict_perpendicularity})}) \\
	& \geq \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| - \|\bDelta\| \| \boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\| \notag \\
	& \geq \frac{1}{2} \|\boldsymbol{\mu}_{j_1} -\boldsymbol{\mu}_{j_2}\|.
\end{align*}
For $\tilde{\bepsilon}_{i}$, 
\begin{align*}
	\tilde{\bepsilon}_{i} &= (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bB\bff_{i} + (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \\
	&= (\bI-\bV_{r}\bV_{r}^{T}) \bB\bff_{i} + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i}  \\
	&= 0 + \bDelta \bB \bff_{i}+ (\bI-\hat{\bV}_{r}\hat{\bV}_{r}^{T}) \bepsilon_{i} \quad (\text{By (\ref{strict_perpendicularity})}) 
\end{align*}
Notice that $\bff_{i} \sim \text{SG}_{r} (c_1^2) $, $\bepsilon_{i} \sim \text{SG}_{d} (\sigma^2)$, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (c(\|\bDelta \bB\|^{2} + \sigma^{2}))$. Also we have
\begin{align*}
	\|\bDelta \bB\|^{2} + \sigma^{2} & \leq \|\bDelta\|^{2} \|\bB\|^{2} + \sigma^{2} \notag \\
	& \leq O(\frac{\log n}{n}) \|\bB\|^{2} + \sigma^{2} \quad (\text{By proposition \ref{matrix_perturbation_proposition}}) \notag \\
	& \leq  O(\frac{d \log n}{n}) + \sigma^{2} \quad (\text{By Assumption \ref{pervasiveness}}) \notag \\
	& \leq O(\frac{1 }{\log n}) + \sigma^{2}  \quad (\text{By the assumption that } d \leq O ( \frac{n}{(\log n)^{2}}) )
\end{align*}
Therefore, when $\sigma^{2} \leq O (\frac{1}{\log n})$, we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\frac{1}{\log n})$. Otherwise we have $\|\bDelta \bB\|^{2} + \sigma^{2} \leq O (\sigma^{2})$. In general, we have $\tilde{\bepsilon}_{i} \sim \text{SG}_{d} (O (\max \{ \frac{1}{\log n}, \sigma^{2}\}))$. Which shows $\tilde{\bepsilon}_{i}$ is a small sub-Gaussian noise.

\paragraph{Second phase: general results for spectral clustering}
For the second phase, we apply the general results for spectral clustering. Suppose we now have data from the following model: 
\begin{align} \label{spectral_clustering_model}
	&\mathbb{P}(y_{i}=j)=p_{j}, \quad j=1,\cdots, K. \notag \\
	&\bx_{i} = \btheta_{y_{i}} + \bepsilon_{i},
\end{align}
where $y_{i}$ is the true label, $\{\btheta_{j}\}_{j=1}^{K}$ is the set of true clustering centers, and $\bepsilon_{i} \sim \text{SG}_{d}(\sigma^{2})$ is independent from all other quantities. The signal-to-noise ratio in this model is defined as 
\begin{equation*}
	\widetilde{\text{SNR}} := \frac{\min_{i\neq j}\|(\boldsymbol{\theta}_{i}-\boldsymbol{\theta}_{j})\|^{2}}{\sigma^2}.
\end{equation*}
We have the following theoretical guarantee for spectral clustering (Algorithm \ref{alg2}), which is a direct consequence of Corollary 3.1 in \cite{zhang2022leaveoneout} with a slight modification (here we use $(1+\epsilon)$-approximate $K$-means).
% (Theorem 3.1 in \cite{abbe2022ellp}): 
\begin{lemma}\label{spectral_clustering_lemma}
	Consider the model defined in (\ref{spectral_clustering_model}). Let $\hat{\by} := (\hat{y}_{1}, \cdots, \hat{y}_{n})$ be the output of Algorithm \ref{alg2}, $\by := (y_{1}, \cdots, y_{n})$ be the true labels. If Assumption \ref{regularity} holds, and $d \leq O (n)$, then there exist constant $C$ and $c$ such that the following hold:
	
	\begin{enumerate}[label=(\alph*)]
		\item If $\widetilde{\text{SNR}} > C \log n $, then $\lim _{n \rightarrow \infty} \mathbb{P}[\mathcal{M}(\hat{\by}, \by)=0]=1$.
		
		\item If $1 \ll \widetilde{\text{SNR}} \leq C \log n$, then $\mathbb{E} [\mathcal{M}(\hat{\by}, \by)] \leq \exp{(-c \cdot \widetilde{\text{SNR}})}$ for sufficiently large $n$.
	\end{enumerate}
\end{lemma}
% See the appendix for the proof of Lemma \ref{spectral_clustering_lemma}. Notice that similar results are already given in many spectral clustering literature, but their proof is usually complicated, due to the fact that $\hat{V}$ is not independent with $\boldsymbol{x}_{i}$. Here we resolve this problem by using the "cross-validation" type algorithm, thus our analysis is much simpler.
Applying Lemma \ref{spectral_clustering_lemma} on $\{\hat{\boldsymbol{u}}_{i}\}_{i=1}^{n}$ will finish the proof for Theorem \ref{main_thm}.  

\begin{remark}
	Notice that the proofs for Lemma \ref{spectral_clustering_lemma} or similar results are very complicated (see \cite{abbe2022ellp,zhang2022leaveoneout}), due to the fact that $\hat{\bV}$ is not independent with $\bx_{i}$. We can resolve this problem by splitting the data to facilitate an easier analysis of spectral clustering algorithm. See Appendix \ref{cv} for further details.
\end{remark} 

